The origin of the high metallicity of close-in giant exoplanets II The nature of the sweet spot for accretion

The composition of giant planets reflects their formation history. Planetesimal accretion during the phase of planetary migration could lead to the delivery of heavy elements into giant planets. In our previous paper (Shibata et al. 2020) we showed that planetesimal accretion during planetary migration occurs in a rather narrow region of the protoplanetary disk, which we refer as "the sweet spot for accretion". The goal of this paper is to reveal the nature of the sweet spot and investigate the role of the sweet spot in determining the composition of gas giant planets. We analytically derive the required conditions for the sweet spot. Then, we compare the derived equations with the numerical simulations. We find that the conditions required for the sweet spot can be expressed by the ratio of the gas damping timescale of the planetesimal orbits and the planetary migration timescale. If the planetary migration timescale depends on the surface density of disk gas inversely, the location of the sweet spot does not change with the disk evolution. The mass of planetesimals accreted by the planet depends on the amount of planetesimals that are shepherded by mean motion resonances. Our analysis suggests that tens Earth-mass of planetesimals can be shepherded into the sweet spot without planetesimal collisions. However, as more planetesimals are trapped into mean motion resonances, collisional cascade can lead to fragmentation of planetesimals. This could affect the location of the sweet spot and the population of small objects in planetary systems. We conclude that the composition of gas giant planets depends on whether the planets crossed the sweet spot during their formation. Constraining the metallicity of cold giant planets, that are expected to be outer than the sweet spot, would reveal key information for understanding the origin of heavy elements in giant planets.

==> Shibata et. al. 2021/newcommands.tex <==
\newcommand{\ikoma}[1]{\textcolor{red}{{\bf #1}}}
\newcommand{\ikome}[1]{\textcolor{magenta}{(\bf #1)}}
\newcommand{\shibata}[1]{\textcolor[rgb]{0,0.5,0}{\bf #1}}
\newcommand{\remove}{\textcolor[gray]{0.8}}

%-------------------------------------
% Abbreviation
\newcommand{\rom}[1]{\MakeUppercase{\romannumeral #1}} %Roman number
\newcommand{\Mcrsb}{M_{\rm oc}^{\rm cr(sb)}}
\newcommand{\comsb}{COM-SB}
\newcommand{\comhp}{COM-HP}

%-------------------------------------
% Units
\newcommand{\s}{{\rm s}}
\newcommand{\g}{{\rm g}}
\newcommand{\erg}{{\rm erg}}
\newcommand{\kg}{{\rm kg}}
\newcommand{\cm}{{\rm cm}}
\newcommand{\m}{{\rm m}}
\newcommand{\km}{{\rm km}}
\newcommand{\AU}{{\rm AU}}

\newcommand{\K}{\rm K}
\newcommand{\yr}{\rm yr}
\newcommand{\yrs}{\rm yrs}

%-------------------------------------
% Physical Parameters
\newcommand{\Gconst}{G}

\newcommand{\Msun}{M_{\odot}}
\newcommand{\Mjup}{M_{\rm Jup}}
\newcommand{\Mear}{M_{\oplus}}
\newcommand{\Rjup}{R_{\rm Jup}}




==> Shibata et. al. 2021/text/App_Method.tex <==
\subsection{Equations of motion}\label{sec:app_eom}
The equation of motion is given by: 
\begin{align}
   \frac{{\rm d} {\bf r}_i }{{\rm d} t} &= \sum_{i\neq j} {\bf f}_{{\rm grav},i,j} + {\bf f}_{\rm aero} +{\bf f}_{\rm tide}, \label{eq:EoM}
\end{align}
where ${\bf r}_i$ is the position vector relative to the initial (i.e., $t = 0$) mass centre of the star-planet-planetesimals system, %$t$ is the time, 
${\bf f}_{{\rm grav},i,j}$ is the mutual gravity between particles $i$ and $j$ given by: 
\begin{align}
   {\bf f}_{{\rm grav},i,j} &= - \mathcal{G} \frac{M_j}{{r_{i,j}}^3} {\bf r}_{i,j} \label{eq:EoM_gravity}
\end{align}
with $\mathbf{r}_{i,j}$ being the position vector of particle $i$ relative to particle $j$ ($r_{i,j} \equiv |{\bf r}_{i,j}|$),
$M_{j}$ is the mass of particle $j$, and $\mathcal{G}$ is the gravitational constant. 
${\bf f}_{\rm aero}$ is the aerodynamic gas drag, and ${\bf f}_{\rm tide}$ is the gravitational tidal drag from the protoplanetary disk gas. 
The central star, planet, and planetesimals  are denoted by the subscripts $i$ (or $j$) = 1, 2, and $\geq$~3, respectively.
The planetesimals are treated as test particles; therefore $f_{{\rm grav},i,j}=0$ in Eq.~(\ref{eq:EoM}) for $j \geq~3$.
The aerodynamic gas drag force and the tidal drag force are given respectively by:  
\begin{align}
  {\bf f}_{\rm aero} &= -\frac{{\bf u}}{\tau_{\rm aero}}, \label{eq:EoM_reduced_gas_drag} \\
  {\bf f}_{\rm tide} &= - \frac{{\bf v}_{\rm p}}{2 \tau_{{\rm tide},a}},
\end{align}
with
\begin{align}
    \tau_{\rm aero} &=  \frac{2 m_{\rm pl}}{ C_{\rm d} \pi R_{\rm pl}^2 \rho_{\rm gas} u} = \tau_{\rm aero, 0} \frac{v_{\rm K}}{u}% \\
%    \tau_{{\rm tide},a} &= \tau_{\rm tide,0} \left( \frac{a_{\rm p}}{1 \AU} \right)^{1/2}. \label{eq:type2_migration_timescale}
\end{align}
Here ${\bf u}={\bf v}_{\rm pl}-{\bf v}_{\rm gas}$ ($u = |{\bf u}|$) is the planetesimal's  velocity (${\bf v}_{\rm pl}$) relative to the ambient gas (${\bf v}_{\rm gas}$), %$\tau_{\rm aero}$ is the timescale of aerodynamic gas drag, 
%$m_{\rm pl}$ is the planetesimal's mass, 
%$C_{\rm d}$ is the non-dimensional drag coefficient and given as $C_{\rm d}=1$, 
%$\rho_{\rm gas}$ is the gas density,
%$R_{\rm pl}$ is the planetesimal's radius,
%${\bf v}_{\rm p}$ is the planet's velocity,
%$a_{\rm p}$ is the planet's semi-major axis,
%and $\tau_{\rm tide,0}$ is a scaling parameter.
%The velocity and density of the ambient disk gas are calculated from the protoplanetary disk model.
Given the range of the planetesimal mass ($\sim10^{16}$-$10^{22} \g$) and planet ($\sim10^{30} \g$), we assume $f_{\rm tide}=0$ for the former and $f_{\rm aero}=0$ for the latter.
The central star is not affected by $f_{\rm aero}$ and $f_{\rm tide}$.

\subsection{Gas disk}\label{sec:app_disk}
\begin{comment}
To focus on the dynamic process, we adopt simply the minimum-mass solar nebula model \citep{Hayashi1981} as our gas disk model. 
We assume that the disk has an axisymmetric, temporally unchanged structure and disregard the difference between the locations between the symmetry axis and the mass centre of the star-planet system.
We also neglect the disk's self-gravity  %meaning no gravitational interaction but 
but include the tidal drag  between the disk and planet.
The surface density $\Sigma_{\rm gas}$ is given by: 
\begin{align}\label{eq:Disk_Gas_MMSN}
    \Sigma_{\rm gas} = \Sigma_{\rm gas,0} \left( \frac{r}{1\AU} \right)^{-\alpha_{\rm disk}},
\end{align}
where $r$ is the radial distance from the initial mass centre of the star-planet system, $\Sigma_{\rm gas,0} = 1.7 \times 10^3 \g/\cm^2$ and $\alpha_{\rm disk}=3/2$.
The disk' temperature $T_{\rm disk}$ is given by: 
\begin{align}
    T_{\rm disk} = T_{\rm disk,0} \left(\frac{r}{1\AU} \right)^{-2\beta_{\rm disk}},
\end{align}
where $T_{\rm disk,0}=280~\K$ and $\beta_{\rm disk}=1/4$.
\end{comment}
The protoplanetary disk is assumed to be vertically isothermal, and the gas density $\rho_{\rm gas}$ is expressed as: 
\begin{align}\label{eq:Disk_Gas_volume}
   \rho_{\rm gas} = \frac{\Sigma_{\rm gas}}{\sqrt{2 \pi} h_{\rm s}} \exp \left( -\frac{z^2}{2 {h_{\rm s}}^2} \right),
\end{align}
where $z$ is the height from the disk mid-plane and $h_{\rm s}$ is the disk's scale height.
The aspect ratio of the protoplanetary disk is given by:  
\begin{align}
    \frac{h_{\rm s}}{r} = \frac{c_{\rm s}}{r\Omega_{\rm K}},
\end{align}
where $\Omega_{\rm K}$ is the Kepler angular velocity and $c_{\rm s}$ is the isothermal sound speed of disk gas.
The sound speed is given as %Assuming locally isothermal case, 
\begin{align}
    c_{\rm s} = \sqrt{\frac{k_{\rm B} T_{\rm disk}}{\mu_{\rm disk} m_{\rm H}}} \propto r^{-\beta{\rm disk}},
\end{align}
where $k_{\rm B}$ is the Boltzmann constant and $\mu_{\rm disk}$ is the mean molecular weight in the unit of proton mass $m_{\rm H}$.
In this study, $\mu_{\rm disk}$ is set as $2.3$ and the aspect ratio of the disk gas at $1\AU$ is $\sim0.03$.

The gas in the protoplanetary disk rotates with a sub-Keplerian velocity because of pressure gradient; namely, $v_{\rm gas} = (1-\eta_{\rm gas}) r \Omega_{\rm K}$, where $\eta_{\rm gas}$ is $\ll 1$ and given as
\begin{align}
	\eta_{\rm gas} &\equiv	\mathbf{-} \frac{1}{2} \left( \frac{h_{\rm s}}{r} \right)^2 \frac{{\rm d} \ln P_{\rm gas}}{{\rm d} \ln r}, \label{eq:eta_gas_definition} \\ 
	               &=		\frac{1}{2} \left( \frac{h_{\rm s}}{r} \right)^2 
	                        \left[ \frac{3}{2} \left( 1 - \frac{z^2}{{h_{\rm s}}^2} \right) +\alpha_{\rm disk} +\beta_{\rm disk} \left(1+\frac{z^2}{{h_{\rm s}}^2}  \right) \right];
\end{align}
$P_{\rm gas}$ is the gas pressure.
%For deriving the above equation, we assume $\eta_{\rm gas} \ll 1$ and use the ideal-gas relation for isothermal sound speed, i.e., $c_{\rm s}^2$ = $P_{\rm gas} / \rho_{\rm gas}$.

\subsection{Planetesimals}
\begin{comment}
For the planetesimals we adopt a simple surface density profile given by: %$\Sigma_{\rm solid}$, which is expressed as
\begin{align}
    \Sigma_{\rm solid} = \Sigma_{\rm solid,0} \left( \frac{r}{1\AU} \right)^{-\alpha_{\rm disk}^{\prime}}, \label{eq:Model_Disk_Solid_Surface_Density}
\end{align}
and set $\alpha_{\rm disk}^{\prime}=\alpha_{\rm disk}=3/2$ and 
\begin{align}
    \Sigma_{\rm solid,0} = Z_{\rm s} \Sigma_{\rm gas,0},    
\end{align}
where $Z_{\rm s}$ is the solid-to-gas ratio (or the metallicity).
We assume that $Z_{\rm s}$ equals the metallicity of the central star.
The planetesimal's mass $m_{\rm pl}$ is calculated as $4\pi\rho_{\rm pl}{R_{\rm pl}}^3/3$, where $\rho_{\rm pl}$ is the planetesimal's mean density and given as $\rho_{\rm pl}=2 \g/\cm^3$.
\end{comment}
The surface number density of planetesimals is given as $\Sigma_{\rm solid}/m_{\rm pl}$ which gives $\sim10^6~/\AU^2$ at maximum.
To speed up the numerical integration, we follow the orbital motion of super-particles.
%The super-particles are distributed in a given radial region, the inner and outer radii of which are denoted by $a_{\rm pl,in}$ and $a_{\rm pl,out}$, respectively. 
The surface number density of super-particles $n_{\rm s}$ is given as: 
\begin{align}
    n_{\rm s} = n_{\rm s,0} \left( \frac{r}{1 \AU} \right)^{-\alpha_{\rm sp}}
\end{align}
where
\begin{align}
    n_{\rm s,0} = \frac{N_{\rm sp}}{2 \pi} \frac{2 -\alpha_{\rm sp}}
                  {\left(a_{\rm pl,out}/1\AU\right)^{2-\alpha_{\rm sp}} -\left(a_{\rm pl,in}/1\AU\right)^{2-\alpha_{\rm sp}} } \left[\frac{1}{\AU^2}\right];
\end{align}
$N_{\rm sp}$ is the total number of super-particles used in a given simulation.
In our simulation, we set $N_{\rm sp}=12,000$ and $\alpha_{\rm sp}=1$ to distribute super-particles uniformly in the radial direction.
The mass per super-particle $M_{\rm sp}$ is given by: 
\begin{align}
    M_{\rm sp} (a_{\rm 0}) = \frac{\Sigma_{\rm solid} (a_{\rm 0})}{n_{\rm s} (a_{\rm 0})} ,
\end{align}
where $a_{\rm 0}$ is the initial semi-major axis of the super-particle.

As for eccentricity and inclination, although planetesimals are treated as test particles in our simulations, assuming that planetesimals are, in reality, scattered by their mutual gravitational interaction, we adopt the Rayleigh distribution as the initial eccentricities $e$ and inclinations $i$ of planetesimals.
We set $\left< e^2 \right>^{1/2}=2\left< i^2 \right>^{1/2}=10^{-3}$.
The orbital angles $\Omega$, $\varpi$ and $\epsilon$ are distributed uniformly.

During the orbital integration, we judge that a super-particle has been captured by the planet once (i) the super-particle enters the planet's envelope or (ii) its Jacobi energy becomes negative in the Hill sphere.
The planet's radius $R_{\rm p}$ is calculated as: 
\begin{align}\label{eq:Rplanet_cap}
    R_{\rm p} = \left( \frac{3 M_{\rm p}}{4 \pi \rho_{\rm p}} \right)^{1/3},
\end{align}
where $\rho_{\rm p}$ is the planet's mean density.
The planet's radius is assumed to be  extended shortly after formation and the density is set to  $\rho_{\rm p}=0.125~\g~\cm^{-3}$, corresponding to a planet's radius twice as large as Jupiter's current radius. 


==> Shibata et. al. 2021/text/conclusion.tex <==
Planetesimal accretion during planetary migration could lead to a significant enrichment of giant planets with heavy elements. 
As revealed in \citet{Shibata+2020}, planetesimal accretion occurs in a sweet spot for planetesimal accretion (\SSP), where planetesimals can be captured by the migrating planet efficiently.
By performing dynamical simulations for planetesimals with a migrating planet, \citet{Shibata+2020} demonstrated that the \SSP\ emerges due to shepherding processes caused by aerodynamic gas drag and mean motion resonances.
However, they conducted no detailed analysis of the nature (especially, the location) of the \SSP\ and therefore in this paper we have focused on the nature of the accretion sweet spot. 

In sec.~\ref{sec:sweet_spot}, we analytically derived an equation describing the location of the \SSP and found the following: 
(i) The  \SSP\ is regulated by the ratio of the damping timescale for the planetesimal eccentricity due to aerodynamic gas drag to the migration timescale of the planet  
(ii) The \SSP\ also depends on the planetary mass, because the accretion bands change with the relative positions between the mean motion resonances and the feeding zone.

In sec.~\ref{sec:sweet_spot_numerical}, we performed numerical simulations and confirmed that the derived conditions reproduce the numerical results well.
In sec.~\ref{sec:discussion}, we discussed the effect of planetesimal collisions and ablation during the shepherding process.
These effects would be important for inner disk region as $\lesssim10\AU$ and put other constraint for planetesimal accretion process.
%{\bf
%We suggest that the mutual collisions of planetesimals in the resonant shepherding is important for determining the population of small objects in planetary systems. 
%}
If the migration timescale is inversely proportional to the disk gas surface density 
\citep[e.g.,][]{Kanagawa+2018}, the timescale ratio is rather insensitive to the structure of the protoplanetary disk.
Therefore, the location of the \SSP\ is fixed during the evolution of the protoplanetary disk.


Finally, we discussed the effect of the \SSP\ on the heavy-element enrichment of gas giant planets.
We suggest that the existence of the \SSP\ makes a difference in the heavy-element mass between planets observed in the regions interior and exterior to the \SSP.
The detailed chemical composition of gas giant planets, such as refractory-to-volatile ratio or C/O ratio, would be also affected by the location of the \SSP.
If such compositional features can be observed, it could be a piece of the evidence of planetesimal accretion during planetary migration.
Future observations in the upcoming decades will reveal whether planetesimal accretion is a main source of heavy elements in giant planets, and therefore advance our understanding of their origin.



==> Shibata et. al. 2021/text/discussion.tex <==
%\subsection{Comparison with \citet{Tanaka+1999}}
\subsection{Collision and ablation of highly-excited planetesimal}
\label{sec:Discussion_Collisions}
Our model neglects the effect of planetesimal collisions.
During the planetary migration, planetesimals are swept by the resonances and the enhanced local density of planetesimals increases the frequency of planetesimal collisions, which might initiate the collisional cascade \citep{Batygin+2015}.
Collisional cascade \citep[e.g.][]{Dohnanyi+1969} changes the size distribution of planetesimals and the perturbation adding on the planetesimal orbits by the collisions would also affect the resonant configuration \citep{Malhotra1993b}.
In this section, we consider the effect of planetesimal collisions on the location of the SSP and the planetesimal accretion.

\subsubsection{Collision timescale of shepherded planetesimals}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{figure/discussion/Axi_Mshep.pdf}
    \caption{
    Maximum mass of planetesimals that can be shepherded in the mean motion resonances without effective mutual collisions.
    We show the cases of $R_{\rm pl}=10^7 \cm$ and $\left< i \right>=10^{-3}$.
    The solid, dashed, and dotted lines correspond to  $\tau_{\mathrm{tide,}a}=10^6 \yr$, $10^5 \yr$ and $10^4 \yr$, respectively.
    }
    \label{fig:Result_Discussion_Mshep}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
First, we estimate the collision timescale using the number density of planetesimals $n_{\rm pl}$, the collision cross section $\sigma$ and the relative velocity $u$.
We consider a swarm of planetesimals that is trapped in mean motion resonances with total mass of $M_{\rm shep}$.
For simplicity, we consider that these planetesimals have the same mass.
The planetesimals are distributed in the ring-like region with a  width of $\sim 2 a\left< e\right>$ and thickness of $\sim 2 a \tan \left< i\right>$.
The collision timescale between these planetesimals $\tau_{\rm col}$ is given as: 
\begin{align}
    \tau_{\rm col}  &= \left( n_{\rm pl} \sigma u \right)^{-1}, \\
                    &= \left(\frac{M_{\rm shep}}{2 \pi a \cdot 2 a \left<e\right> \cdot 2 a \tan \left<i\right>} \cdot \pi {R_{\rm pl}}^2 \cdot \left< e\right> v_{\rm K} \right)^{-1}, \\
                    &= 3\times10^5 \yr \left( \frac{M_{\rm shep}}{10 M_{\oplus}} \right)^{-1} \left( \frac{\rho_{\rm pl}}{2 \g/\cm^3} \right) \left( \frac{R_{\rm pl}}{10^{7}\cm} \right)  \nonumber \\
                    & \left( \frac{a}{10 \AU} \right)^{7/2} \left( \frac{\tan \left< i\right>}{10^{-3}} \right) \left( \frac{M_{\rm s}}{M_{\odot}} \right)^{-1/2}.  \label{eq:tau_collision}
\end{align}
Here, we neglect the effect of gravitational focusing because of the high relative velocities of planetesimals.
$M_{\rm shep}$ increases as the protoplanet migrates and sweeps planetesimals, but decreases after reaching the SSP because the trapped planetesimals start to escape from the mean motion resonances.
As suggested by eq.~(\ref{eq:tau_collision}), $\tau_{\rm col}$ rapidly decreases with the inward planetary migration.
Planetesimals start to collide with each other where the collision timescale $\tau_{\rm col}$ is comparable to the migration timescale $\tau_{\mathrm{tide},a}$.
The maximum mass of planetesimals shepherded into the SSP without active planetesimal collisions $M_{\rm shep,max}$ is estimated as:
\begin{align}
    M_{\rm shep,max} &= 30 M_{\oplus} \left( \frac{\tau_{\mathrm{tide},a}}{10^5 \yr} \right)^{-1} \left( \frac{\rho_{\rm pl}}{2 \g/\cm^3} \right) \left( \frac{R_{\rm pl}}{10^7 \cm} \right) \nonumber \\ 
     &\left( \frac{a}{10 \AU} \right)^{7/2} \left( \frac{\tan \left< i\right>}{10^{-3}} \right) \left( \frac{M_{\rm s}}{M_{\odot}} \right)^{-1/2}. \label{eq:maximum_Mshep}
\end{align}
Figure~\ref{fig:Result_Discussion_Mshep} shows $M_{\rm shep,max}$ as a function of the radial distance from the central star.
During the planetary migration, despite the increase of $M_{\rm shep}$, $M_{\rm shep,max}$ rapidly decreases.
We conclude that the trapped planetesimals collide with each other during the planetary migration phase if the protoplanet migrates a long distance in the radial direction before entering the SSP.


\subsubsection{Collisional cascade in the resonant shepherding}
The outcome of planetesimal collision is determined by the specific energy, which is the kinetic energy of impacting planetesimal normalised by the mass of impacted planetesimal, given by \citep[e.g.][]{Armitage+2010}: 
\begin{align}\label{eq:specific_value}
    Q &= 1.1\times10^{12} {\rm erg}/{\g} \left( \frac{e}{0.5} \right)^2 \left( \frac{R_{\rm im}}{R_{\rm pl}} \right)^{3} \left(\frac{M_{\rm s}}{M_{\odot}} \right) \left( \frac{a}{10 \AU} \right)^{-1},
\end{align}
where $R_{\rm im}$ is the radius of the impacting planetesimal. %and $R_{\rm tg}$ are
The critical value for shattering planetesimals can be scaled as: 
\begin{align}
    Q_{\rm D}^{*} = q_{\rm s} \left( \frac{R_{\rm pl}}{1 \cm} \right)^{a} + q_{\rm g} \rho_{\rm pl} \left( \frac{R_{\rm pl}}{1 \cm} \right)^{b}. \label{eq:specific_value_dispersing}
\end{align}
\citet{Benz+1999} and \cite{Leinhardt+2009} determined the values of fitting parameters in this equation.
For icy planetesimals with an impact velocity of $3\km/\s$, they obtained $q_{\rm s}=1.6\times10^7~\erg/\g$, $q_{\rm g}=1.2~\erg~\cm^3/\g^2$, $a=-0.39$ and $b=1.26$.
Using eq.~(\ref{eq:specific_value}) and (\ref{eq:specific_value_dispersing}), we find that 
km-sized planetesimals are shattered by the collisions of planetesimals larger than $R_{\rm im,th}$, which is given as: 
\begin{align}\label{eq:Rbreak_threathhold}
    \frac{R_{\rm im,th}}{R_{\rm pl}} = 0.13 \left( \frac{R_{\rm pl}}{10^7 \cm} \right)^{0.42} \left( \frac{e}{0.5} \right)^{-2/3} \left(\frac{M_{\rm s}}{M_{\odot}} \right)^{-1/3} \left( \frac{a}{10 \AU} \right)^{1/3}.
\end{align}

We find that collisions of trapped planetesimals easily result in the dispersal and formation of many smaller planetesimals. 
The generated smaller planetesimals shortens the collisional timescale.
Namely, during the planetary migration phase, $M_{\rm shep}$ increases and once it exceeds the threshold value $M_{\rm shep,max}$, the trapped planetesimals start to collide with each other and initiate collisional cascade.
The planetesimal size distribution is largely changed and the major source of solid material would be the smaller planetesimals. % than $R_{\rm pl}$.
As shown by our simulations, the decrease in planetesimal size shifts the location of the SSP outward.
Therefore the possibility of collisional cascade occuring during planetary migration could affect the efficiency of planetesimal accretion.

The value of $M_{\rm shep,max}$ after the initiation of the collisional cascade would be affected by the amount of dispersed planetesimals left in the mean motion resonances. %larger than $R_{\rm im,th}$
Non-dispersed planetesimals with radii of $R_{\rm pl}$ can be supplied as the planet migrates, however,
if a large amount of dispersed planetesimals larger than $R_{\rm im,th}$ are left in the resonance, $M_{\rm shep,max}$ is decreased by a factor of $\sim{R_{\rm im,th}}/{R_{\rm pl}}$ at most.
As we discuss below, impacted planetesimals might be removed from the mean motion resonances and small fragments generated by the collisional cascades would be drifted into the inner disk region faster than the planet.
Thus, after the initiation of the collisional cascade, the size distribution of planetesimals in the resonant shepherding would be affected by various physical processes.
{\bf 
We suggest that the mutual collisions of planetesimals in the resonant shepherding could be important for determining the population of small objects in planetary systems. 
}

In the above discussion, we assumed that the relative velocity of planetesimals $u$ is approximated by $\sim~e~v_{\rm K}$.
However, the alignment of planetesimal orbits via gravitational perturbation from the protoplanet is known to reduce the relative velocity of planetesimals.
\citet{Guo+2021} investigated the effect of orbital alignment due to the secular perturbation which converges the longitude of pericenter into a certain value; namely, planetesimal orbits are aligned on the inertial plane.
Using N-body simulations, they found that the relative velocity of planetesimals are reduced outside the mean motion resonances.
According to their results, orbital alignment is not effective inside the mean motion resonances because of the resonant perturbation.
In the planetary migration phase, however, the resonance angle $\varphi$ {\bf converges} into zero and planetesimal orbits can be aligned on the plane rotating with the protoplanet (see fig.~C1 and C2 in \citet{Shibata+2020}).
In the ideal case, the relative velocity of these planetesimals is smaller than $\sim~e~v_{\rm K}$ and some collisions would result in sticking.
In addition, the mean inclination of planetesimals $\left< i \right>$ is difficult to estimate, but it is important for collision timescale. 
The viscous stirring between trapped planetesimals might affect the mean inclination of planetesimals $\left< i \right>$, which is not considered in our simulations.
Under effective viscous stirring, the velocity dispersion of the planetesimal swarm keeps a simple relation of $\left< e^2 \right>^{1/2}\sim 2 \left< i^2 \right>^{1/2}$ \citep[e.g.][]{Ohtsuki+2002}.
In this case, the collision timescale  increases and $M_{\rm shep,max}$ would be larger than indicated in fig.~\ref{fig:Result_Discussion_Mshep}.
However, it is still unclear whether the energy equipartition works in the resonant trapping where the planetesimal's eccentricity is excited by the protoplanet.
It is clear that  both $M_{\rm shep,max}$ and the planetesimal size distribution depends on the interactions between planetesimals in the mean motion resonances. We suggest that this topic should be investigated in detail in future work. 


\subsubsection{Breakup of resonant trap}\label{sec:Discussion_CompareTI99}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{figure/sweet_spot/time_Phase_wPerturbation.pdf}
    \caption{
    Same as Fig.~\ref{fig:Result_ParameterStudy_time_phase_angle}, but (a) for the case with artificial perturbation given by Eq.~(\ref{eq:artificial_perturbation}) and (b) without artificial perturbation.
    Here we use our reference model with $R_{\rm pl}=1\times10^7\cm$, $\tau_{\rm tide,0}=1\times10^5\yr$ and $M_{\rm p}/M_{\rm s}=1\times10^{-3}$.
    %\ikoma{FOR THE REFERENCE MODEL?}
    }
    \label{fig:Result_Discussion_time_phase_angle_wfp}
  \end{center}
\end{figure}

\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{figure/sweet_spot/ParameterStudy_psMp_wfp.pdf}
    \caption{
    Same as Fig.~\ref{fig:Result_ParameterStudy_Rpl}, but for the results of a parameter study for planetary mass $M_{\rm p}$ with the artificial perturbations (see Eq.~(\ref{eq:artificial_perturbation})).
    In the right panel, the results of a parameter study for planetary mass $M_{\rm p}$ without the artificial perturbations are plotted with gray circles for comparison.
    }
    \label{fig:Result_Discussion_Mp_wfp}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

High-velocity collisions of planetesimals perturb the orbit of trapped planetesimals and break the resonant trapping.
Using numerical simulations, \cite{Malhotra1993b} found that for a planet of 10 $M_\oplus$, resonant trapping is broken with a velocity kick of $\gtrsim0.003 v_{\rm K}$. 
Therefore, once $M_{\rm shep}$ exceeds the threshold value and the trapped planetesimals start to collide with each other, the resonant trapping can be broken by planetesimal collisions.
However, the resonant width increases with increasing planetary mass (see Eq.~(\ref{eq:1st_order_resonant_width}); namely breaking the resonant trapping is more difficult for more massive planets) and not all high-velocity collisions lead to the breaking of resonant trapping (see Fig.~6b of \citet{Malhotra1993b}).
In addition, as mentioned in the previous section, the alignment of the orbits by the resonant trapping might reduce the relative velocity of planetesimals.
The possibility of resonant breaking by the planetesimal collisions need to be investigated in future work.
Here, we consider the cases where the resonant trapping is broken by planetesimal collisions.

As shown in sec.~\ref{sec:sweet_spot}, planetesimal accretion occurs only in a limited ring-like region within the protoplanetary disk.
This accretion process seems different from the one found for Earth-mass planets in  \citet{Tanaka+1999}.
In their dynamical simulations, \citet{Tanaka+1999} broke the resonant traps instantaneously by exerting artificial perturbations on the trapped planetesimals (see below), supposing that the planetesimals have their motion changed via the interactions with other planetesimals. Then, comparing the timescale for the protoplanet's migration with that for scattering of planetesimals by the migrating protoplanet, they derived a condition required for planetesimal accretion as: 
\begin{align}
    \tau_{{\rm tide},a} &< 0.81 \left\{ \sqrt{1+0.45 \left(\frac{\tau_{\rm aero,0}}{T_{\rm K,p}} \right)^{2/3} } +1 \right\}^2 \frac{T_{\rm K,p}}{h^{2}}. \label{eq:critical_migration_timescale_Tanaka+1999}
\end{align}
By contrast, when deriving Eq.~(\ref{eq:sweet_spot}) and also performing the dynamical simulations, we considered an extreme case without such modification to the planetesimals motion.


Using the artificial perturbation developed in \citet{Tanaka+1997}, we perform additional numerical simulations.
We randomise the phase angle by adding displacements in orbital elements except $a$, $e$ and $i$. 
The size of the displacement is set as: 
\begin{align}
    \Delta \theta = 2 \pi f_{\rm p}, \label{eq:artificial_perturbation}
\end{align}
where $f_{\rm p}$ is a scaling factor of perturbation strength and randomly given from $-0.01$ to $0.01$.
We add $\Delta \theta$ to orbital angles (longitude of ascending node $\Omega$, longitude of pericentre $\varpi$ and mean longitude at epoch $\epsilon$) every conjunction time.
Figure~\ref{fig:Result_Discussion_time_phase_angle_wfp} shows the temporal change in the phase angle in the case with (a) and without (b) the artificial perturbations.
As shown in panel~(a), even under strong perturbations (corresponding to up to $1~\%$ displacement in the phase angle at every conjunction), the mean motion resonances with a Jupiter-mass planet are efficient in trapping planetesimals and, thereby, resonance shepherding occurs. This is because the resonance width (see Eq.~(\ref{eq:1st_order_resonant_width})) is larger for Jupiter-mass planets than that for Earth-mass planets.
The perturbations is, however, found to hasten the breakup of resonant trapping, because resonant trapping is weakened and over-stable libration is accelerated.

Figure~\ref{fig:Result_Discussion_Mp_wfp} shows the results of the parameter study when varying the planetary mass $M_{\rm p}/M_{\rm s}$ including the artificial perturbations given by Eq.~(\ref{eq:artificial_perturbation}).
For comparison, we also show the results without artificial perturbations with open circles in the right panel. 
Due to the artificial perturbations, the \SSP\ shifts outward (see the left panel) and the total mass of captured planetesimals is reduced (see the right panel). 
In the left panel, the black solid line shows the condition of shepherding obtained in \citet{Tanaka+1999} (see eq.~(\ref{eq:critical_migration_timescale_Tanaka+1999})); planetesimal accretion occurs in regions exterior to it. 
This black line corresponds to the inner boundary of the \SSP\ for the case where resonant traps are perfectly broken.
Although it might seem counter-intuitive, we conclude that without perturbations, resonant trapping shifts the \SSP\ inward and enhances planetesimal accretion due to the effect of accretion bands.


\subsubsection{Ablation of eccentric planetesimals}\label{sec:Discussion_Ablation}
A highly-excited planetesimal has a high relative velocity compared to that of the disk gas.
Strong gas drag from the gaseous disk \citep[e.g.,][]{Pollack+1986} and generated bow-shock \citep[e.g.,][]{Tanaka+2013} heats the planetesimal's surface and triggers the ablation of volatile materials.
Planetesimals trapped in the mean motion resonances have eccentric orbits and feel strong gas drag, and therefore ablation is expected to be important.
The ablation rate depends on the rate of heat transfer from the ambient disk gas $\Lambda$.
We set $\Lambda$ to range between  $0.003$ and $0.6$ for gas drag heating, and between $\sim0.01$ and $\sim0.1$ for bow shock heating \citep[see][and references therein]{Tanaka+2013}.
Recently \citet{Eriksson+2021} explored the possibility of perfect ablation of planetesimals around a  massive protoplanet using $\Lambda=C_{\rm d}/4$, which is the upper limit of the heat transfer rate \citep{DAngelo+2015}.
According to their nominal model result, ablation of highly excited planetesimals is effective in the inner disk region $\lesssim10\AU$ and large amount of solid materials are ablated.
The heating process strongly depends on the eccentricity of planetesimals.
Using eqs.~(\ref{eq:equilibrium_resonant_argument_app}) and (\ref{eq:sweet_spot}), we find that the eccentricity of planetesimals inside the SSP decreases from $\sim0.5$ to $0.1$.
To avoid effective ablation planetesimals must enter the SSP in the outer disk region $\gtrsim10\AU$.
If the secular resonance triggered by the disk's gravity is effective, the ablation would be effective  in more outer disk region \citep{Nagasawa+2019}.
On the other hand, if $\Lambda$ is much smaller than $C_{\rm d}/4$, the ablation of planetesimals would be inefficient.

The investigation presented above concerning planetesimal collision and ablation implies that planetesimal accretion is favoured in the outer disk region $\gtrsim10\AU$. 
Detailed future studies that focus on collision and ablation processes are clearly desirable. 







\subsection{The case of Type II migration with shallow-gap}\label{sec:Discussion_Kanagawa}
In the classical picture of the Type II migration \citep[e.g.][]{Lin+1993}, a giant planet migrates with a deep gap opened in the vicinity of its orbit in a gaseous protoplanetary disk. 
For an extremely deep gap, the radial gas flow toward the central star is stemmed completely by the gap and, consequently, the planet migrates with the gaseous disk contracting via viscous diffusion.
Recent hydrodynamic simulations, however, reveal that the gap bottom is not so deep and the gas can cross the gap \citep{Kanagawa+2015,Kanagawa+2016,Kanagawa+2017}.
In this case, the planetary migration is not in the classical regime; instead, the torque exerted on the planet is given similarly to that in the Type I regime \citep{Kanagawa+2018}.
Thus, the migration timescale in the new type II regime is written as: 
\begin{align}\label{eq:type2_migration_regime_K18} 
    \tau_{\rm tide,{\it a},II} &\sim  \frac{1}{2 c} \left(\frac{M_{\rm p}}{M_{\rm s}}\right)^{-1} 
                                \left(\frac{{r_{\rm p}}^2\Sigma_{\rm gap}}{M_{\rm s}}\right)^{-1} 
                                \left(\frac{h_{\rm s}}{r_{\rm p}} \right)^2 {\Omega_{\rm K}}^{-1}, 
\end{align} 
where $c$ is a constant of the order of unity and $\Sigma_{\rm gap}$ is the surface density of disk gas at the gap bottom; $\Sigma_{\rm gap}$ depends on the unperturbed surface density of disk gas $\Sigma_{\rm gas}$ and is given from the hydrodynamic simulations of \citet{Kanagawa+2017} as: 
\begin{align}\label{eq:gap_Kanagawa}
    \Sigma_{\rm gap} = \frac{\Sigma_{\rm gas}}{1+0.04 K},
\end{align}
with
\begin{align}
    K = \left( \frac{M_{\rm p}}{M_{\rm s}} \right)^2 \left( \frac{h_{\rm s}}{r_{\rm p}} \right)^{-5} {\alpha_{\rm vis}}^{-1},
\end{align}
where $\alpha_{\rm vis}$ is the alpha parameter for disk gas turbulent viscosity \citep{Shakura+1973}.
From Eqs.~(\ref{eq:type2_migration_regime_K18}) and (\ref{eq:gap_Kanagawa}), we obtain: 
\begin{align}
    \tau_{{\rm tide},a,{\rm II}} &\sim   \frac{0.02}{c} {\alpha_{\rm vis}}^{-1} \left(\frac{{r_{\rm p}}^2\Sigma_{\rm gas}}{M_{\rm p}}\right)^{-1} 
                                \left(\frac{h_{\rm s}}{r_{\rm p}} \right)^{-3} {\Omega_{\rm K}}^{-1}, \label{eq:type2_migration_regime_simple}
\end{align}
for $1 \ll 0.04 K$ or 
\begin{align}
    M_{\rm p} \gg 8 M_{\oplus} \left( \frac{\alpha_{\rm vis}}{10^{-3}} \right)^{1/2} \left( \frac{r_{\rm p}}{1 \AU} \right)^{5(1-2\beta_{\rm disk})/4}.
\end{align}
Here we discuss the location of SSP and planetesimal accretion onto the protoplanet migrating with eq.~(\ref{eq:type2_migration_regime_simple}).

\subsubsection{The location of the accretion sweet spot}\label{sec:Discussion_SweetSpot}
The location of the \SSP\ depends on the ratio of the planetary migration and aerodynamic gas drag timescales.
The timescale of damping by aerodynamic gas drag $\tau_{\rm aero,0}$ in the disk mid-plane also depends on the disk structure (see Eq.~(\ref{eq:aerodynamic_damping_timescale})) as: 
\begin{align}
    \tau_{\rm aero,0} &= \frac{8\sqrt{2\pi}}{3 C_{\rm d}} \left(\frac{\Sigma_{\rm gas}}{\rho_{\rm pl} R_{\rm pl}}\right)^{-1} \frac{h_{\rm s}}{r_{\rm pl}} {\Omega_{\rm K}}^{-1}. \label{eq:damping_timescale_simple}
\end{align} %
Note that $\tau_{\rm tide,{\it a},II}$ is a function of $r_{\rm p}$, whereas $\tau_{\rm aero,0}$ is a function of $r_{\rm pl}$; $r_{\rm p}/r_{\rm pl}=((j-1)/j)^{2/3}$ for a planetesimal in the $j$:$j-1$ mean motion resonance with the planet.
In this case, Eq.~(\ref{eq:damping_timescale_simple}) can be written as a function of $r_{\rm p}$ as: 
\begin{align}
    \tau_{\rm aero,0} &= \frac{8\sqrt{2\pi}}{3 C_{\rm d}} \left(\frac{\Sigma_{\rm gas}}{\rho_{\rm pl} R_{\rm pl}}\right)^{-1} \frac{h_{\rm s}}{r_{\rm p}} {\Omega_{\rm K}}^{-1} \left(\frac{j-1}{j}\right)^{2\gamma_{\rm disk}/3}, \label{eq:damping_timescale_simple2}
\end{align}
with
\begin{align}
    \gamma_{\rm disk} = 2+\alpha_{\rm disk} -\beta_{\rm disk}. \label{eq:sweet_spot_constant_gamma}
\end{align}
Here, we have assumed that the planetesimals trapped in mean motion resonances are outside the gap.
If the disk viscosity is small, however, the gap slope reaches the locations of the resonances; in that case, the damping timescale increases a few times.
For simplicity, we neglect this effect.

From Eqs.~(\ref{eq:type2_migration_regime_simple}) and (\ref{eq:damping_timescale_simple2}), the ratio of the two timescales is given by: 
\begin{align}
    \frac{\tau_{\rm aero,0}}{\tau_{{\rm tide},a,{\rm II}}} = 
    1 \times10^{-6} C^{-1} \left(\frac{M_{\rm p}}{M_{\rm s}}\right)^{-1} 
                                                                                \left(\frac{r_{\rm p}}{1\AU}\right)^{4(1-\beta_{\rm disk})}
                                                                                \left(\frac{j-1}{j}\right)^{2\gamma_{\rm disk}/3}, \label{eq:fraction_timescales_simple}
\end{align}
with
\begin{align}
    C       &=  \frac{2C_{\rm d}}{c}
                \left(\frac{\alpha_{\rm vis}}{10^{-3}}\right)^{-1}
                \left(\frac{\rho_{\rm pl}}{2 \g/\cm^3}\right)^{-1}
                \left(\frac{R_{\rm pl}}{10^7~\cm}\right)^{-1}
                \left(\frac{M_{\rm s}}{M_{\rm \odot}}\right)
                \left(\frac{\left|h_{\rm s}/r\right|_{\rm 1\AU}}{0.03}\right)^{-4}, \label{eq:sweet_spot_constant_C}
\end{align}
Equation~(\ref{eq:fraction_timescales_simple}) indicates that the surface gas density profile only weakly affects the timescale ratio, which does not explicitly depend on $\Sigma_{\rm gas}$ and weakly depends on $\alpha_{\rm disk}$, namely, $((j-1)/j)^{2\alpha_{\rm disk}/3}$. 
This means that as the protoplanetary disk evolves, the timescale ratio hardly changes, suggesting that the location of the \SSP\ is fixed. % during the planetary formation stage.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}%f1
    \begin{center}
    \includegraphics[width=80mm]{figure/discussion/SweetSpot4.png}
        \caption{
        Distribution of confirmed exoplanets in the semi-major axis vs. planetary mass plane 
        (http://exoplanet.eu).
        The black points are exoplanets observed by the radial-velocity method.
        The red points are exoplanets observed by the radial-velocity + transit methods.
        As for masses of exoplanets indicated with the black points, the observe values of $M_{\rm p} \sin i$ are simply used.
        The gray area shows the theoretical sweet spot for planetesimal capture given by Eqs.~(\ref{eq:sweet_spot_in_disk_1}) and (\ref{eq:sweet_spot_in_disk_2}) with $C=10$. 
        The red dashed line shows the theoretical sweet spot for planetesimal capture with $C=10^3$, which corresponds to the case where collisional cascade broke planetesimals down to $R_{\rm pl}\lesssim10^5 \cm$. 
        }
        \label{fig:Application_Exoplanet}
    \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Assuming $\alpha_{\rm disk}$ = 1, which is valid in a steady viscous accretion disk except for its outermost region 
\citep[e.g.][]{Lynden-Bell+1974}, and $\beta_{\rm disk} = 1/4$, which is valid in an optically thin disk, and substituting Eq.~(\ref{eq:fraction_timescales_simple}) into Eq.~(\ref{eq:sweet_spot}), we obtain the semi-major axes of the inner and outer edge of \SSP\ , $a_{\rm SS,in}$ and $a_{\rm SS,out}$, respectively, as: 
\begin{align}
    a_{\rm SS,in} &= {\rm max} \left.
            \begin{cases}
                1 C^{1/3} \left(\frac{M_{\rm p}/M_{\rm s}}{10^{-3}}\right)^{2/3} \left(\frac{j}{j-1} \right)^{10/9} \\%1.4 
                1 C^{1/3} \left(\frac{M_{\rm p}/M_{\rm s}}{10^{-3}}\right)^{1/3} \left\{\frac{j^{11}}{(j-1)^5} \right\}^{1/18} \frac{e_{\rm cross}}{0.1}
            \end{cases} \right\} \AU, \label{eq:sweet_spot_in_disk_1} \\%1.1 
    a_{\rm SS,out} &= 8 C^{1/3} \left(\frac{M_{\rm p}/M_{\rm s}}{10^{-3}}\right)^{1/3} \left\{ \frac{j^{11}}{(j-1)^{14}} \right\}^{1/18} \AU. \label{eq:sweet_spot_in_disk_2}%7.6
\end{align}

Figure~\ref{fig:Application_Exoplanet} shows exoplanets identified so far and the predicted location of the \SSP\ in the $a_{\rm p}$-$M_{\rm p}$ plane for {\bf $C=10$}.
The \SSP\ locates from $\sim$ 1~$\AU$ to $\sim$ 30~$\AU$ and shifts outward with increasing planetary mass.
The red and black symbols show exoplanets observed using the transit method and the radial velocity method, respectively (http://exoplanet.eu).
Given that planetary growth occurs via the runaway gas accretion, followed by inward migration, the evolution path of a gas giant planet can be drawn from right-bottom to left-top direction in the $a_{\rm p}$-$M_{\rm p}$ plane \citep[e.g.,][]{Ida+2004a,Mordasini+2009a}. 
If runaway gas accretion begins in outer disk region, which might be favoured for planetary core formation because of the increasing isolation mass of protoplanet \citep[e.g.][]{Armitage+2010}, the exoplanets currently observed in the region interior to the \SSP\ must have crossed the \SSP\ during their formation stages. 

\subsubsection{Maximum mass of planetesimals shepherded into the SSP}\label{sec:Discussion_SweetSpot_Mshep}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}%f1
  \begin{center}
    \includegraphics[width=80mm]{figure/discussion/Mp_Mshep.pdf}
    \caption{
    The maximum mass of planetesimals shepherded into the SSP without active planetesimal collisions $M_{\rm max,shep}$ as a function of planetary mass $M_{\rm p}$.
    Here, we consider the case where the protoplanet migrates with the type II regime obtained by \citet{Kanagawa+2018} (see eq.~(\ref{eq:type2_migration_regime_K18})).
    The solid and dashed lines show the cases of $\left< i \right>=10^{-3}$ and $10^{-2}$, respectively.
    The black and red lines are cases of massive disk with $\Sigma_{\rm gas,0}=1400 \g/\cm^2$ and $800 \g/\cm^2$, respectively.
    We adapt the optically thick disk of $T_{\rm 0}=140 \K$, the disk viscosity $\alpha_{\rm vis}=10^{-3}$, the size of planetesimal $R_{\rm pl}=10^7 \cm$ and the planetesimal density $\rho_{\rm pl}=1 \g/\cm^3$.
    The scaling parameter of the location of the SSP $C$ is obtained as $C=17$.
    }
    \label{fig:Mp_Mshep}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The total mass of accreted planetesimals depends on the amount of planetesimals that  shepherded into the SSP. 
By substituting eqs.~(\ref{eq:resonant_center}), (\ref{eq:type2_migration_regime_simple}) and (\ref{eq:sweet_spot_in_disk_2}) into eq.~(\ref{eq:maximum_Mshep}), we can estimate $M_{\rm shep,max}$ when the protoplanet reaches the outer edge of the SSP.
In this case, $M_{\rm shep,max}$ weakly depends on $\alpha_{\rm vis}$, $\rho_{\rm pl}$, $R_{\rm pl}$ and ${M_{\rm p}}^{-1}$ ($-1/4$ powers of each value), but linearly depends on $\tan \left< i \right>$, $\Sigma_{\rm gas,0}$ and ${T_{\rm 0}}^{-1}$.
Here, we adapt the optically thick disk of $T_{\rm 0}=140\K$ \citep{Sasselov+2000} and consider two disks with  $\Sigma_{\rm gas,0}=1400 \g/\cm^2$ and $800 \g/\cm^2$.
The former disk corresponds to the massive disk of total mass $0.1 M_{\rm s}$ and typical radius $100\AU$.
Figure~\ref{fig:Mp_Mshep} shows $M_{\rm shep,max}$ as a function of planetary mass $M_{\rm p}/M_{\rm s}$.
We find that a few tens $M_{\oplus}$ of planetesimals can be shepherded into the SSP before initiating collisional cascade even with $\tan\left< i \right>=10^{-3}$.
For the capture of several tens or more planetesimals,  the effect enhancing $\tan\left< i \right>$ needs to be considered. 

Note that $M_{\rm shep,max}$ only provides the maximum mass of planetesimals shepherded into the SSP and not the mass of  planetesimals that can be captured by the protoplanet.
The numerical simulations we presented in sec.~\ref{sec:sweet_spot_numerical} suggest that $\sim 30\%$ of the shepherded planetesimals are captured by the protoplanet. 
This accretion efficiency, however, depends on various parameters such as the inclination of planetesimals \citep{Tanaka+1999} and the planetary capture radius \citep{Inaba+2003}.
In addition, the initial semi-major axis of planetesimals also affects the capture efficiency because of the mean motion resonances. 
A detailed investigation of the accretion efficiency under various conditions should be conducted in future research.  









\subsection{Heavy-element enrichment of giant planets}\label{sec:Application_Model_InnerPlanet_result}
If giant planets cross the sweet spot during the migration phase, planetesimal accretion could take place.
If tens Earth-masses of planetesimals were shepherded into the SSP as shown in fig.~\ref{fig:Mp_Mshep}, we would expect a clear difference in the total heavy-element mass of planets depending on whether they migrated interior or exterior to the \SSP.
If such a difference between planetary populations is observed, it could confirm that planetesimal accretion is a significant process that takes place during planetary migration. 
However, once the collisional cascade occurs, the location of the SSP moves to the outer disk region and the metallicity difference between the populations would be reduced.
It is therefore still unclear whether such a difference is detectable. 

Currently, there are no estimated  metallicities for giant exoplanets within the outer disk region (i.e., at distances  $\gtrsim 10\AU$).
To estimate the metallicity of giant exoplanets, measurements of the radius, mass and age of the planet are required. 
At the moment, data of the masses and radii of cold giant planets are still unavailable.
Nevertheless, the upcoming decades are expected to provide vast observations thanks to various missions.
Wide field observations, such as TESS and Plato, will increase the number of cold giant planets \citep{Ricker+2014,Rauer+2014}.
Follow-up observations using precise radial velocity measurement, such as HARPS \citep{Mayor+2003} and ESPRESSO \citep{Pepe+2010}, and precise transit measurement, such as NGTS \citep{Wheatley+2018} and WASP \citep{Pollacco+2006}, are suitable for obtaining the masses and radii of giant planets at large radial distances. 
In addition, high-dispersion coronagraphy technique \citep[e.g.][]{Kotani+2020} could  constrain the atmospheric composition of cold giant planets.
Next generation observations will constrain the main source of heavy elements.


In this study, we focus on planetesimal accretion and consider it as the main source of heavy-element enrichment in gas giant planets.
However, other various processes could also lead to heavy-element enrichment. 
The metallicity of the gaseous disk can be enriched by the sublimation of dust grains and pebbles crossing each ice lines \citep{Booth+2017,Booth+2019}. 
The accretion of these enriched disk gas brings massive heavy elements into gas giant planets \citep{Schneider+2021}.
Giant impacts have also been investigated as a source of enrichment  \citep{Ikoma+2006b,Liu+2015,Liu+2019,Ginzburg+2020, Ogihara+2021}.
By combining the effects of pebble accretion and giant impacts, \citet{Ogihara+2021} found that up to $\sim100~M_{\oplus}$ of heavy elements can be accreted by a giant planet through multi-giant impacts of Neptune-mass planets.

In order to determine what is the main source of the heavy-element enrichment in giant exoplanets, other observational information such as elemental ratios (refractory-to-volatile, C/O, O/H, etc) is valuable. 
In recent observations, the existences of TiO and VO in Hot-Jupiters is suggested by the transmission spectrum analysis \citep{Evans+2016,Chen+2021}.
The amount of these refractory materials is useful for constraining the dominant process of heavy-element accretion.
The accretion of massive refractory materials is only possible through solid accretion, thus using the information of refractory materials, we can constrain whether the heavy elements are brought by solid accretion or gas accretion.

The elemental ratio of volatile materials also provides information on the accretion process of heavy-elements \citep[e.g.,][]{Madhusudhan+2014,Notsu+2020,Turrini+2021,Schneider+2021}.
\citet{Turrini+2021} investigated the effect of planetesimal accretion on elemental ratios of volatile materials such as C/O, N/O or S/N.
They considered a Jupiter-mass planet in a typical disk model, however, the relative position between the \SSP\ and each ice lines changes with the planetary mass and disk conditions.
The elemental ratio of planetesimals shepherded into the  \SSP\ would depend on the evolution pathways of the giant planets on the $a_{\rm p}$-$M_{\rm p}$ plane and disk conditions.
We hope to further investigate the link between elemental ratios and the formation history in followup studies. 
This is highly relevant since future missions like JWST and Ariel will provide accurate measurements of the atmospheric composition of gaseous planets that can then be used to better understand the planetary origin. 







==> Shibata et. al. 2021/text/intro.tex <==
The formation of gas giant planets is a complex process which involves many underlying physical processes, such as core formation, gas accretion, and planetary migration.
Recent planetary population synthesis models \citep[e.g.,][]{Ida+2018,Mordasini2018} aim to consider as many processes as possible and construct a  comprehensive planetary formation model which begins at the early stages of planetesimal accretion up to the formation of gas giant planets.
However, there are still many uncertainties related to each of these processes as well as the initial conditions. 
%which are not observable in current planetary systems.
Constraining theories using observed physical parameters is crucial for understanding the formation and evolution  of gas giant planets.
Along with the development of observation and characterisation of exoplanets, many studies aimed to validate theoretically proposed formation models and  constrain the initial parameters that control giant planet formation. 
The planetary chemical composition is a key characteristic that can be used to constrain formation models because the formation history is imprinted in the composition of gas giant planets. %and internal structure 

Recent observations provide information on the chemical composition of gas giant planets. %, in particular, when it comes to giant exoplanets.
Typically it is the planetary metallicity is used for their characterisation and for constraining their formation and evolution histories \citep[e.g.,][]{Helled2021}.  
The composition of gas giant planets was first constrained for the solar-system giant planets Jupiter and Saturn \citep[e.g.][]{Guillot+1999,Saumon+2004}.
From the gravitational moments observed by spacecrafts, the total heavy-element mass in Jupiter $M_{\rm Z,Jup}$ was estimated to be  $\sim25$-$45\Mear$ \citep{Wahl+2017,Debras+2019} and $M_{\rm Z,Sat}\sim16$-$30\Mear$ for Saturn \citep{Saumon+2004,Helled+2013,Movshovitz+2020,Mankovich+2021}. 
Heavy-element enrichment has also been inferred for giant exoplanets  \citep[e.g.,][]{Guillot+2006,Miller+2011,Thorngren+2016}.
According to \citet{Thorngren+2016}, close-in gas giant planets contain large amounts of heavy elements of the order of tens of Earth masses, with  bulk planetary metallicities that are significantly higher than stellar metallicities. 
Surprisingly, some of these planets are estimated to consist of more than $\sim100\Mear$ of heavy elements.
Revealing the origin of this significant heavy-element enrichment in giant planets is a key objective in giant planet formation theory. 

Planetesimal accretion has been proposed to be one of the main sources of heavy-element enrichment of giant planets. 
After the onset of runaway gas accretion, a large amount of planetesimals enters the expanding feeding zone where the planetesimals can be captured by the protoplanet \citep{Zhou+2007,Shiraishi+2008,Shibata+2019,Podolak+2020}.
During the rapid gas accretion phase, up to 30\% of planetesimals inside the feeding zone are captured by the protoplanet \citep{Shibata+2019}.
For a massive protoplanetary disk, this accretion process is sufficient to explain the estimated heavy-element masses in Jupiter and Saturn.
For close-in giant exoplanets,  however, the heavy-element mass that  accreted during rapid gas accretion  is rather low because the total mass planetesimals inside the feeding zone of these planets is significantly lower. 


During the planetary migration phase, migrating planets encounter planetesimals in wide regions within the  protoplanetary disk.
Planetesimal accretion during  the migration phase was investigated in the context of accelerating the formation of Jupiter's core \citep[e.g.][]{Tanaka+1999,Alibert+2005}.
It was found that the formation timescale of Jupiter's core can be shortened if planetary migration is included.  
For the origin of large amounts of heavy elements in close-in giant exoplanets, planetesimal accretion by a migrating Jupiter-size planet was also investigated by \citet{Shibata+2020} and \citet{Turrini+2021}.
\citet{Shibata+2020} performed  orbital integration calculations of planetesimals around a migrating planet,  and found that several-tens Earth mass of planetesimals can be accreted by a gas giant planet if the planet migrates tens of AU in a massive protoplanetary disk.
\citet{Turrini+2021} also investigated this process and found that planetesimal accretion during planetary migration is a useful tracer of the formation location of giant planets.
Thus, planetesimal accretion during the planetary migration phase is a key mechanism in the formation history of gas giant planets. 

If the migrating planet is as massive as Jupiter, efficient planetesimal accretion is limited to a narrow ring-like region within the  protoplanetary disk \citep{Shibata+2020}; in this paper, we refer to this region  as the {\it sweet spot for planetesimal accretion} (hereafter, \SSP).
Even in the case of a migrating  Earth-mass planet, the accretion area is limited to an outer disk region (without outer edge) because of the disk gas drag \citep{Tanaka+1999}.  However, such a ring-like region of \SSP\ is specific to the Jupiter-mass planet.
The shape and location of the accretion region 
%are important for determining the accretion efficiency because the total heavy-element mass of captured planetesimals 
during the  planetary migration determine the accretion area and the accretion efficiency. 
The accretion area of planets with  different masses depends on the strength of mean motion resonances accompanied by the migrating planet.
Nevertheless, the detailed nature of \SSP\ is not fully understood.

In this paper, we investigate the nature of \SSP \ in detail and derive analytical equations for determining its location.
In sec.~\ref{sec:sweet_spot}, we analytically investigate the orbital evolution of planetesimals around the migrating planet.
We derive a condition required for planetesimal accretion during the  planetary migration phase.
In sec.~\ref{sec:sweet_spot_numerical}, we compare the derived condition with the numerical simulations.
In sec.~\ref{sec:discussion}, we discuss about the location of \SSP\ in a protoplanetary disk and the heavy-element enrichment of giant planets.
Our conclusions are summarised in Section~\ref{sec:conclusion}. 






==> Shibata et. al. 2021/text/sweet_spot.tex <==

\subsection{An overview of planetesimal accretion during planetary migration}\label{sec:overview}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=90mm]{figure/sweet_spot/Axi_Ecc.pdf}
    \caption{
    Orbital evolution of a planetesimal initially located at $13.8\AU$ dictated via the gravitational interaction with a migrating Jupiter-mass protoplanet. 
    The dots and crosses show the locations of the planetesimal and the protoplanet, respectively, and are colour-coded according to time.
    In this simulation the surface density of disk gas is 
    set to that of the minimum-mass solar nebula and aerodynamic gas drag is included. 
    Here the protoplanet migrates from $15.0\AU$ with migration rate of $10^5$ AU/yr.
    For the details of the numerical simulation, see sec.~\ref{sec:sweet_spot_numerical}.
    }
    \label{fig:axi_ecc}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Mean motion resonances play an important role in the accretion of planetesimals onto a migrating protoplanet.
Here, we summarise the orbital evolution of planetesimals dictated via their gravitational interaction with a migrating protoplanet, which as found by the numerical simulations of \citet{Shibata+2020}.
Figure~\ref{fig:axi_ecc} shows the orbital evolution of a planetesimal initially located at $13.8\AU$ around a migrating Jupiter-mass protoplanet. 
The orbital evolution of the planetesimal is divided into three characteristic phases as discussed below.

First phase ($t=0~\yr$ -- $4\times10^5~\yr$; bluish symbols): 
The planetesimal encounters the migrating protoplanet and is trapped in the $2:1$ mean motion resonance; this phenomenon is referred to as the \textit{resonant trapping}.
The planetesimal trapped in the mean motion resonance is transported inward together with the migrating protoplanet and its eccentricity is highly enhanced.
This phenomenon is known as the {\it resonant shepherding} \citep[][]{Batygin+2015}.

Second phase ($t=4\times10^5~\yr$ -- $7\times10^5~\yr$; green-yellow symbols): 
As time progresses the resonantly-trapped planetesimal starts to escape from the mean motion resonance, and its eccentricity begins to decrease.
This is because of the stronger aerodynamic drag in the inner regions.
The break of resonant trapping shown in Fig.~\ref{fig:axi_ecc} is caused by overstable liblation \citep{Goldreich+2014}.
The eccentricity of the trapped planetesimal is excited through gravitational scattering by the migrating protoplanet but is also damped by the disk gas drag. 
This overstable equilibrium condition makes the planetesimal orbit unstable and breaks the resonant trapping.

Third phase ($t=7\times10^5~\yr$ --; reddish symbols): 
In the farther inner region, the disk gas is dense enough that the resonantly-trapped planetesimal is damped faster than the planetary migration and, therefore, the planetesimal is eliminated from the feeding zone.
We refer to this phenomenon as the {\it aerodynamic shepherding}, which was found by \citet{Tanaka+1999} in the context of terrestrial planet formation. 

According to the numerical simulations preformed in \citet{Shibata+2020}, planetesimal accretion occurs during the second phase, and the region in which for efficient planetesimal accretion occurs is referred to as \SSP. 
During the first and third phases, planetesimal accretion is negligible.  
The existence of these three different phases (or regions) is associated with the change in strength of the aerodynamic gas drag which increases as the protoplanet migrates inward.

In the following sections, we derive the conditions for the \SSP\ analytically. 
In Sec.~\ref{sec:condition_for_resonant_trapping}, we show that planetesimals are generally trapped in the mean motion resonances with an approaching protoplanet in standard protoplanetary disks. 
In Sec.~\ref{sec:orbital_evolution_in_resonant_trapping}, we show that the eccentricity of the resonantly-trapped planetesimal reaches an equilibrium value, $e_{\rm eq}$, that is determined by the ratio of  the aerodynamic damping timescale (or the friction timescale) for the planetesimal ($\tau_{\rm aero, 0}$; Eq.~[\ref{eq:aerodynamic_damping_timescale}]) and the tidal damping timescale (or the migration timescale) of the protoplanet ($\tau_{\mathrm{tide}, a}$). 
A necessary condition for a planetesimal to be captured is that it enters the feeding zone of the protoplanet. 
As for the resonantly trapped planetesimal, $e_{\rm eq}$ must exceed the eccentricity at the feeding zone boundary ($e_{\rm cross}$; Eq.~[\ref{eq:ecc_cross_resonance_feeding_zone}]), which is derived in Sec.~\ref{sec:Condition_for_Aerodynamic_Shepherding}. 
Even if such a condition is satisfied, however, for the trapped planetesimal to escape the resonance completely, the perturbed planetesimal's orbit must oscillate more widely relative to the resonant width (i.e., the overstable libration) and such an oscillation must be amplified more rapidly than the protoplanet's migration.
The conditions are derived in Sec.~\ref{sec:condition_for_resonant_breaking}. 
Finally, by putting everything above together, we infer the condition for the \SSP  \, in Sec.~\ref{sec:condition_for_sweet_spot}.




\subsection{Before resonant trapping}\label{sec:condition_for_resonant_trapping}
When the radial distance between two objects decreases, which is referred to as convergent orbital evolution, the objects are eventually locked in a resonant state.
Such resonant trapping has been discussed in the contexts of the formation of satellite pairs \citep[e.g.,][]{Goldreich1965,Dermott+1988,Malhotra1993b}, the transport of small bodies \citep[e.g.,][]{Yu+2001,Batygin+2015}, and the formation of exoplanet pairs \citep[e.g.,][and references therein]{Fabrycky+2014,Goldreich+2014,Batygin+2015b}. 
%; see also references in \citet{Batygin+2015b}.
However, not all resonant encounters result in resonant trapping. 
The resonant trapping requires the following conditions for a planetesimal-protoplanet pair \cite[e.g.][]{Malhotra1993}:
\begin{itemize}
    \item[(i)] The two orbits converge with each other;
    \item[(ii)] The eccentricity of the planetesimal, $e$, before it is trapped in the resonance is smaller than the critical value $e_{\rm crit}$ (see Eq.~(\ref{eq:critical_eccentricity}));
    \item[(iii)] The timescale for the planetesimal to cross the resonant width $\tau_{\rm cross}$ is longer than the libration timescale $\tau_{\rm lib}$ (see Eqs.~(\ref{eq:crossing_timescale}) and (\ref{eq:1st_order_libration_time_in})).
\end{itemize}
Here, we consider a trap of a planetesimal in the inner first-order mean motion resonances ($j:j-1$ resonance) with a protoplanet migrating inward and assume the mass of the planetesimal is negligibly small relative to %the mass 
that of the protoplanet.

The first condition can be obtained by comparing the timescales of change in the semi-major axis of the planetesimal and the protoplanet.
In a protoplanetary gaseous disk, the orbits of objects shrink by the aerodynamic gas drag and gravitational tidal drag from the disk gas.
The former drag is dominant for planetesimal-size objects ($\lesssim10^{24}\g$) and the latter drag is for planet-size objects ($\gtrsim10^{24}\g$) \citep{Zhou+2007}.
Using the aerodynamic damping timescale for semi-major axis $\tau_{\mathrm{aero},a}$ for the planetesimal and the tidal damping timescale for semi-major axis $\tau_{{\rm tide},a}$ for the protoplanet, we can write the first condition as: 
\begin{align}
    \tau_{{\rm aero},a} > \tau_{{\rm tide},a}. \label{eq:condition_converge_orbits}
\end{align}

As for the second condition, the critical eccentricity for the $j:j-1$ resonances is given by \citep[e.g.][]{Murray+1999}:
\begin{align}
    e_{\rm crit} = \sqrt{6} \left[ \frac{3}{|f_{\rm d}|} \left(j-1\right)^{4/3} j^{2/3} \frac{M_{\rm s}}{M_{\rm p}} \right]^{-1/3}, \label{eq:critical_eccentricity}
\end{align}
where $M_{\rm p}$ and $M_{\rm s}$ are the masses of the planet and central star, respectively, and $f_{\rm d}$ is the interaction coefficient whose values are summarised in Table~\ref{tab:interaction_coefficient}.

When $\tau_{{\rm aero},a} \gg \tau_{{\rm tide},a}$, the timescale for the planetesimal to cross the resonant width $\tau_{\rm cross}$ is given by: 
\begin{align}
    \tau_{\rm cross} = \left| \frac{\Delta a_{\rm res}}{\dot{a}_{\rm c}} \right| = \left| \frac{\Delta a_{\rm res}}{a_{\rm c}} \right| \tau_{{\rm tide},a}, \label{eq:crossing_timescale}
\end{align}
where $a_{\rm c}$ is the semi-major axis of the resonance centre, which is related to the protoplanet's semi-major axis $a_{\rm p}$ as: 
\begin{align}
    a_{\rm c} &= \left(\frac{j-1}{j}\right)^{2/3} a_{\rm p}, \label{eq:resonant_center}
\end{align}
$\dot{a}_{\rm c}$ is the temporal change of $a_{\rm c}$, and $\Delta a_{\rm res}$ is the width of the resonance given by \citep[e.g.][]{Murray+1999}: 
\begin{align}
    \frac{\Delta a_{\rm res}}{a_{\rm c}} &= 2 \left\{ \frac{16}{3} \frac{M_{\rm p}}{M_{\rm s}} \left( \frac{j-1}{j} \right)^{2/3} e \left|f_{\rm d} \right| \right\}^{1/2} \nonumber \\
    & \qquad \left\{ 1+\frac{1}{27 (j-1)^2 e^3} \frac{M_{\rm p}}{M_{\rm s}} \left( \frac{j-1}{j} \right)^{2/3} \left| f_{\rm d} \right| \right\}^{1/2}. \label{eq:1st_order_resonant_width} 
\end{align}
%Note that the resonance centre migrates with the same rate of the protoplanet during the planetary migration phase.
The width of the resonance depends on the eccentricity and takes the minimum value at: 
\begin{align}
    e = \frac{2^{1/3}}{3} \left( \left|j \right|^{-2/3} \left|j-1\right|^{-4/3} \left| f_{\rm d} \right| \frac{M_{\rm p}}{M_{\rm s}} \right)^{1/3}. \label{eq:ecc_at_minimum_resonant_width}
\end{align}
By substituting Eq.~(\ref{eq:ecc_at_minimum_resonant_width}) into Eq.~(\ref{eq:1st_order_resonant_width}), we obtain the minimum width of the resonance as:
\begin{align}
    \left. \frac{\Delta a_{\rm res}}{a_{\rm c}} \right|_{\rm min} = \frac{2^{8/3}}{3^{1/2}} j^{-4/9} (j-1)^{1/9} {|f_{\rm d}|}^{2/3} \left( \frac{M_{\rm p}}{M_{\rm s}} \right)^{2/3}. \label{eq:minimum_resonant_width}
\end{align} 
The libration timescale at internal resonances are given by \citep[e.g.][]{Murray+1999,Batygin+2015}:
\begin{align}
    \tau_{\rm lib}  = \frac{2 \pi}{n} &\left| \left( \frac{j-1}{j} \right)^{4/3} \left( \frac{M_{\rm p}}{M_{\rm s}} \right)^2 \frac{{f_{\rm d}}^2 }{e^2} \right. \nonumber \\
                    & \left.  - 3 (j-1)^2 \left(\frac{j-1}{j} \right)^{2/3} \frac{M_{\rm p}}{M_{\rm s}} f_{\rm d} e \right|^{-1/2}, \label{eq:1st_order_libration_time_in}
\end{align}
where $n$ is the planetesimals' mean motion. 
Substituting Eq.~(\ref{eq:ecc_at_minimum_resonant_width}) into Eq.~(\ref{eq:1st_order_libration_time_in}), we obtain the corresponding libration timescale as: 
\begin{align}
    \tau_{\rm lib} = 0.48 j^{4/9} (j-1)^{-10/9} \left( \frac{M_{\rm p}}{M_{\rm s}} \right)^{-2/3} |f_{\rm d}|^{-2/3} T_{\rm K} \label{eq:corresponding_libration_timescale}.
\end{align}
where $T_{\rm K}$ ($= 2 \pi / n$) is the Kepler period at the resonance centre.
Using Eqs.~(\ref{eq:crossing_timescale}), (\ref{eq:minimum_resonant_width}) and (\ref{eq:corresponding_libration_timescale}), we obtain the third (sufficient) condition as
\begin{align}
    \frac{\tau_{\rm cross}}{\tau_{\rm lib}} = 7.7 j^{1/9} \left(j-1\right)^{2/9} |f_{\rm d}|^{4/3} \left(\frac{M_{\rm p}}{M_{\rm s}}\right)^{4/3} \frac{\tau_{{\rm tide},a}}{T_{\rm K,p}} \gtrsim 1, \label{eq:condition_for_resonant_trapping_mig}
\end{align}
where $T_{\rm K,p}$ is the Kepler period of the migrating protoplanet; namely, $T_{\rm K, p}$ = $T_{\rm K} \, j/(j-1)$.


Far from the protoplanet and outside mean motion resonances, the planetesimal's eccentricity is determined by the balance between the viscous stirring from the planetesimal swarm and the aerodynamic gas drag. 
The mean value of r.m.s. eccentricities of the planetesimal swarm is on the order of $\lesssim10^{-2}$ \citep{Ohtsuki+2002}. %[e.g.][]
For km-sized planetesimals with $e=10^{-2}$, the radial drift timescale $\tau_{{\rm damp},a}$ is longer than the planetary migration timescale in the type II regime ($\tau_{{\rm tide},a}\lesssim10^7~\yr$) over a wide region of a protoplanetary disk \citep{Adachi+1976}. 
Also, the critical eccentricity is $e_{\rm crit}\sim0.15$ for $j=2$ and $M_{\rm p}/M_{\rm s}=10^{-3}$.
Thus, the first and second conditions are expected to be achieved in protoplanetary disks.
Figure~\ref{fig:Timescales_for_resonant_trapping} shows the timescale ratio $\tau_{\rm cross}/\tau_{\rm lib}$ as a function of  semi-major axis, calculated from Eq.~(\ref{eq:condition_for_resonant_trapping_mig}). %Eqs.~(\ref{eq:crossing_timescale}) and (\ref{eq:corresponding_libration_timescale}).
Here, we show the cases of $2:1$ (thick lines) and $3:2$ (thin lines) resonances, and consider the type II regime for the migration timescale $\tau_{{\rm tide},a}$ obtained in \citet{Kanagawa+2018}. 
To calculate $\tau_{{\rm tide},a}$, we adopt the self-similar solution of \citet{Lynden-Bell+1974} for the disk structure with a disk accretion rate of $10^{-8} M_{\odot}/\yr$ and viscosity of $10^{-3}$.
The disk aspect ratio is set to $0.03 r^{1/4}$. 
The timescales ratio $\tau_{\rm cross}/\tau_{\rm lib}$ is larger than unity except for the cases of $M_{\rm p}/M_{\rm s}= 10^{-4}$ in outer disk $a \gg 10 \AU$.
Thus, we conclude that the resonant trapping of planetesimals usually occurs during the migration of a giant protoplanet.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c} \hline
        $p+q:p$ & $f_{\rm s}$ & $f_{\rm d}$  \\ \hline
        2:1     & $0.387627$ & $-1.19049$ \\
        3:2     & $1.15279$  & $-2.02521$ \\
        4:3     & $2.27923$  & $-2.84042$ \\
        5:4     & $3.76541$  & $-3.64962$ \\ \hline
    \end{tabular}
    \caption{Values of the secular term $f_{\rm s}$ and the direct term $f_{\rm d}$ for the first order mean motion resonances.}
    \label{tab:interaction_coefficient}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=90mm]{figure/sweet_spot/axi_TcrossTlib.pdf}
    \caption{
    The ratio between the crossing timescale $\tau_{\rm cross}$ (Eq.~\ref{eq:crossing_timescale}) and the libration timescale $\tau_{\rm lib}$ (Eq.~\ref{eq:corresponding_libration_timescale}) as a function of the planetesimal's semi-major axis. 
    Here, we consider the type II regime obtained in \citet{Kanagawa+2018} for the migration timescale $\tau_{{\rm tide},a}$.
    Solid, dash-dotted, and dotted lines show the cases of the planet-to-star mass ratio $M_{\rm p}/M_{\rm s}=10^{-2}$, $10^{-3}$ and $10^{-4}$, respectively. 
    We consider the inner first-order mean motion resonances (or $j$:$j-1$ resonances); thick lines are for $j=2$ and thin lines are for $j=3$.
    To calculate the migration timescale, we used a disk model same as that in \citet{Ida+2018}. 
    The disk accretion rate, disk's viscosity parameter, and disk aspect ratio are set to $10^{-8} M_{\odot}/\yr$, $10^{-3}$ and $0.03 r^{1/4}$, respectively.
    }
    \label{fig:Timescales_for_resonant_trapping}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Orbital evolution under resonant trapping}\label{sec:orbital_evolution_in_resonant_trapping}
Trapped planetesimals suffer from gravitational perturbation from the migrating protoplanet and aerodynamic gas drag from the disk gas. 
The Lagrange's equations under the aerodynamic gas drag are given by \citep[e.g.,][]{Murray+1999}:
\begin{align}
    \dot{a} &= 2 (j-1) C_{\rm r} a e   \sin \varphi -\frac{a}{\tau_{{\rm aero},a}}, \label{eq:Lagrange_axi_wGas} \\
    \dot{e} &=       - C_{\rm r}       \sin \varphi -\frac{e}{\tau_{{\rm aero},e}}, \label{eq:Lagrange_ecc_wGas}
\end{align}
where $\varphi$ is the resonant angle and
\begin{align}
    C_{\rm r} =  \frac{M_{\rm p}}{M_{\rm s}} n \alpha f_{\rm d};  \label{eq:coefficient_resonance}
\end{align} 
$\tau_{{\rm aero},a}$ and $\tau_{{\rm aero},e}$ are the aerodynamic damping timescales for semi-major axis and eccentricity, which are given by \citep{Adachi+1976}:
\begin{align}
    \tau_{{\rm aero},a} &= \frac{\tau_{\rm aero,0}}{2} \left\{ (0.97 e +0.64 i +   |\eta_{\rm gas}|)\eta_{\rm gas}  \right\}^{-1}, \label{eq:aerodynamic_damping_axi} \\
    \tau_{{\rm aero},e} &=       \tau_{\rm aero,0}     \left(   0.77 e +0.64 i +1.5|\eta_{\rm gas}| \right)^{-1}, \label{eq:aerodynamic_damping_ecc}
\end{align}
where 
\begin{align}
    \tau_{\rm aero,0} = \frac{2 m_{\rm pl}}{C_{\rm d} \pi {R_{\rm pl}}^2 \rho_{\rm gas} v_{\rm K}}. \label{eq:aerodynamic_damping_timescale}
\end{align}
Here $C_{\rm d}$ is the non-dimensional drag coefficient, 
$m_{\rm pl}$ is the planetesimal's mass, 
$R_{\rm pl}$ is the planetesimal's radius, 
$\rho_{\rm gas}$ is the gas density, and 
$v_{\rm K}$ is the Kepler velocity.
The planetesimal's mass $m_{\rm pl}$ is calculated as $4\pi\rho_{\rm pl}{R_{\rm pl}}^3/3$, where $\rho_{\rm pl}$ is the planetesimal's mean density.% and given as $\rho_{\rm pl}=2 \g/\cm^3$.
$\eta_{\rm gas}$ is a parameter that defines the sub-Keplerian velocity of disk gas as: 
\begin{align}\label{eq:Disk_Gas_Velocity_sub-Kepler}
	v_{\rm gas} = v_{\rm K} \left( 1- \eta_{\rm gas} \right).
\end{align}
Note that we have neglected the high-order terms in eccentricity in Eqs.~(\ref{eq:Lagrange_axi_wGas}), (\ref{eq:Lagrange_ecc_wGas}), (\ref{eq:aerodynamic_damping_axi}) and (\ref{eq:aerodynamic_damping_ecc}).
Although the eccentricities of the trapped planetesimals are easily excited to $e^2 \sim 0.1$, the location of the sweet spot analytically derived with these equations is found to be  consistent with the numerical results, as shown in section~\ref{sec:sweet_spot_numerical}.

During the resonant trapping, the period ratio between the protoplanet and trapped planetesimal remains constant, by definition, and
%to be
%\begin{align}
%    \frac{j-1}{j} &= \frac{n_{\rm p}}{n} = \left( \frac{a}{a_{\rm p}} \right)^{3/2} = \text{const.}, \label{eq:Period_Ratio_in_Resonances}
%\end{align}
%where $n_{\rm p}$ is the planet's mean motion.
%Taking a time derivative of eq.~(\ref{eq:Period_Ratio_in_Resonances}), we find
\begin{align}
    \frac{a}{\dot{a}} = \frac{a_{\rm p}}{\dot{a_{\rm p}}} = -\tau_{{\rm tide},a}. \label{eq:Timescles_in_resonant_trapping}
\end{align}
%Using eqs.~(\ref{eq:Lagrange_axi_wGas}), (\ref{eq:Lagrange_ecc_wGas}), (\ref{eq:Timescles_in_resonant_trapping}) and $\tau_{{\rm damp},a}~\gg~\tau_{{\rm tide},a}$, we obtain
%\begin{align}
%    \dot{e}     &=  \frac{1}{2(j-1)e \tau_{{\rm tide},a}} -\frac{e}{\tau_{{\rm damp},e}}, \label{eq:Solution_Lagrange_ecc} \\
%    \sin \varphi   &= -\frac{1}{2(j-1) C_{\rm r} e \tau_{{\rm tide},a}}. \label{eq:Solution_Lagrange_phi}
%\end{align}
When $\tau_{{\rm aero},a} \gg \tau_{{\rm tide},a}$, using Eq.~(\ref{eq:Timescles_in_resonant_trapping}), we can re-write  Eq.~(\ref{eq:Lagrange_axi_wGas}) as: 
\begin{align}
    \sin \varphi   &= -\frac{1}{2(j-1) C_{\rm r} e \tau_{{\rm tide},a}}. \label{eq:Solution_Lagrange_phi}
\end{align}
Also, using Eq.~(\ref{eq:Solution_Lagrange_phi}) in Eq.~(\ref{eq:Lagrange_ecc_wGas}), we obtain: 
\begin{align}
    \dot{e}     &=  \frac{1}{2(j-1)e \tau_{{\rm tide},a}} -\frac{e}{\tau_{{\rm aero},e}}. \label{eq:Solution_Lagrange_ecc} 
\end{align}
Just after trapped into the resonances, $e$ is small and $\dot{e}$ is positive.
Equation~(\ref{eq:Solution_Lagrange_ecc}) indicates that $e$ increases on a timescale $\sim~e^2~\tau_{{\rm tide},a}~(\ll~\tau_{{\rm tide},a})$ and reaches an equilibrium value.
Solving Eqs.~(\ref{eq:Solution_Lagrange_phi}) and (\ref{eq:Solution_Lagrange_ecc}) with $\dot{e}=0$, we obtain the equilibrium eccentricity and resonant argument given by: 
\begin{align}
    e_{\rm eq}          &= \left\{ \frac{1}{2(j-1)} \frac{\tau_{{\rm aero},e}}{\tau_{{\rm tide},a}} \right\}^{1/2}, \label{eq:equilibrium_eccentricity} \\
    \sin \varphi_{\rm eq}  &= - \frac{e_{\rm eq}}{C_{\rm r} \tau_{{\rm aero},e}}. \label{eq:equilibrium_resonant_argument}
\end{align}
Unlike the eccentricity, the planetesimals' inclinations are not excited by the migrating protoplanet because the planetesimals are far from the protoplanet.
When $e \gg i$ and $e \gg \eta_{\rm gas}$, $\tau_{\mathrm{aero},e} = \tau_{\rm aero,0} (0.77 e)^{-1}$ from Eq.~(\ref{eq:aerodynamic_damping_ecc}) and, thus, $e_{\rm eq}$ and $\sin \varphi_{\rm eq}$ are written approximately as: 
\begin{align}
    e_{\rm eq}          &\sim \left\{ \frac{1}{1.54 (j-1)} \frac{\tau_{\rm aero,0}}{\tau_{{\rm tide},a}} \right\}^{1/3}, \label{eq:equilibrium_eccentricity_app} \\
    \sin \varphi_{\rm eq}  &\sim -\frac{0.77{e_{\rm eq}}^2}{C_{\rm r} \tau_{\rm aero,0}}. \label{eq:equilibrium_resonant_argument_app}
\end{align}
Note that if the high-order terms of the  eccentricity are considered, the equilibrium eccentricity is smaller than that given by Eq.~(\ref{eq:equilibrium_eccentricity_app}). % for $e\gtrsim0.3$.

\subsection{Aerodynamic shepherding}\label{sec:Condition_for_Aerodynamic_Shepherding}
As shown in \citet{Shibata+2020}, the mean motion resonances play a role like narrow flow channels for planetesimals to enter the planet's feeding zone; the channels are called the {\it accretion bands}. 
Mathematically speaking, planetesimals with negative values of the Jacobi energy, $E_{\rm Jacobi}$, can enter the feeding zone, once their eccentricities are sufficiently enhanced so that their Jacobi energy becomes positive.
The Jacobi energy is given by \citep{Hayashi+1977}: 
\begin{align}\label{eq:Ejacobi}
    E_{\rm Jacobi} = \frac{\mathcal{G} M_{\rm s}}{a_{\rm p}} \left\{ -\frac{a_{\rm p}}{2 a} - \sqrt{\frac{a}{a_{\rm p}} \left(1-e^2\right)} \cos {i} + \frac{3}{2} + \frac{9}{2} h^2 +O(h^3) \right\},
\end{align}
where $h$ is the reduced Hill radius defined as 
\begin{align}\label{eq:reduced_Hill_radius}
    h = \left( \frac{M_{\rm p}}{3 M_{\rm s}} \right)^{1/3}.
\end{align}
Substituting $E_{\rm jacobi}=0$ and $a/a_{\rm p} = \left\{(j-1)/j\right\}^{2/3}$ into Eq.~(\ref{eq:Ejacobi}) and assuming $\cos^2 i \sim 1$, one obtains the eccentricity of the accretion band, $e_{\rm cross}$, as: 
\begin{align}
    e_{\rm cross} = \left[ 1- \left( \frac{j}{j-1} \right)^{2/3} \left\{ \frac{3}{2} +\frac{9}{2} h^2 -\frac{1}{2} \left( \frac{j}{j-1} \right)^{2/3} \right\}^2 \right]^{1/2}. \label{eq:ecc_cross_resonance_feeding_zone}
\end{align}
The condition required for entering the feeding zone is that the equilibrium eccentricity $e_{\rm eq}$ (see Eq.~\ref{eq:equilibrium_eccentricity_app}) is larger than $e_{\rm cross}$, which is given by: 
\begin{align}
    1.54 (j-1) {e_{\rm cross}}^3 &< \frac{\tau_{\rm aero,0}}{\tau_{{\rm tide},a}}. \label{eq:condition_for_aerodynamic_shepherding}
\end{align}
Figure~\ref{fig:Mp_EccCross} shows $e_{\rm cross}$ as a function of $M_{\rm p}/M_{\rm s}$ for different values of $j$ from Eq.~(\ref{eq:ecc_cross_resonance_feeding_zone}).
As indicated in this figure, $e_{\rm cross}$ decreases with increasing planetary mass. 
This is because as the protoplanet mass increases, the feeding zone expands and, consequently, the crossing point (i.e., the accretion band) itself is located inside the feeding zone, once the planetary mass exceeds a certain value.
For example, while there are three crossing points $(j=2,3,4)$ when $M_{\rm p}/M_{\rm s}=10^{-3.5}$, there is only one crossing point $(j=2)$ when $M_{\rm p}/M_{\rm s}=10^{-2.5}$ and no points when $M_{\rm p}/M_{\rm s}=10^{-2}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{figure/sweet_spot/mu_ecross.pdf}
    \caption{
    The dependence of the crossing point eccentricity $e_{\rm cross}$ (see Eq.~\ref{eq:ecc_cross_resonance_feeding_zone}) on the planet-to-star mass ratio $M_{\rm p}/M_{\rm s}$ for different four cases of $j=2$ (solid), $j=3$ (dashed), $j=4$ (dash-dotted) and $j=5$ (dotted), respectively.
    }
    \label{fig:Mp_EccCross}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Resonant breaking}\label{sec:condition_for_resonant_breaking}
Even when entering the feeding zone, planetesimals trapped in the mean motion resonances are not  always accreted by the migrating protoplanet.
The conjunction point of a trapped planetesimal with the protoplanet is given in terms of the mean longitude as: 
\begin{align}
     \lambda_{\rm con} = \varphi + \varpi,
\end{align}
where $\varpi$ is the longitude of pericenter. 
The resonant argument, $\varphi$, which is the displacement of the longitude of conjunction from the pericenter, takes $\varphi_{\rm eq} \sim 0$ during the converging orbital evolution.
This means that every conjunction occurs at the pericenter of the planetesimal orbit; namely, the planetesimal's orbit is far from the protoplanet's one at the conjunction.
Thus, trapped planetesimals cannot enter the Hill sphere of the protoplanet and planetesimal accretion does not occur \citep[see Figs.~C.1 and C.2 in][]{Shibata+2020}.

A planetesimal is captured by the migrating protoplanet only if the resonant trapping is  broken.
Under the forces damping and enhancing the planetesimal's eccentricity, the orbit of the trapped planetesimal becomes unstable and starts to oscillate.
Once the amplitude of oscillation exceeds the resonant width, the resonant trapping is broken.
This phenomenon is called the \textit{overstable libration} and \citet{Goldreich+2014} is derived the condition required for the instability to grow.
Substituting Eqs.~(\ref{eq:aerodynamic_damping_ecc}) and (\ref{eq:equilibrium_eccentricity_app}) into Eq.~(28) of \citet{Goldreich+2014}, we obtain the breaking condition for resonant trapping due to overstable libration under the aerodynamic gas drag as: 
\begin{align}
    3.29 \left(\frac{j}{j-1}\right)^{3/2} \frac{M_{\rm p}}{M_{\rm s}} < \frac{\tau_{\rm aero,0}}{\tau_{{\rm tide},a}}. \label{eq:overstable_libration_due_to_gasdrag}
\end{align}
Even once this condition is satisfied, it takes a time of $\sim\tau_{{\rm aero},e}$ for the instability to grow \citep{Goldreich+2014}.
If $\tau_{{\rm aero},e}~>~\tau_{{\rm tide},a}$, the trapped planetesimal is shepherded into the inner disk before escaping the resonance.
The second condition required for the overstable libration is $\tau_{{\rm aero},e}~<~\tau_{{\rm tide},a}$, which one can write as: 
\begin{align}
    \frac{\tau_{\rm aero,0}}{\tau_{{\rm tide},a}} < 0.54 (j-1)^{-1/2}, \label{eq:condition_for_resonant_breaking_grow}
\end{align}
using Eqs.~(\ref{eq:aerodynamic_damping_ecc}) and (\ref{eq:equilibrium_eccentricity_app}).



\subsection{Required condition for the Accretion Sweet Spot}\label{sec:condition_for_sweet_spot}
The required condition for the \SSP\ is summarised as: 
\begin{align}
    {\rm max} \left. 
        \begin{cases}
            1.54 (j-1) {e_{\rm cross}}^3\\
            \displaystyle{            
                3.29 \left(\frac{j}{j-1}\right)^{3/2} \frac{M_{\rm p}}{M_{\rm s}}
            }
        \end{cases}
    \right\}
    < \frac{\tau_{\rm aero,0}}{\tau_{{\rm tide},a}} < 0.54 (j-1)^{-1/2} \label{eq:sweet_spot}.
\end{align}
The inner edge of the \SSP\ is regulated by the aerodynamic shepherding and resonant shepherding.
The dominating  process depends on the planetary mass.
On the other hand, the outer edge of \SSP\ is regulated by the resonant shepherding only. 

To derive above equations, we assume that $\tau_{\mathrm{aero},a}\gg\tau_{\mathrm{tide},a}$.
Using the equilibrium eccentricity, we transform this condition as
\begin{align}
    \frac{2.18 {\eta_{\rm gas}}^{3/2}}{\sqrt{j-1}} \ll \frac{\tau_{\mathrm{aero},0}}{\tau_{\mathrm{tide},a}}.
\end{align}
In the nominal disk model, $\eta_{\rm gas}$ is the order of $10^{-3}$ and this condition is easily achieved in the SSP.
Thus, the eqs.~(\ref{eq:sweet_spot}) can be used for small planetesimals as long as the gas drag strength is scaled by eq.~(\ref{eq:aerodynamic_damping_timescale}).
We find that the location of the \SSP\ is determined by the ratio of the gas drag damping timescale $\tau_{\rm aero,0}$ and the planetary migration timescale $\tau_{{\rm tide},a}$.
We therefore conclude that our theoretical prediction is robust (and rather general) since 
the derivation of this condition does not depend on the assumed disk and migration models.  
As a result, Eq.~(\ref{eq:sweet_spot}) can be generally applied to various models of planetesimal accretion. 



==> Shibata et. al. 2021/text/sweet_spot_numerical.tex <==
In this section we validate the derived equation for the \SSP\ by comparison with numerical results.
To that end, we perform $N$-body simulations similar to those presented in \citet{Shibata+2020}.
We adopt different values of model parameters from those in \citet{Shibata+2020} in order to identify whether the \SSP\ is indeed regulated by the ratio of the two timescales, $\tau_{\rm aero,0}$ and $\tau_{{\rm tide},a}$.
%Note that we changed the disk model from the viscous evolving disk to the minimum mass solar nebulae \citep{Hayashi1981} for simplifying the simulation. 
%An overview of the model is given in Appendix~\ref{sec:app_model}.

\subsection{Numerical Model and Settings}\label{sec:model_settings}
We consider the following scenario: 
Gas accretion has terminated and the young giant planet no longer grows in mass. 
The planet then migrates radially inward from a given semi-major axis within a protoplanetary disk. 
Initially there are many single-sized planetesimals interior to the planet's orbit.  
The migrating planet then encounters these planetesimals and captures some of them. 
The planetesimals are represented by test particles and, therefore, are affected only by the gravitational forces from the central star and planet, and the drag force by the disk gas.
Here, we summarise our numerical model.
The details of our numerical model are described in Appendix~\ref{app:method}.

We assume that the planetary migration timescale is given by:  
\begin{align}
    \tau_{{\rm tide},a} &= \tau_{\rm tide,0} \left( \frac{a_{\rm p}}{1 \AU} \right)^{1/2}, \label{eq:type2_migration_timescale}
\end{align}
where $\tau_{\rm tide,0}$ is a scaling parameter.
For the drag force by the disk gas, we adapt a model by \citet{Adachi+1976}.
The gas drag force depends on the size of planetesimal $R_{\rm pl}$ and the profile of ambient disk gas.
To focus on the dynamic process, we adopt simply the minimum-mass solar nebula model \citep{Hayashi1981} as our gas disk model.
The surface density $\Sigma_{\rm gas}$ and the disk' temperature $T_{\rm disk}$ are given by: 
\begin{align}
    \Sigma_{\rm gas} &= \Sigma_{\rm gas,0} \left( \frac{r}{1\AU} \right)^{-\alpha_{\rm disk}}, \label{eq:Disk_Gas_MMSN} \\
    T_{\rm disk} &= T_{\rm disk,0} \left(\frac{r}{1\AU} \right)^{-2\beta_{\rm disk}}, \label{eq:Disk_Temperature_MMSN}
\end{align}
where $r$ is the radial distance from the initial mass centre of the star-planet system, $\Sigma_{\rm gas,0} = 1.7 \times 10^3 \g/\cm^2$, $\alpha_{\rm disk}=3/2$, $T_{\rm disk,0}=280~\K$ and $\beta_{\rm disk}=1/4$.
%The surface density $\Sigma_{\rm gas}$ is given by: 
%\begin{align}\label{eq:Disk_Gas_MMSN}
%    \Sigma_{\rm gas} = \Sigma_{\rm gas,0} \left( \frac{r}{1\AU} \right)^{-\alpha_{\rm disk}},
%\end{align}
%where $r$ is the radial distance from the initial mass centre of the star-planet system, $\Sigma_{\rm gas,0} = 1.7 \times 10^3 \g/\cm^2$ and $\alpha_{\rm disk}=3/2$.
%The disk' temperature $T_{\rm disk}$ is given by: 
%\begin{align}
%    T_{\rm disk} = T_{\rm disk,0} \left(\frac{r}{1\AU} \right)^{-2\beta_{\rm disk}},
%\end{align}
%where $T_{\rm disk,0}=280~\K$ and $\beta_{\rm disk}=1/4$.
The protoplanetary disk is assumed to be vertically isothermal.

For the planetesimals we adopt a simple surface density profile given by:
\begin{align}
    \Sigma_{\rm solid} = Z_{\rm s} \Sigma_{\rm gas,0} \left( \frac{r}{1\AU} \right)^{-\alpha_{\rm disk}^{\prime}}, \label{eq:Model_Disk_Solid_Surface_Density}
\end{align}
where $Z_{\rm s}$ is the solid-to-gas ratio (or the metallicity) and $\alpha_{\rm disk}^{\prime}=\alpha_{\rm disk}=3/2$.
%We assume that $Z_{\rm s}$ equals the metallicity of the central star.
To speed up the numerical integration, we follow the orbital motion of super-particles, each of which contains several equal-size planetesimals.
The super-particles are initially distributed in $a_{\rm pl,in}< r < a_{\rm pl,out}$ with $a_{\rm pl,in}=0.3\AU$ and $a_{\rm pl,out}=20~\AU$.
%The number of super-particles $N_{\rm sp}$ is $12 000$.
The planet is initially located in such a way that the inner boundary of the feeding zone is consistent with the outer edge of the planetesimals disk, namely: 
\begin{align}
    a_{\rm p,0} = \frac{a_{\rm pl,out}}{1-2\sqrt{3} h}. \label{eq:part1_initial_semimajoraxis_planet}
\end{align}

The calculation is artificially stopped once the planet reaches the orbit of $a_{\rm p,f}=0.5 \AU$.
First, we investigate the planetesimal accretion in a reference case, where $\tau_{{\rm tide},0}= 1 \times 10^5~\yr$, $R_{\rm pl}= 1 \times 10^7~\cm$ and $M_{\rm p} = 1 \times 10^{-3}M_{\rm s}$.
In the reference case, the total amount of planetesimals are $M_{\rm tot} \sim 43 \Mear$.
The choices of the parameter values for the reference model are summarised in Table~\ref{tb:settings}.
We perform a parameter study for various values of $\tau_{\rm tide,0}$, $R_{\rm pl}$, and $M_{\rm p}$.
The dynamical integration for the planetesimals is performed using the numerical simulation code developed by \citet{Shibata+2019}.
In this code, we integrate the equation of motion using the forth-order-Hermite integration scheme \citep{Makino+1992}.
For the timesteps, we adopt the method of \citet{Aarseth1985}.

\begin{comment}
\subsubsection{Equations of motion}\label{sec:app_eom}
The equation of motion is given by: 
\begin{align}
   \frac{{\rm d} {\bf r}_i }{{\rm d} t} &= \sum_{i\neq j} {\bf f}_{{\rm grav},i,j} + {\bf f}_{\rm aero} +{\bf f}_{\rm tide}, \label{eq:EoM}
\end{align}
where ${\bf r}_i$ is the position vector relative to the initial (i.e., $t = 0$) mass centre of the star-planet-planetesimals system, %$t$ is the time, 
${\bf f}_{{\rm grav},i,j}$ is the mutual gravity between particles $i$ and $j$ given by: 
\begin{align}
   {\bf f}_{{\rm grav},i,j} &= - \mathcal{G} \frac{M_j}{{r_{i,j}}^3} {\bf r}_{i,j} \label{eq:EoM_gravity}
\end{align}
with $\mathbf{r}_{i,j}$ being the position vector of particle $i$ relative to particle $j$ ($r_{i,j} \equiv |{\bf r}_{i,j}|$),
$M_{j}$ is the mass of particle $j$, and $\mathcal{G}$ is the gravitational constant. 
${\bf f}_{\rm aero}$ is the aerodynamic gas drag, and ${\bf f}_{\rm tide}$ is the gravitational tidal drag from the protoplanetary disk gas. 
The central star, planet, and planetesimals  are denoted by the subscripts $i$ (or $j$) = 1, 2, and $\geq$~3, respectively.
The planetesimals are treated as test particles; therefore $f_{{\rm grav},i,j}=0$ in Eq.~(\ref{eq:EoM}) for $j \geq~3$.
We assume that the aerodynamic gas drag force and the tidal drag force are given respectively by:  
\begin{align}
  {\bf f}_{\rm aero} &= -\frac{{\bf u}}{\tau_{\rm aero}}, \label{eq:EoM_reduced_gas_drag} \\
  {\bf f}_{\rm tide} &= - \frac{{\bf v}_{\rm p}}{2 \tau_{{\rm tide},a}},
\end{align}
with
\begin{align}
    \tau_{\rm aero} &=  \frac{2 m_{\rm pl}}{ C_{\rm d} \pi R_{\rm pl}^2 \rho_{\rm gas} u} = \tau_{\rm aero, 0} \frac{v_{\rm K}}{u} \\
    \tau_{{\rm tide},a} &= \tau_{\rm tide,0} \left( \frac{a_{\rm p}}{1 \AU} \right)^{1/2}. \label{eq:type2_migration_timescale}
\end{align}
Here ${\bf u}={\bf v}_{\rm pl}-{\bf v}_{\rm gas}$ ($u = |{\bf u}|$) is the planetesimal's  velocity (${\bf v}_{\rm pl}$) relative to the ambient gas (${\bf v}_{\rm gas}$), %$\tau_{\rm aero}$ is the timescale of aerodynamic gas drag, 
$m_{\rm pl}$ is the planetesimal's mass, 
$C_{\rm d}$ is the non-dimensional drag coefficient and given as $C_{\rm d}=1$, 
$\rho_{\rm gas}$ is the gas density,
$R_{\rm pl}$ is the planetesimal's radius,
${\bf v}_{\rm p}$ is the planet's velocity,
$a_{\rm p}$ is the planet's semi-major axis,
and $\tau_{\rm tide,0}$ is a scaling parameter.
The velocity and density of the ambient disk gas are calculated from the protoplanetary disk model.
Given the range of the planetesimal mass ($\sim10^{16}$-$10^{22} \g$) and planet ($\sim10^{30} \g$), we assume $f_{\rm tide}=0$ for the former and $f_{\rm aero}=0$ for the latter.
The central star is not affected by $f_{\rm aero}$ and $f_{\rm tide}$.

\subsubsection{Gas disk}\label{sec:app_disk}
To focus on the dynamic process, we adopt simply the minimum-mass solar nebula model \citep{Hayashi1981} as our gas disk model. 
We assume that the disk has an axisymmetric, temporally unchanged structure and disregard the difference between the locations between the symmetry axis and the mass centre of the star-planet system.
We also neglect the disk's self-gravity  %meaning no gravitational interaction but 
but include the tidal drag  between the disk and planet.
The surface density $\Sigma_{\rm gas}$ is given by: 
\begin{align}\label{eq:Disk_Gas_MMSN}
    \Sigma_{\rm gas} = \Sigma_{\rm gas,0} \left( \frac{r}{1\AU} \right)^{-\alpha_{\rm disk}},
\end{align}
where $r$ is the radial distance from the initial mass centre of the star-planet system, $\Sigma_{\rm gas,0} = 1.7 \times 10^3 \g/\cm^2$ and $\alpha_{\rm disk}=3/2$.
The disk' temperature $T_{\rm disk}$ is given by: 
\begin{align}
    T_{\rm disk} = T_{\rm disk,0} \left(\frac{r}{1\AU} \right)^{-2\beta_{\rm disk}},
\end{align}
where $T_{\rm disk,0}=280~\K$ and $\beta_{\rm disk}=1/4$.
The protoplanetary disk is assumed to be vertically isothermal, and the gas density $\rho_{\rm gas}$ is expressed as: 
\begin{align}\label{eq:Disk_Gas_volume}
   \rho_{\rm gas} = \frac{\Sigma_{\rm gas}}{\sqrt{2 \pi} h_{\rm s}} \exp \left( -\frac{z^2}{2 {h_{\rm s}}^2} \right),
\end{align}
where $z$ is the height from the disk mid-plane and $h_{\rm s}$ is the disk's scale height.
The aspect ratio of the protoplanetary disk is given by:  
\begin{align}
    \frac{h_{\rm s}}{r} = \frac{c_{\rm s}}{r\Omega_{\rm K}},
\end{align}
where $\Omega_{\rm K}$ is the Kepler angular velocity and $c_{\rm s}$ is the isothermal sound speed of disk gas.
The sound speed is given as %Assuming locally isothermal case, 
\begin{align}
    c_{\rm s} = \sqrt{\frac{k_{\rm B} T_{\rm disk}}{\mu_{\rm disk} m_{\rm H}}} \propto r^{-\beta{\rm disk}},
\end{align}
where $k_{\rm B}$ is the Boltzmann constant and $\mu_{\rm disk}$ is the mean molecular weight in the unit of proton mass $m_{\rm H}$.
In this study, $\mu_{\rm disk}$ is set as $2.3$ and the aspect ratio of the disk gas at $1\AU$ is $\sim0.03$.

The gas in the protoplanetary disk rotates with a sub-Keplerian velocity because of pressure gradient; namely, $v_{\rm gas} = (1-\eta_{\rm gas}) r \Omega_{\rm K}$, where $\eta_{\rm gas}$ is $\ll 1$ and given as
\begin{align}
	\eta_{\rm gas} &\equiv	\mathbf{-} \frac{1}{2} \left( \frac{h_{\rm s}}{r} \right)^2 \frac{{\rm d} \ln P_{\rm gas}}{{\rm d} \ln r}, \label{eq:eta_gas_definition} \\ 
	               &=		\frac{1}{2} \left( \frac{h_{\rm s}}{r} \right)^2 
	                        \left[ \frac{3}{2} \left( 1 - \frac{z^2}{{h_{\rm s}}^2} \right) +\alpha_{\rm disk} +\beta_{\rm disk} \left(1+\frac{z^2}{{h_{\rm s}}^2}  \right) \right];
\end{align}
$P_{\rm gas}$ is the gas pressure.
%For deriving the above equation, we assume $\eta_{\rm gas} \ll 1$ and use the ideal-gas relation for isothermal sound speed, i.e., $c_{\rm s}^2$ = $P_{\rm gas} / \rho_{\rm gas}$.

\subsubsection{Planetesimals}
For the planetesimals we adopt a simple surface density profile given by: %$\Sigma_{\rm solid}$, which is expressed as
\begin{align}
    \Sigma_{\rm solid} = \Sigma_{\rm solid,0} \left( \frac{r}{1\AU} \right)^{-\alpha_{\rm disk}^{\prime}}, \label{eq:Model_Disk_Solid_Surface_Density}
\end{align}
and set $\alpha_{\rm disk}^{\prime}=\alpha_{\rm disk}=3/2$ and 
\begin{align}
    \Sigma_{\rm solid,0} = Z_{\rm s} \Sigma_{\rm gas,0},    
\end{align}
where $Z_{\rm s}$ is the solid-to-gas ratio (or the metallicity).
We assume that $Z_{\rm s}$ equals the metallicity of the central star.
The planetesimal's mass $m_{\rm pl}$ is calculated as $4\pi\rho_{\rm pl}{R_{\rm pl}}^3/3$, where $\rho_{\rm pl}$ is the planetesimal's mean density and given as $\rho_{\rm pl}=2 \g/\cm^3$.
The surface number density of planetesimals is given as $\Sigma_{\rm solid}/m_{\rm pl}$ which gives $\sim10^6~/\AU^2$ at maximum.

To speed up the numerical integration, we follow the orbital motion of super-particles, each of which contains several equal-size planetesimals.
The super-particles are distributed in a given radial region, the inner and outer radii of which are denoted by $a_{\rm pl,in}$ and $a_{\rm pl,out}$, respectively. 
The surface number density of super-particles $n_{\rm s}$ is given as: 
\begin{align}
    n_{\rm s} = n_{\rm s,0} \left( \frac{r}{1 \AU} \right)^{-\alpha_{\rm sp}}
\end{align}
where
\begin{align}
    n_{\rm s,0} = \frac{N_{\rm sp}}{2 \pi} \frac{2 -\alpha_{\rm sp}}
                  {\left(a_{\rm pl,out}/1\AU\right)^{2-\alpha_{\rm sp}} -\left(a_{\rm pl,in}/1\AU\right)^{2-\alpha_{\rm sp}} } \left[\frac{1}{\AU^2}\right];
\end{align}
$N_{\rm sp}$ is the total number of super-particles used in a given simulation.
In our simulation, we set $N_{\rm sp}=12,000$ and $\alpha_{\rm sp}=1$ to distribute super-particles uniformly in the radial direction.
The mass per super-particle $M_{\rm sp}$ is given by: 
\begin{align}
    M_{\rm sp} (a_{\rm 0}) = \frac{\Sigma_{\rm solid} (a_{\rm 0})}{n_{\rm s} (a_{\rm 0})} ,
\end{align}
where $a_{\rm 0}$ is the initial semi-major axis of the super-particle.

As for eccentricity and inclination, although planetesimals are treated as test particles in our simulations, assuming that planetesimals are, in reality, scattered by their mutual gravitational interaction, we adopt the Rayleigh distribution as the initial eccentricities $e$ and inclinations $i$ of planetesimals.
We set $\left< e^2 \right>^{1/2}=2\left< i^2 \right>^{1/2}=10^{-3}$.
The orbital angles (longitude of ascending node $\Omega$, longitude of pericentre $\varpi$ and mean longitude at epoch $\epsilon$) are distributed uniformly.

During the orbital integration, we judge that a super-particle has been captured by the planet once (i) the super-particle enters the planet's envelope or (ii) its Jacobi energy becomes negative in the Hill sphere.
The planet's radius $R_{\rm p}$ is calculated as: 
\begin{align}\label{eq:Rplanet_cap}
    R_{\rm p} = \left( \frac{3 M_{\rm p}}{4 \pi \rho_{\rm p}} \right)^{1/3},
\end{align}
where $\rho_{\rm p}$ is the planet's mean density.
The planet's radius is assumed to be  extended shortly after formation and the density is set to  $\rho_{\rm p}=0.125~\g~\cm^{-3}$, corresponding to a planet's radius twice as large as Jupiter's current radius. 

\subsubsection{Model settings}\label{sec:app_settings}
The planetesimals are initially distributed in $a_{\rm pl,in}< r < a_{\rm pl,out}$ and $a_{\rm pl,in}$ is fixed at $0.3 \AU$ in our simulation.
The planet is initially located in such a way that the inner boundary of the feeding zone is consistent with the outer edge of the planetesimals disk, namely: 
\begin{align}
    a_{\rm p,0} = \frac{a_{\rm pl,out}}{1-2\sqrt{3} h}. \label{eq:part1_initial_semimajoraxis_planet}
\end{align}
The calculation is artificially stopped once the planet reaches the orbit of $a_{\rm p,f}=0.5 \AU$.
First, we investigate the planetesimal accretion in a reference case, where $\tau_{{\rm tide},0}= 1 \times 10^5~\yr$, $R_{\rm pl}= 1 \times 10^7~\cm$, $a_{\rm pl,out}=20~\AU$ and $M_{\rm p} = 1 \times 10^{-3}M_{\rm s}$.
In the reference case, the total amount of planetesimals are $M_{\rm tot} \sim 43 \Mear$.
The choices of the parameter values for the reference model are summarised in Table~\ref{tb:settings}.
We perform a parameter study for various  values of  $\tau_{\rm tide,0}$, $R_{\rm pl}$, and $M_{\rm p}$.
\end{comment}


\begin{table*}
	\centering
	\begin{tabular}{ llllll } % four columns, alignment for each
		%\hline
		%Parameters used in the model &&&&&\\
		\hline
		$M_{\rm s}$             & Mass of central star	                        & $1.0$				                & $\Msun$ 	\\
		$Z_{\rm s}$             & Metallicity of central star	                & $0.018$				            & - \\
		$M_{\rm p}$             & Mass of planet		                        & $1.0$		                        & $\Mjup$  \\
%		$R_{\rm p}$             & Radius of planet		                        & eq.~(\ref{eq:Rplanet_cap})        & \\
%		$\rho_{\rm p}$          & Mean density of planet                        & $0.125$                           & $\g~\cm^{-3}$ \\
        $a_{\rm p,0}$           & Initial semi-major axis of planet             & eq.~(\ref{eq:part1_initial_semimajoraxis_planet})  & \\
        $a_{\rm p,f}$           & Final semi-major axis of planet               & $0.5$                             & $\AU$ \\
		$\tau_{\rm tide,0}$     & Scaling factor of migration timescale	        & $1.0 \times 10^5$                 & $\yr$ \\
        $\Sigma_{\rm disk,0}$   & Surface density of disk gas at $1\AU$         & $1.7\times10^{3}$		            & $\g/\cm^2$  \\
        $T_{\rm disk,0}$        & Temperature at $1\AU$                         & $280$		                        & $\K$  \\
        $\alpha_{\rm disk}$     & Exponent of disk gas profile                  & $3/2$                             & - \\
        $\beta_{\rm disk}$      & Exponent of disk temperature profile          & $1/4$                             & - \\
        $R_{\rm pl}$            & Radius of planetesimal			            & $1.0 \times 10^7$	                & $\cm$		    \\
        $a_{\rm pl,in}$         & Inner edge of planetesimal disk	            & $0.3$	                            & $\AU$		    \\
        $a_{\rm pl,out}$        & Outer edge of planetesimal disk	            & $20$	                            & $\AU$		    \\
%        $\alpha_{\rm sp}$       & Exponent of test particle distribution        & $1$                               & - \\
		$\rho_{\rm pl}$         & Mean density of planetesimal			        & $2.0$	                            & $\g~\cm^{-3}$		    \\
		$N_{\rm sp}$            & Initial number of super-particles             & 12 000                            & - \\
		$C_{\rm d}$             & Non-dimensional drag coefficient              & 1                                 & - \\
		\hline
	\end{tabular}
	\caption{
	Parameters used in the reference model.
    }
    \label{tb:settings}
\end{table*}



\subsection{Comparison with the numerical result}\label{sec:sweet_spot_compare}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{figure/sweet_spot/axip_dMcap.pdf}
    \caption{
    The planetesimal accretion rate vs.~the semi-major axis of the migrating planet. 
    The vertical solid lines show the boundaries of the sweet spot for planetesimal accretion (\SSP) given by Eq.~(\ref{eq:sweet_spot}).
    The red lines are for the case of $j=2$ and the green lines are for $j=3$.
    The filled areas show the \SSP.
    }
    \label{fig:Axi_dMcap}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Figure~\ref{fig:Axi_dMcap} shows the planetesimal accretion rate at each semi-major axis of the migrating protoplanet, obtained in the simulation for the reference model.
Planetesimal accretion is found to occur efficiently in a region of $2~\AU \lesssim a_{\rm p} \lesssim 10~\AU$. 
Beyond 10~$\AU$, planetesimals are trapped in the mean motion resonances of $j$ = 2 and 3 with the migrating protoplanet.
%When the protoplanet migrates in $\gtrsim10\AU$, 
%$j=2$ and $j=3$ mean motion resonances trap planetesimals as 
%the protoplanet migrates. 
Our analysis of the numerical results shows  that the condition of overstable libration is achieved, but the timescale of the instability growth is longer than the migration timescale; thus, the trapped planetesimals are shepherded without being captured by the protoplanet.
Around $\sim10\AU$, planetesimals trapped in the $2:1$ mean motion resonance start to escape due to the overstable libration.
The large amount of shepherded planetesimals are supplied into the planetary feeding zone, so that the accretion rate peaks at around $\sim8\AU$.
Aerodynamic shepherding starts around $5\AU$ for the planetesimals in the $2:1$ mean motion resonance, halting the supply of planetesimals through the $2:1$ mean motion resonance and reducing the accretion rate significantly.
Instead, planetesimal supply resumes through the $3:2$ mean motion resonance around $7\AU$ and the accretion rate increases again.
More specifically, planetesimals that remain to be brought into the feeding zone through $2:1$ mean motion resonance move to the $3:2$ resonance; namely, the accretion band shifts from $j=2$ to $j=3$. 
The accretion rate peaks again around $3\AU$ and then rapidly decreases around $2\AU$ due to aerodynamic shepherding.

In the simulation setting, the timescale ratio is given by: 
\begin{align}
    \frac{\tau_{\rm aero,0}}{\tau_{{\rm tide},a}} &= \left| \frac{\tau_{\rm aero,0}}{\tau_{{\rm tide},a}} \right|_{1 \AU} \left( \frac{j-1}{j} \right)^{1/3} a^{11/4}, \label{eq:tau_frac_dependence_on_a} \\
                                                &= \left| \frac{\tau_{\rm aero,0}}{\tau_{{\rm tide},a}} \right|_{1 \AU} \left( \frac{j-1}{j} \right)^{13/6} {a_{\rm p}}^{11/4}, \label{eq:tau_frac_dependence_on_ap} 
\end{align}
where
\begin{align}
    \left| \frac{\tau_{\rm aero,0}}{\tau_{{\rm tide},a}} \right|_{1 \AU} = 4.2 \times 10^{-3} \left(\frac{R_{\rm pl}}{10^7~\cm} \right) \left(\frac{\tau_{\rm tide,0}}{10^5~\yr} \right)^{-1}. \label{eq:tau_frac_0}
\end{align}
The red-shaded and green-shaded areas in Fig.~\ref{fig:Axi_dMcap} show the predicted regions of the \SSP, %given by Eq.~(\ref{eq:sweet_spot}), (\ref{eq:tau_frac_dependence_on_ap}) and (\ref{eq:tau_frac_0}), where 
$5~\AU~\lesssim~a_{\rm p}~\lesssim~10~\AU$ for $j=2$ and $1~\AU~\lesssim~a_{\rm p}~\lesssim~7~\AU$ for $j=3$, respectively, which one obtains using Eqs.~(\ref{eq:tau_frac_dependence_on_ap}) and (\ref{eq:tau_frac_0}) in Eq.~(\ref{eq:sweet_spot}).
Those regions turn out to cover the areas where the accretion rate is higher than  $10^{-6}~\Mear/\yr$.
Thus, we conclude that the derived equation for the \SSP\ reproduces well the numerical results in the reference model.


\subsection{Results of parameter studies}
As seen in Eq.~(\ref{eq:sweet_spot}), the location of the \SSP\ depends on the ratio of the gas drag damping timescale $\tau_{{\rm aero}, 0}$ to the planetary migration timescale $\tau_{{\rm tide}, a}$ and the planetary mass $M_{\rm p}$.
To investigate this dependence, we perform parameter studies for the size of planetesimals $R_{\rm pl}$, which determines $\tau_{\mathrm{aero}, 0}$, the scaling factor of migration timescale $\tau_{\rm tide,0}$, and the planetary mass $M_{\rm p}$.

\subsubsection{Dependence on the planetesimal's  size}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{figure/sweet_spot/ParameterStudy_psRpl.pdf}
    \caption{
    The results of the parameter study regarding the size of planetesimals $R_{\rm pl}$.
    {\bf Left:} Planetesimal accretion rate shown as a color contour on a plane of the semi-major axis of the migrating protoplanet and the planetesimal's radius.
    The analytically predicted inner and outer boundaries of the sweet spot are indicated with solid and dashed lines, respectively.
    The red lines are for $j=2$ and the green lines are for $j=3$.
    {\bf Right:} Total mass of captured planetesimals as a function of the planetesimal radius.
    }
    \label{fig:Result_ParameterStudy_Rpl}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Since the gas drag damping timescale $\tau_{\rm aero,0}$ increases with the size of planetesimals, the location of the \SSP\ is predicted to be closer to the central star for larger planetesimals (see, e.g., Eqs.~(\ref{eq:tau_frac_dependence_on_ap}) and (\ref{eq:tau_frac_0})).
We perform the numerical simulations, changing the size of planetesimals from $1 \times 10^5~\cm$ to $1 \times 10^8~\cm$ (or $\sim0.01\Mear$). 
Note that the assumption that mutual gravitational interaction among  planetesimals is negligible is not valid for large planetesimals with sizes of $R_{\rm pl} \sim 10^8~\cm$.
Nevertheless, a study for a wide parameter range is useful to deepen the  physical understanding of the effect of the damping timescale on planetesimal accretion.

Figure~\ref{fig:Result_ParameterStudy_Rpl} shows the results of the parameter study when changing the planetesimal's radius $R_{\rm pl}$.
In the left panel, the planetesimal accretion rate is shown as a color contour on a plane of the semi-major axis of the migrating protoplanet and the planetesimal's radius.
The analytically predicted inner and outer boundaries of the \SSP\ derived in sec.~\ref{sec:orbital_evolution_in_resonant_trapping} are shown with the solid and dashed lines, respectively.
The red lines are for $j=2$ and the green lines are for $j=3$.
In the right panel, the total mass of captured planetesimals $M_{\rm cap, tot}$ is plotted as a function of the planetesimal's radius.

The location of the \SSP\ (i.e., the region of high accretion rates) is found to be well reproduced by the analytical expressions derived in sec.~\ref{sec:orbital_evolution_in_resonant_trapping}.
The maximum accretion rate and the total captured heavy-element mass are higher for larger planetesimals.
This is because as the \SSP\ moves inward, the amount of planetesimals shepherded into the \SSP\ increases.
More planetesimals are shepherded into the \SSP\ when the planetesimals are larger, where the \SSP\ locates farther from the initial planet location (or closer to the central star).

\subsubsection{Dependence on the planetary migration timescale}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{figure/sweet_spot/ParameterStudy_psTtide0.pdf}
    \caption{
    Same as Fig.~\ref{fig:Result_ParameterStudy_Rpl}, but for the results of the parameter study regarding the migration timescale $\tau_{\rm tide,0}$.
    The gray circles in the right panel show the results of the parameter study regarding the size of planetesimals $R_{\rm pl}$ for comparison using the fraction of timescales $\tau_{\mathrm{aero}, 0}/\tau_{\mathrm{tide}, a}$ in vertical axis.
    }
    \label{fig:Result_ParameterStudy_Tmig0}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Next, we perform a parameter study when changing the planetary migration timescale. 
Our analytic consideration above indicates that the location of the \SSP\ is closer to the central star for faster planetary migration. 
We perform numerical simulations with various migration timescales by changing the scaling factor of migration timescale $\tau_{\rm tide,0}$ from $1 \times 10^4~\yr$ to $1 \times 10^6~\yr$.

Figure~\ref{fig:Result_ParameterStudy_Tmig0} shows the dependence of the results to the migration timescale $\tau_{\rm tide,0}$.
Indeed, in the left panel, the \SSP\ is found to be closer to the star for faster planetary migration (or smaller $\tau_{\rm tide,0}$). 
Since the \SSP\, moves inward as $\tau_{\rm tide,0}$ decreases, for the same reason described above, the total mass of captured planetesimals $M_{\rm cap, tot}$ increases with decreasing $\tau_{\rm tide,0}$, which is confirmed in the right panel.
The right axis shows $\tau_{\mathrm{aero}, 0}/\tau_{\mathrm{tide}, a}$
at $1\AU$ calculated with Eq.~(\ref{eq:tau_frac_0}).
For comparison, we also plot with grey circles $M_{\rm cap, tot}$ vs. $\tau_{\mathrm{aero}, 0}/\tau_{\mathrm{tide}, a}$ relation by converting the result shown in the right panel of Fig.~\ref{fig:Result_ParameterStudy_Rpl} when using  Eq.~(\ref{eq:tau_frac_0}).
Except for $\tau_{\rm tide,0}$ $\lesssim$ $10^{4.6}\yr$, the two results are similar. 
This confirms that the location of the \SSP\ scales with the ratio of the timescales $\tau_{\rm aero,0}/\tau_{\rm tide,a}$.

The effects of planetary migration, however, seems somewhat more complicated relative to the dependence on the planetesimal's radius.
First, as shown in the left panel, for relatively fast migration ($\tau_{\rm tide,0} \lesssim 10^{4.6}$~yr), the outer boundary of the \SSP\, expands beyond the one inferred analytically. 
Second, the $M_{\rm cap, tot}$ vs. $\tau_{\mathrm{aero}, 0}/\tau_{\mathrm{tide}, a}$ relation differs between the cases when we vary $R_{\rm pl}$ and varying  $\tau_{\mathrm{tide},0}$ for $\tau_{\rm tide,0} \lesssim 10^{4.6}~\yr$. 
This is related to the stability of resonant trapping.
As shown in sec.~\ref{sec:condition_for_resonant_trapping}, the condition required for resonant trapping is that the timescale for planetesimals to cross the mean motion resonance is longer than the libration timescale.
Using Eq.~(\ref{eq:condition_for_resonant_trapping_mig}), we find that stable resonant trapping is difficult for fast planetary migration like $\tau_{\rm tide,0} \lesssim 10^4~\yr$.
%In this case, the planetesimals are barely trapped into the resonances, but the resonant trapping is unstable due to the fast planetary migration.

Figure~\ref{fig:Result_ParameterStudy_time_phase_angle} shows the changes in the phase angle of a planetesimal initially located at $a_{\rm 0}=13.8~\AU$ in the cases of (a) $\tau_{\rm tide,0}=10^4~\yr$ and (b) $\tau_{\rm tide,0}=10^5~\yr$.
In panel (a), the phase angle continues libration even after trapped into the resonance.
This is because fast planetary migration perturbs the orbit of the trapped planetesimal and accelerates the overstable libration. 
The resonant trapping is, thus, broken earlier in the case of $\tau_{\rm tide,0}=10^4~\yr$ than in the case of $\tau_{\rm tide,0}=10^5~\yr$, which results in the outward expansion of the \SSP.
However, such an outward shift of the outer edge of the \SSP\ does not lead to an  increase in the mass of captured planetesimals.
This is because fast planetary migration breaks the resonant trapping as soon as the trapped planetesimal reaches the equilibrium condition.
The planetesimal in panel (a) escapes from the resonant trapping with $e\sim0.7$ and that in panel (b) with $e\sim0.4$.
The capture probability of planetesimals decreases with increasing eccentricity \citep{Ida+1989}; thus, the total mass of captured planetesimals does not increase with the expansion of the \SSP\ in the cases of $\tau_{\rm tide,0}\lesssim10^{4.6}~\yr$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{figure/sweet_spot/time_Phase.pdf}
    \caption{
    Change in the phase angle of a planetesimal initially located at $a_{\rm 0}=13.8~\AU$.
    Panel~(a) shows the case of $\tau_{\rm tide,0} = 1 \times 10^4~\yr$ and panel~(b) shows the case of $\tau_{\rm tide,0} = 1 \times 10^5~\yr$. 
    In panel~(a), the phase angle oscillates indicating that the resonant trapping is unstable due to the fast planetary migration.
    Then, the resonant trapping is broken earlier in the case of panel~(a) than that shown in panel~(b). 
    }
    \label{fig:Result_ParameterStudy_time_phase_angle}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsubsection{Dependence on the planetary mass}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{figure/sweet_spot/ParameterStudy_psMp.pdf}
    \caption{
    Same as Fig.~\ref{fig:Result_ParameterStudy_Rpl}, but for the results of the parameter study when varying the protoplanet's mass $M_{\rm p}$.
    The red, green, skyblue, and blue lines represent the \SSP\ inner (solid lines) and outer (dashed lines) boundaries determined by the resonant trapping, which is predicted by Eq.~(\ref{eq:sweet_spot}) for $j$ = 2, 3, 4, and 5, respectively.
    The coloured lines change into the gray lines once the protoplanet mass exceeds a threshold value, beyond which the accretion bands disappear (see Fig.~\ref{fig:Mp_EccCross}).
    }
    \label{fig:Result_ParameterStudy_Mp}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Finally, we perform a parameter study of the simulations when varying the mass of the migrating protoplanet $M_{\rm p}$ in the range of $M_{\rm p}/M_{\rm s}$ between $1 \times 10^{-4}$ and $1 \times 10^{-2}$.
The results are summarised in Figure~\ref{fig:Result_ParameterStudy_Mp}. 
We find that the semi-major axis of the outer boundary of the \SSP\, is insensitive to the protoplanet mass, which is consistent with Eq~(\ref{eq:sweet_spot}). 
In this figure we indicate the locations of the inner edge of the \SSP\, for $j$ = 4 and 5 in addition to those for $j$ = 2 and 3 given by Eq.~(\ref{eq:sweet_spot}), confirming that Eq.~(\ref{eq:sweet_spot}) accuratly reproduces the numerical result.
As shown in Fig.~\ref{fig:Mp_EccCross}, the crossing points between the resonance centre and the feeding zone boundary disappear once the planetary mass exceeds a specific value. 
In Fig.~\ref{fig:Result_ParameterStudy_Mp}, we show the $M_{\rm p}$-$a_{\rm p}$ relation corresponding to the disappearance of the crossing points with gray solid lines.
This is also consistent with the numerical result.

As found in \citet{Shibata+2020}, the total mass of captured planetesimals $M_{\rm cap,tot}$ changes with the planetary mass in a non-monotonic manner and takes local maxima at $M_{\rm p}/M_{\rm s}\sim10^{-3.6}$, $10^{-3.3}$, $10^{-2.7}$ and $10^{-2.2}$. 
This periodical changes come from the corresponding shifts of the inner boundary of the  \SSP.
The shepherding process that regulates the inner boundary of the \SSP\ changes from the aerodynamic shepherding to the resonant shepherding with increasing planetary mass.  
The accretion bands also change with the protoplanet mass.
%This change of the regulating process occurs at $M_{\rm p}/M_{\rm s}\sim10^{-3.6}$ for $j=5$, $M_{\rm p}/M_{\rm s}\sim10^{-3.4}$ for $j=4$, $M_{\rm p}/M_{\rm s}\sim10^{-3.0}$ for $j=3$ and $M_{\rm p}/M_{\rm s}\sim10^{-2.4}$ for $j=2$.
%Due to 
Because of these effects, the location of the inner boundary of the \SSP\ shifts  non-monotonically which results in the non-monotonic change of $M_{\rm cap,tot}$. %the total captured mass of planetesimals .
The global decreasing trend with increasing protoplanet mass comes from the outward shift of the inner boundary.
%is explained by the shift of the mean motion resonances through which planetesimals enter the feeding zone and the change of $e_{\rm cross}$.

%The periodical change of the total mass of captured planetesimals comes from the shift of the effective accretion bands.
%The feeding zone boundary expands with the planetary mass.
%The cross points between the resonances and the feeding zone boundary change with the planetary mass, and some of the cross points disappear for larger planetary mass as shown in Fig.~\ref{fig:Mp_EccCross}.
%Figure~\ref{fig:Result_ParameterStudy_histgram} shows the total mass of planetesimals that enter the feeding zone, or the total mass flow of planetesimals, as a function of their period ratio with the migrating planet at the time of entry.
%histogram of mass flow into the feeding zone with the period ratio between planetesimals and migrating planet.
%From top panel to bottom panel, planetary mass is $M_{\rm p}/M_{\rm s} = 1.0\times10^{-4}$, $M_{\rm p}/M_{\rm s} = 2.0\times10^{-4}$, $M_{\rm p}/M_{\rm s} = 7.9\times10^{-4}$ and $M_{\rm p}/M_{\rm s} = 1.6\times10^{-3}$, respectively.
%In the case of $M_{\rm p}/M_{\rm s} = 1.0\times10^{-4}$, effective accretion bands are $3:2$, $4:3$ and $5:4$ mean motion resonances.
%$2:1$ resonance is ineffective because planetary mass is too small for the resonance to trap planetesimals, namely the condition given by eq.~(\ref{eq:condition_for_resonant_trapping_mig}) is not achieved.
%As the planetary mass increases, the effective accretion bands shift for those with smaller $j$.
%Accretion bands of $5:4$, $4:3$ and $3:2$ resonances are disappear in the case of $M_{\rm p}/M_{\rm s} = 1.6\times10^{-3}$.



==> Shibata et. al. 2021/text/trash/heavy_elements.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}%f1
    \begin{center}
    \includegraphics[width=80mm]{figure/sweet_spot/SS_Type2mig.pdf}
        \caption{
        Distribution of confirmed exoplanets in the semi-major axis vs. planetary mass plane.
        The black points are exoplanets observed by the radial-velocity method.
        The red points are exoplanets observed by the radial-velocity + transit methods.
        As for masses of exoplanets indicated with the black points, the observe values of $M_{\rm p} \sin i$ are simply used.
        The gray area shows the theoretical sweet spot for planetesimal capture given by eqs.~(\ref{eq:sweet_spot_in_disk_1}) and (\ref{eq:sweet_spot_in_disk_2}) with $C=1$.
        }
        \label{fig:Application_Exoplanet}
    \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The location of the sweet spot depends on the ratio of the two timescales of gas drag and tidal damping.
We consider that the planet migrates in the type II regime, the migration rate for which is given  by \citet{Kanagawa+2018} and that the surface density profile in the protoplanetary disk is given by the so-called self-similar solution \citep{Lynden-Bell+1974}, where $\alpha_{\rm disk}\sim1$ except around the outer edge of the protoplanetary disk.
Assuming the optically thin disk $\beta_{\rm disk}=1/2$ and substituting eq.~(\ref{eq:fraction_timescales_simple}) into the analytical expressions of the sweet spots, eqs.~(\ref{eq:condition_for_aerodynamic_shepherding}), (\ref{eq:overstable_libration_due_to_gasdrag}) and (\ref{eq:condition_for_resonant_breaking_grow}), we obtain the inner and outer edge of the sweet spot $a_{\rm SS,in}$ and $a_{\rm SS,out}$ as
\begin{align}
    a_{\rm SS,in} &= {\rm max} \left.
            \begin{cases}
                1.4 C^{1/3} \left(\frac{M_{\rm p}/M_{\rm s}}{10^{-3}}\right)^{2/3} \left(\frac{j}{j-1} \right)^{7/9} \\
                1.1 C^{1/3} \left(\frac{M_{\rm p}/M_{\rm s}}{10^{-3}}\right)^{1/3} \left(\frac{j}{j-1} \right)^{5/18} \frac{e_{\rm cross}}{0.1}
            \end{cases} \right\} \AU, \label{eq:sweet_spot_in_disk_1} \\
    a_{\rm SS,out} &= 7.6 C^{1/3} \left(\frac{M_{\rm p}/M_{\rm s}}{10^{-3}}\right)^{1/3} \left\{ \frac{j^{5}}{(j-1)^{8}} \right\}^{1/18} \AU. \label{eq:sweet_spot_in_disk_2} %\frac{r_{\rm p}}{1\AU} <
    \end{align}
Hereafter, we consider the case of $C=1$ (see eq.~(\ref{eq:sweet_spot_constant_C})).

Figure~\ref{fig:Application_Exoplanet} shows observed exoplanets and the location of the sweet spot in the $a_{\rm p}$-$M_{\rm p}$ plane.
The sweet spot locates from $\sim0.3\AU$ to $10\AU$ and shifts outward with the increase of planetary mass.
The red and black dots show exoplanets observed using  the transit method and the radial velocity method, respectively.
After the onset of runaway gas accretion, $M_{\rm p}$ increases.
Also, $a_{\rm p}$ decreases due to type II planetary migration.
The evolution paths of gas giant planets plane can be drawn from right-bottom to left-top direction in the $a_{\rm p}$-$M_{\rm p}$.
If the runaway gas accretion started in the region exterior to the water snow line, which is considered to locate at $\sim1$-$3\AU$, the exoplanets currently observed in the region interior to the sweet spot crossed the sweet spot during their migration.
On the other hand, the exoplanets currently observed in the region exterior to the sweet spot did not crossed the sweet spot.
Planetesimal mass that is accreted onto the planets would differ between those two populations of planets.
If we observe the difference in the amount of heavy elements between gas giant planets inside and outside the predicted sweet spot, it could be an evidence of planetesimal accretion during planetary migration.
Hereafter, we estimate the heavy-element mass in gas giant planets expected from planetesimal accretion.



%\subsection{Heavy element contents in gas giant planets}\label{sec:Application_Model}
\subsection{A model of planetesimal accretion along formation paths of gas giant planets}\label{sec:Model_PlanetsimalAccretion}
We consider that a protoplanet with a critical core mass $M_{\rm p}=M_{\rm p,0}$ begins runaway gas accretion at $a_{\rm p}=a_{\rm p,0}$.
The planet grows in mass to $M_{\rm p}=M_{\rm p,f}$ thorough a rapid gas accretion, followed by inward migration in the Type II regime and stops at $a_{\rm p}=a_{\rm p,f}$ with $M_{\rm p}=M_{\rm p,f}$ due to disk dissipation.
The formation phase can be divided into two phases, mass growth phase ($M_{\rm p}:M_{\rm p,0}\rightarrow~M_{\rm p,f}$) and planetary migration phase ($r_{\rm p}:r_{\rm p,0}\rightarrow~r_{\rm p,f}$), and planetesimal accretion occurs in both phases.
In the reality the protoplanet is expected to start migrating before runaway gas accretion terminates, but for the sake of simplicity we assume that migration and gas accretion occur one after the other. 
In this case, the total accreted heavy-element mass  $M_{\rm Z,tot}$ is given by: 
\begin{align}
    M_{\rm Z,tot} = M_{\rm Z,core} +M_{\rm Z,grow} +M_{\rm Z,mig}, \label{eq:Application_Mztot}
\end{align}
where $M_{\rm Z,core}$, $M_{\rm Z,grow}$ and $M_{\rm Z,mig}$ are the core mass, planetesimal mass accreted onto the planet during the planetary growth, and the accreted mass during the planetary migration phase, respectively.
\shibata{
----- It would be better to use $M_{\rm Z,crit}$ instead of $M_{\rm Z,core}$.
$M_{\rm Z,crit}$ is a total amount of heavy elements at the onset of runaway gas accretion.
}

The core mass is set as the critical core mass $M_{\rm crit}$, at which runaway gas accretion begins.
Planetesimal accretion after the onset of the runaway gas accretion and core erosion could change the core mass from the critical core mass. 
{\bf what about Claudio's calculations that show that there is a lot of H-He accreted before runaway gas accretion takes place??\\}
Some of the accreted planetesimals during runaway gas accretion could reach the deeep interior  \citep{Mordasini+2006,Valletta2019}.
The convection of envelope gases can erode the solid core and reduce the core mass \citep{Guillot+2004}. 
{\bf but see Cumming et al and references therein  suggesting that giant planets could be radiative... \\}
%from $M_{\rm crit}$ 
Both effects could change the distribution of heavy elements inside the gas giant planet, but the total amount of heavy element $M_{\rm Z,tot}$ is conserved.
To focus on $M_{\rm Z,tot}$, we neglect the effects which could change the heavy-element distribution.
{\bf so why are we discussing it in detail??\\}
\shibata{
------ Maybe we don't need to discuss on this point...
}

%Thus, we consider that the core mass does not change after the onset of the rapid gas accretion.
Recent studies suggest $M_{\rm crit}\lesssim10\Mear$ \citep{Hori+2011,Venturini+2015,Brouwers+2018}.
Here we set $M_{\rm Z,core}=10\Mear$.

During the early stages of the planetary growth, the heavy-element accretion depends on the mass of planetesimals inside the planetary feeding zone.
The planetesimal accretion rate depends on the timescales of planetary mass growth and gas damping of planetesimal orbits \citep{Shiraishi+2008,Shibata+2019}.
We define the fraction of planetesimals captured by the planet in the early phase $f_{\rm growth}$ as
\begin{align}
    f_{\rm growth} \equiv \frac{M_{\rm Z,grow}}{M_{\rm Z,fz}(a_{\rm p,0},M_{\rm p,f})}.
\end{align}
where $M_{\rm Z,fz}$ is the mass of planetesimals inside the feeding zone given as
\begin{align}
    M_{\rm Z,fz} (a_{\rm p},M_{\rm p}) &= \int_{\rm a_{\rm fz,in}(a_{\rm p},M_{\rm p})}^{\rm a_{\rm fz,out}(a_{\rm p},M_{\rm p})} 2 \pi r \Sigma_{\rm solid} {\rm d} r,
\end{align}
with
\begin{align}
    a_{\rm fz,in}   &= a_{\rm p} \left\{1-2\sqrt{3} \left(\frac{M_{\rm p}}{3M_{\rm s}} \right)^{1/3} \right\}, \label{eq:feeding_zone_0_axi_in} \\
    a_{\rm fz,out}  &= a_{\rm p} \left\{1+2\sqrt{3} \left(\frac{M_{\rm p}}{3M_{\rm s}} \right)^{1/3} \right\}. \label{eq:feeding_zone_0_axi_out}
\end{align}
According to the results of numerical simulations by \citet{Shibata+2019}, $f_{\rm growth}$ takes $\lesssim0.3$. % and takes the maximum when the timescale of mass growth is shorter than the timescale of gas damping.

On the other hand, during planetary migration the  planet can capture planetesimals which are shepherded into the sweet spot $M_{\rm Z,shep}$.
During the migration, planetesimals initially located from the inner edge of the sweet spot $a_{\rm SS,in}$ to the inner edge of the feeding zone when the planet begins to migrate $a_{\rm fz,in}(a_{\rm p,0},M_{\rm p,f})$ have a possibility to be shepherded into the sweet spot.
$M_{\rm Z,shep}$ is given by
\begin{align}
    M_{\rm Z,shep} &= \int_{\rm a_{\rm SS,in}}^{\rm a_{\rm fz,in}} 2 \pi r \Sigma_{\rm solid} {\rm d} r. \label{eq:M_z_shep}
\end{align}
%$a_{\rm SS,in}$ is given by eqs.~(\ref{eq:sweet_spot_in_disk_1}) and (\ref{eq:sweet_spot_in_disk_2}).
We define the fraction of planetesimals captured by the planet during planetary migration as
\begin{align}
    f_{\rm mig} \equiv \frac{M_{\rm Z,mig}}{M_{\rm Z,shep}}.
\end{align}
where we found that $f_{\rm mig}$ is $\lesssim 0.3$.
%Note that $a_{\rm SS,in}$ depends on many parameters like $\alpha_{\rm vis}$ and $R_{\rm pl}$ as shown in eq.~\ref{eq:sweet_spot_constant_C}.
%Here we neglect those effects on $M_{\rm Z,tot}$ because the variation in $f_{\rm disk}$ is much more important for estimating $M_{\rm Z,tot}$ as shown below.

Both $M_{\rm Z,growth}$ and $M_{\rm Z,mig}$ depend on the radial distribution of planetesimals in the protoplanetary disk.
Two potential planetesimal formation mechanisms include:
continuous coagulation of fluffy dust particles \citep{Okuzumi+2012} and
gravitational contraction of particle clumps formed by the streaming instability \citep{Youdin+2005}.
In recent studies, the planetesimal formation through the streaming instability is actively discussed because it can directly form km-size planetesimals from pebble-size particles skipping problems concerning the continuous growth of small particles, such as the bouncing problem of collision growth \citep{Windmark+2012}.
In addition, observed features in Solar System's Kuiper belt objects support the formation of planetesimals through the streaming instability.
The Kuiper belt binaries are typically made of the similar size and the same color objects \citep{Noll+2008}, which is consistent with the result that the formation of a binary is the natural result of the gravitational collapse of the pebble clump \citep{Nesvorny+2010}.
The streaming instability requires sedimentation of particles in disks with more than $\sim1\%$ metallicity  \citep{Youdin+2002,Johansen+2009,Simon+2016}.
Certain locations like the vicinity of snowline \citep{Armitage+2016} or the vicinity of disk inner edge \citep{Drazkowska+2016} enhance the local disk metallicity due to the pile up of radially drifted pebbles.
Even in other locations, non-laminar flow, or zonal flow originating from various instabilities, traps radially drifted solid particles and enhances local solid-to-gas ratio \citep[see references in][]{Klahr+2018,Lenz+2019}.
These studies suggest that planetesimal formation through the streaming instability can be triggered everywhere in the circumstellar disk.
Assuming the planetesimal formation rate depends on the instantaneous radial pebble flux, \citet{Lenz+2019} found that the surface density profile of planetesimals tends to be steeper than that of gas.
Their model helps explain the discrepancy between the minimum-mass solar nebula, which is modeled from the distribution of solid materials in our solar system, and viscous accretion disks.
Here, we consider the limiting case where planetesimal formation occurs everywhere in the disk and all solid materials are in the form of planetesimals.
We set $\alpha_{\rm disk}^{\prime}=3/2$ and parameterize $\Sigma_{\rm solid}$ using a scaling factor $f_{\rm disk}$ as
\begin{align}
    \Sigma_{\rm solid}  &= f_{\rm disk} \times
        \begin{cases}
            7.1\times\left(\frac{r}{1\AU}\right)^{-3/2}~\text{ for } r<r_{\rm ice} \\
            30.\times\left(\frac{r}{1\AU}\right)^{-3/2}~\text{ for } r_{\rm ice}<r,
        \end{cases} \label{eq:disk_solid_MMSN}
\end{align}
where $r_{\rm ice}$ is the radial distance of the water ice line and given as $r_{\rm ice}\sim2.7\AU$ in our disk model.
The values of $\Sigma_{\rm solid}$ for $f_{\rm disk}=1$ is the same as that in the minimum-mass solar nebula.
Given the initial formation location $a_{\rm p,0}$ and observed parameters $a_{\rm p,f}$ and $M_{\rm p,f}$, we can calculate the amounts of heavy elements in gas giant planets $M_{\rm Z,tot}$ from the above equations.


\subsection{Heavy element content of inner gas giant planets}\label{sec:Application_Model_InnerPlanet_result}
\subsubsection{Model estimate}\label{sec:Application_result_innerplanet}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}%f1
  \begin{center}
    \includegraphics[width=80mm]{figure/discussion/Axip0_Mpz_Mcap.pdf}
    \caption{
    The estimated heavy-element mass in a gas giant planet as a function of the initial semi-major axis of the planet $a_{\rm p,0}$.
    We consider the case of $f_{\rm disk}=2$ and $M_{\rm p,f}/M_{\rm s}=10^{-3}$.
    The red, green, and blue lines show $M_{\rm Z,core}$, $M_{\rm Z,grow}$ and $M_{\rm Z,mig}$, respectively.
    The black solid line shows $M_{\rm Z,tot}$ for planets which crossed the sweet spot in the planetary migration phase.
    The black dashed line shows $M_{\rm Z,tot}$ for planets which did not reach the sweet spot, namely $M_{\rm Z,tot}=M_{\rm Z,core}+M_{\rm Z,mig}$.
    }
    \label{fig:Application_Mtot}
  \end{center}
\end{figure}
%
\begin{figure}%f1
  \begin{center}
    \includegraphics[width=80mm]{figure/discussion/mu_Mpz_Mcap_Axip20.pdf}
    \caption{
    Same as Fig.~\ref{fig:Application_Mtot}, but as a function of the final planet mass $M_{\rm p,f}$.
    We consider the case of $f_{\rm disk}=2$ and $a_{\rm p,0}=20~\AU$.
    }
    \label{fig:Application_Mtot2}
  \end{center}
\end{figure}
%
\begin{figure}%f1
  \begin{center}
    \includegraphics[width=80mm]{figure/discussion/hist_fdiskp.pdf}
    \caption{
    The distribution of $f_{\rm disk}$ of circumstellar disks in star formation regions.
    $f_{\rm disk}$ is calculated from the disk total mass $M_{\rm disk}$ and disk characteristic radius $R_{\rm disk}$ obtained in \citet{Andrews+2010}.
    Here, we assume that the disk inner edge locates at $0.1~\AU$ and $Z_{\rm s}=Z_{\rm \odot}$ for simplicity.
    }
    \label{fig:Application_fdisk}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Here we investigate the accreted heavy-element mass for  giant planets in regions interior to the sweet spot. 
These planets crossed the sweet spot during their formation stages if the planets started runaway gas accretion in the outer disk as $1\AU\lesssim~a_{\rm p,0}$.
We set $f_{\rm growth}=0.3$ and $f_{\rm mig}=0.15$, which was obtained from our numerical calculations in \citet{Shibata+2019} and in sec.~\ref{sec:sweet_spot_compare}.
The mass of the planetesimal disk is set as $f_{\rm disk}=2$.
Note that the value of $f_{\rm growth}$ and $f_{\rm mig}$ depends on various physical conditions such as the planetary growth rate and the  capture radius.
Here, we neglect those effects and use the results of specific numerical simulations.
Detailed investigations of $f_{\rm growth}$ and $f_{\rm mig}$ should be done in future works.

Figure~\ref{fig:Application_Mtot} shows the estimated heavy-element mass  $M_{\rm Z,tot}$ as a function of the initial semi-major axis of the planet $a_{\rm p,0}$. %where the planet started runaway gas accretion
During the accretion phase, the amount of planetesimals inside the feeding zone $M_{\rm Z,fz}$ increases with $a_{\rm p,0}$ because the area of the feeding zone expands. %increases approximately with ${a_{\rm p,0}}^2$.
During the planetary migration, the amount of planetesimals shepherded into the sweet spot $M_{\rm Z,shep}$ increases with $a_{\rm p,0}$.
As a result, both of the amounts of planetesimals accreting onto the planet during the accretion phase $M_{\rm Z,grow}$ and the planetary migration phase $M_{\rm Z,mig}$ increase with $a_{\rm p,0}$.
$M_{\rm Z,mig}$ more rapidly increases with $a_{\rm p,0}$ than $M_{\rm Z,grow}$ and $M_{\rm Z,mig}$ becomes larger than $M_{\rm Z,grow}$ around $\sim10\AU$.
The total heavy-element mass $M_{\rm Z,tot}$ also increases with $a_{\rm p,0}$ and several tens Earth-masses of planetesimals are captured by the planet if the planet starts the runaway gas accretion at $a_{\rm p,0}\gtrsim10\AU$.

Figure~\ref{fig:Application_Mtot2} shows $M_{\rm Z,tot}$ vs.~the final planetary mass $M_{\rm p,f}$.
Here, we set $a_{\rm p,0}=20\AU$.
As the planetary mass increases, $M_{\rm Z,grow}$ increases because the feeding zone expands with $M_{\rm p,f}$.
On the other hand, $M_{\rm Z,mig}$ decreases with $M_{\rm p,f}$ because the inner edge of the sweet spot $a_{\rm SS,in}$ moves outward.
As a result, $M_{\rm Z,tot}$ increases slightly with $M_{\rm p,f}$.

In the above results, we considered the case where the mass of the planetesimal disk $f_{\rm disk}$ is set as 2.
However, $f_{\rm disk}$ must change among between different disks and $M_{\rm Z,tot}$ linearly increases with $f_{\rm disk}$.
We consider that the disk of mass $M_{\rm disk}$ has a radius $R_{\rm disk}$ and a metallicity of $Z_{\rm s}$.
Assuming a continuous solid distribution, we can obtain $f_{\rm disk}$ from $M_{\rm disk}$, $R_{\rm disk}$ and $Z_{\rm s}$.
%We consider that $f_{\rm disk}$ relates with the disk total mass $M_{\rm disk}$, the characteristic disk radius $R_{\rm disk}$ and the metallicity of central star $Z_{\rm s}$.
According to observations of protoplanetary disks in star formation regions \citep{Andrews+2010}, the most frequent disk total mass and characteristic disk radius are $\sim0.03\Msun$ and $\sim50\AU$, respectively.
The disk mass and radius also have large scatterings: from $0.004\Msun$ to $0.136\Msun$ in disk total mass and from $14\AU$ to $198\AU$ in characteristic disk radius.
Given $M_{\rm disk}$ and $R_{\rm disk}$, we can obtain the value of $f_{\rm disk}$ solving
%\begin{align}
%    f_{\rm disk} = \frac{M_{\rm disk}}{4 \pi \Sigma_{\rm MMSN,0}} \left( R_{\rm disk}^{1/2}-R_{\rm disk,in}^{1/2} \right)^{-1}, \label{eq:Calculating_fdisk}
%\end{align}
\begin{align}
    Z_{\rm s} M_{\rm disk} = \int_{R_{\rm disk,in}}^{R_{\rm disk}} 2 \pi \Sigma_{\rm solid} {\rm d} r, \label{eq:Calculating_fdisk}
\end{align}
where $R_{\rm disk,in}$ is the radial distance of the disk inner edge.
Assuming the disk inner edge locates at $0.1\AU$ and $Z_{\rm s}=Z_{\odot}$, we can obtain $f_{\rm disk}$ from observed $M_{\rm disk}$ and $R_{\rm disk}$. % and metallicity of central star is same as solar metallicity $Z_{\rm \odot}$
Figure.~\ref{fig:Application_fdisk} shows the distribution of $f_{\rm disk}$ of disks used in \citet{Andrews+2010}.
Around stars with the solar metallicity, $f_{\rm disk}$ is most frequent around $\sim2$ and scattered in a wide range.
Considering the scattering in the metallicity of the  host stars, we suggest that $f_{\rm disk}$ changes from $\sim0.2$ to $\sim10$. % in two orders magnitude.
Thus, the distributions of $M_{\rm Z,tot}$ also has large scattering.

The scattering in $M_{\rm Z,tot}$ also comes from the scattering of other parameters.
$M_{\rm Z,tot}$ depends on $M_{\rm Z,shep}$, which decreases with the location of the inner edge of the sweet spot ${a_{\rm SS,in}}$. %^{1/2}
The location of the sweet spot depends on many parameters, such as disk viscosity $\alpha_{\rm vis}$, planetesimal density $\rho_{\rm pl}$, planetesimal size $R_{\rm pl}$, mass of central star $M_{\rm s}$, and disk temperature at $1\AU$ $T_{\rm disk,0}$ as shown in eqs.~(\ref{eq:sweet_spot_constant_C}) and (\ref{eq:sweet_spot_in_disk_2}). %sec.~\ref{sec:Part1_Discussion_SweetSpot}.
From eqs.~(\ref{eq:sweet_spot_constant_C}), (\ref{eq:sweet_spot_in_disk_2}) and (\ref{eq:M_z_shep}), we find that $M_{\rm Z,tot}$ depends on the $-1/6$ power of $\alpha_{\rm vis}$, $\rho_{\rm pl}$, $R_{\rm pl}$ and $M_{\rm s}$, and the $1/3$ power of $T_{\rm disk,0}$.
Here, we use the relation of $|h_{\rm s}/r|_{\rm 1AU}\propto {M_{\rm s}}^{-1/2} {T_{\rm disk,0}}^{1/2}$.
The effects of the scatterings in these parameters are smaller than the effect of the scattering in $f_{\rm disk}$, with which $M_{\rm Z,tot}$ increases linearly.
We conclude that the scattering in $M_{\rm Z,tot}$ mainly comes from the scattering in the disk mass $f_{\rm disk}$.


\subsubsection{Comparison with \citet{Thorngren+2016}}\label{sec:Application_Thorngren+2016}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}%f1
  \begin{center}
    \includegraphics[width=80mm]{figure/discussion/mu_Mpz.pdf}
    \caption{
    The amounts of heavy elements of gas giant planets estimated in \citet{Thorngren+2016} with the mass fraction $M_{\rm p}/M_{\rm s}$.
    }
    \label{fig:Application_Thorngren_mu_Mpz}
  \end{center}
\end{figure}
%
\begin{figure}%f1
  \begin{center}
    \includegraphics[width=80mm]{figure/discussion/hist_Mpz.pdf}
    \caption{
    The histogram of the amount of heavy elements $M_{\rm Z,tot}$ estimated in \citet{Thorngren+2016}.
    We select only the data the errors of which are less than $50\%$ from the samples in \citet{Thorngren+2016} and the number of selected samples is 32.
    The black bars show the histogram of all the samples and the red bars are Jupiter-size planets which have $10^{-3.5}<M_{\rm p}/M_{\rm s}<10^{-2.5}$.
    The width of the bin is set as $0.2$ in logarithmic scale.
    }
    \label{fig:Application_Thorngren}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Some of the gas giant planets that are located in the inner disk interior to the sweet spot are observed by both the radial velocity and transit methods and, thereby, their mass and radius are both measured.
\citet{Thorngren+2016} estimated the amounts of heavy elements in close-in gas giant planets and found some important features in the distribution of $M_{\rm Z,tot}$.
Figure~\ref{fig:Application_Thorngren_mu_Mpz} shows the $M_{\rm Z,tot}$ estimated in \citet{Thorngren+2016} with $M_{\rm p}/M_{\rm s}$. % instead of $M_{\rm p}$.
Here, we focus on the features found in the distribution of $M_{\rm Z,tot}$;
(i) $M_{\rm Z,tot}$ increases with $M_{\rm p}/M_{\rm s}$,
(ii) $M_{\rm Z,tot}$ have large diversity between similar mass planets,
(iii) there are some extremely enriched planets as $M_{\rm Z,tot}\gtrsim100\Mear$.
Note that \citet{Muller+2020} showed that the uncertainties originating from the model assumptions used in \citet{Thorngren+2016} are comparable or even larger than those from observation.
Hereafter we focus on the qualitative features obtained by \citet{Thorngren+2016} and discuss the formation of close-in gas giant planets using our model.

\citet{Thorngren+2016} derived a relation $M_{\rm Z,tot}~\propto~{M_{\rm p}}^{2/3}$ by fitting their estimated values.
In Fig.~\ref{fig:Application_Thorngren_mu_Mpz}, we take $M_{\rm p}/M_{\rm s}$ as the horizontal axis instead of $M_{\rm p}$ and find that $M_{\rm Z,tot}$ also increases with $M_{\rm p}/M_{\rm s}$.
In our model, $M_{\rm Z,tot}$ depends on $M_{\rm p}/M_{\rm s}$ but the dependence is too weak to explain the observed relation between $M_{\rm Z,tot}$ and $M_{\rm p}/M_{\rm s}$ (see Fig.~\ref{fig:Application_Mtot2}).
On the other hand, $M_{\rm Z,tot}$ increases with $a_{\rm p,0}$ (see Fig.~\ref{fig:Application_Mtot}).
To explain the relation between $M_{\rm Z,tot}$ and $M_{\rm p}/M_{\rm s}$, we suggest that heavier close-in gas giant planets had formed cores of critical mass farther away from the central stars and then migrated over longer radial distances.
Such a relation between the initial formation location and the final planet mass of gas giant planet is also suggested from the formation theories of gas giant planets.
The model combining the gas accretion rate and planetary migration rate \citep{Tanigawa+2007,Tanigawa+2016} showed that planets which start runaway gas accretion in the outer disk grow to be heavier planets.
The evolution paths shown in population synthesis models \citep[e.g.][]{Bitsch+2015,Mordasini2014,Ida+2018} also imply that heavier gas giant planets migrate longer radial distances and the possibility for Jupiter-mass planets to migrate several tens $\AU$ in planetary migration phase.
On the other hand, \citet{Tanaka+2020} showed that close-in gas giant planets with $M_{\rm p}/M_{\rm s}\lesssim10^{-2}$ had started runaway gas accretion interior to the water snow line and migrated only a few $\AU$ in their formation stages.
Along their formation paths, close-in gas giant planets barely capture planetesimals and the outcome is inconsistent with the result in \citet{Thorngren+2016}.
To migrate long distance, gas giant planets needs to move before reaching higher planetary mass, because migration timescale in type II regime increases with the planetary mass.
Our results suggest that the migration timescale compared to the mass growth timescale is smaller than that used in \citet{Thorngren+2016}.

\begin{comment}
In the above formation models, the radial migration distance of gas giant planets is determined by the competitions between the timescales of gas accretion and planetary migration.
Both timescales depend on the gap structure opened by the planet and the studies of these timescales are still under discussion, especially for the gas accretion timescale.
\citet{Tanigawa+2002} investigated the gas accretion rate of giant planets using a two-dimensional hydrodynamic simulations.
They found that gas accretion occurs through a narrow band and derived an analytical formula for the width of the accretion band.
Three-dimensional hydrodynamic simulations, however, showed the possibilities that gas accretion rate is smaller than that obtained in two-dimensional hydrodynamic simulations \citep{Lissauer+2009,Machida+2010}.
%The timescale of type II migration is regulated by the viscous timescale of the circumstellar disk in the classical regime \citep[e.g.][]{Lin+1993}.
\citet{Kanagawa+2018} investigated the migration timescale using two-dimensional hydrodynamic simulations and found that the migration timescale for gap opening planets depends on the surface density of disk gas at the gap bottom. %is longer than the classical one.
Their fitting model of migration timescale, which is written by eq.~(\ref{eq:type2_migration_regime_K18}), has still uncertainties up to 1 order.
In the model of \citet{Tanaka+2020}, the migration timescale is long relative to the gas accretion timescale, which results in the short migration distance.
If the migration rate is faster than that used in their model, the migration distance becomes longer.
Thus, our model suggests the possibility that gas accretion timescale is longer than that obtained in two-dimensional hydrodynamic simulations.
\end{comment}

The large scattering in $M_{\rm Z,tot}$ between similar mass planets is also important characteristic of close-in gas giant planets.
Figure~\ref{fig:Application_Thorngren} shows the histogram of $M_{\rm Z,tot}$ estimated in \citet{Thorngren+2016}.
To draw this figure, we select only the data, the errors of which are less than $50\%$ from the samples in \citet{Thorngren+2016} and the number of selected samples is 32.
The black bars show the histogram of all the samples and the red bars are Jupiter-size planets which have $10^{-3.5}<M_{\rm p}/M_{\rm s}<10^{-2.5}$.
The distribution of $M_{\rm Z,tot}$ of Jupiter-size planets spreads from $10\Mear$ to $200\Mear$ and the peak of the distribution is around $50\Mear$.
As discussed in sec.~\ref{sec:Application_result_innerplanet}, the scattering in $M_{\rm Z,tot}$ mainly comes from the scattering of $0.2~\lesssim~f_{\rm disk}~\lesssim~10$, which covers the scattering found in $M_{\rm Z,tot}$ estimated by \citet{Thorngren+2016}.
The effects of other parameters, such as the disk viscosity or planetesimal radius, are not enough to generate such a large scattering.
We suggests that the large scattering shown in the distribution of $M_{\rm Z,tot}$ comes from the scattering of $f_{\rm disk}$.
This suggestion should be discussed in future when the number of observations in $M_{\rm Z,tot}$ and circumstellar disk increases.

Finally, we focus on some close-in gas giant planets that contain more than $100\Mear$ heavy elements as shown in Fig.~\ref{fig:Application_Thorngren_mu_Mpz}.
To capture such massive heavy elements via planetesimal accretion, those planets need to be formed in a massive circumstellar disk as $f_{\rm disk}\sim10$ and migrate more than $\gtrsim50\AU$. %from the outer edge of the circumstellar disk.
Disk instability model is preferred for such formation paths of gas giant planets than core accretion model.
Our model suggests that close-in gas giant planets containing more than $100\Mear$ heavy elements formed via disk instability.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Heavy element contents in outer gas giant planets} \label{sec:Application_Model_OuterPlanet}
Gas giant planets which locate in the region exterior to the sweet spot are observed by radial velocity method and, thereby, their masses are measured as shown in fig.~\ref{fig:Application_Exoplanet}.
Jupiter and Saturn also locate in this region.
Here we consider the amounts of heavy elements contained in gas giant planets which locate in the region exterior to the sweet spot.

\subsubsection{In exoplanets}
\label{sec:Application_Model_OuterExoplanets}
%Here, we consider the single gas giant planet and do not consider the outward migration as considered in Grand-Tuck model \citep{Walsh+2011}, which occurs in multi-planetary systems.
We consider the heavy elements contents in exoplanets observed in the region exterior to the sweet spot.
During the formation phase, the circumstellar disk dissipated before the planets reached the sweet spot.
In this case, the accretion of planetesimals did not occur in the planetary migration phase.
Between the populations of planets which locate in the regions interior and exterior to the sweet spot, a clear difference in $M_{\rm Z,tot}$ would exist.
If we can observe the clear difference in $M_{\rm Z,tot}$ between these populations, it suggests that the heavy elements in gas giant planets are mainly brought by planetesimal accretion.

The transition frequency and probability decrease with the orbital period of planets.
So the transit observation of planets in the region exterior to the sweet spot is lack now.
Considering the scattering of $M_{\rm Z,tot}$, we need large number of observations to compare the populations.
In addition, we need high accuracy in measuring the radius of those gas giant planets.
If the formation of Jupiter-size planet starts around $a_{\rm p,0} \sim 20\AU$ in the disk of $f_{\rm disk}=2$, the planets which crossed the sweet spot contain more $\sim10\Mear$ heavy elements than the planets which did not reached the sweet spot during the planetary migration phase (see fig.~\ref{fig:Application_Mtot}).
The $10\Mear$ difference in the amount of heavy elements in Jupiter-mass planet makes a few percent difference in the radius of the planets $\sim0.01~R_{\rm Jup}$ \citep{Thorngren+2016}.
$\sim1\%$ accuracy in the observation of planet radius is limited for some planetary systems.
In conclusion, long term and wide field observations with high accuracy are required for comparing the populations of planets in the regions interior and exterior to the sweet spot.
Such observation should be done in future.

\subsubsection{Jupiter and Saturn}\label{sec:Application_Model_SolarSystem}
For the gas giant planets in our solar system, not only the mass and radius but also the gravitational moments $J_{n}$ are measured. 
%by spacecrafts exploration.
The bulk amounts of heavy elements contained in Jupiter and Saturn are not well-determined but are estimated to be $\sim24$-$46\Mear$ and $\sim16$-$30\Mear$, respectively.
Jupiter and Saturn are located in the region exterior to the sweet spot, and the accretion of planetesimals probably did not occur during  planetary migration phase. {\bf I am not sure I understand what you mean...\\}
The heavy elements in Jupiter come from the initial core and accretion of planetesimals in mass growth phase.
In this case, the amount of heavy elements increases with $f_{\rm disk}$, $a_{\rm p,0}$ and $M_{\rm p,f}$.
If this is indeed the case, it suggests that Jupiter formed in more than five times heavier circumstellar disk than the minimum-mass solar nebula \citep{Shibata+2019}, or Jupiter's core formed in outer disk.
Jupiter and Saturn formed in the same circumsolar disk, so the difference in the amount of heavy elements comes from the different values of $a_{\rm p,0}$ and $M_{\rm p,f}$.
Considering that Saturn contains comparable or smaller amount of heavy elements relative to Jupiter, we suggests that the core formation region of Saturn was outer than that of Jupiter, but at most two times outer than that of Jupiter.

The asteroid belt also gives important constraints on the formation of Jupiter and Saturn.
If Jupiter core formed in outer disk as several tens $\AU$, large amount of planetesimals were shepherded by the mean motion resonances.
More than several $\Mear$ planetesimals were shepherded into the region of asteroid belt even in the disk of $f_{\rm disk}=1$, which is inconsistent with the estimated total amount of solid materials currently distribute in the  asteroid belt $4\times10^{-4}\Mear$ \citep{Pitjeva+2018}.
Formation mechanisms of Kirkwood gaps could reduce the amount of planetesimals around the mean motion resonances of Jupiter, however, removing several Earth-masses planetesimals was difficult because removed planetesimals had been brought into the inner rocky planets.
As a result, the migration distance of Jupiter need to be small.

The grand-Tuck model \citep{Walsh+2011} proposed the solution for the small solid mass in asteroid belt considering the outward migration of giant planets. %triggered by the interactions between Jupiter and Saturn.
In their model, Jupiter and Saturn change migration direction at $1.5\AU$ from inward to outward, which makes it possible for the gas giant planets observed outer than the sweet spot to accrete planetesimals during their  migration phase.
Planetesimals initially located around $1$-$3\AU$ are shepherded into the inner planetesimals disk and terrestrial planets formed in the concentrated planetesimal disk.
After the passage of Jupiter migrating outward, a small amount of planetesimals are scattered from other regions and left in the asteroid belt.
In this case, Jupiter crossed the sweet spot and some parts of shepherded planetesimals accreted onto the planet.
In their original model, however, only a few Earth-masses of planetesimals are captured by Jupiter because the radial distance of inward migration is small $a_{\rm p,0}=3\AU$ and the initial distribution of solid material is similar to minimum-mass solar nebula $f_{\rm disk}\sim1$.
To accrete several tens Earth-masses of planetesimals, we need to consider the case where $a_{\rm p,0}$ and $f_{\rm disk}$ are larger than those in their original model.
For Saturn, $M_{\rm Z,mig}$ might be much smaller than that of Jupiter because planetesimals had been shepherded by Jupiter when Saturn migrates inward.
Thus, Grand-Tuck model does not only explain the structure of the asteroid belt but also the amount of heavy elements in Jupiter and Saturn.
However, large amount of planetesimals are shepherded into the inner disk and final structure of terrestrial planets might be changed from that of the original model.
It is clear that further investigations of ths topic are required. 
%Numerical simulations must be done for further discussions.
% as estimated from observations





\subsection{Model limitations} % and comparison with other models
\label{sec:Application_Model_HeavyElements}
First, in our model, we assume that all the solid material is in the form of planetesimals.
In addition, we neglect the continuous growth of planetesimals via mutual collision of planetesimals.
Second, other protoplanets could form before a gas giant planet starts migration.
%As discussed in \citet{Shibata+2020},
The existence of other planets would affect the accretion of planetesimals because the gravitational scattering of other planets breaks the resonant trapping.
In addition, we neglect the effect of planetesimal collisions on the capture of planetesimals.
Planetesimal collisions have a possibility to break resonant trapping \citep{Malhotra1993}.
So the amount of heavy elements obtained by the planetesimal accretion would be reduced by these effects.
%change the value of $f_{\rm mig}$ used in our model.
In this section, we set $f_{\rm mig}=0.15$ based on the results of numerical simulations in sec.~\ref{sec:sweet_spot_compare}.
In future work, the value of $f_{\rm mig}$ should be investigated in the model including above effects neglected in our model.

Nevertheless, some important features obtained in our model would be valid even in the case where $f_{\rm mig}$ is altered by the above effects.
The first one is that the amount of heavy elements increases with the semi-major axis of core formation region.
The second one is that the scattering in $M_{\rm Z,tot}$ mainly comes from the diversity of the planetesimal disk mass.
These features could explain the distribution of $M_{\rm Z,tot}$ obtained in close-in gas giant planets in \citet{Thorngren+2016}.
%Further observations in gas giant planets to obtain $M_{\rm Z,tot}$ are important for the theory of gas giant planet formation.



==> text/trash/heavy_elements.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}%f1
    \begin{center}
    \includegraphics[width=80mm]{figure/sweet_spot/SS_Type2mig.pdf}
        \caption{
        Distribution of confirmed exoplanets in the semi-major axis vs. planetary mass plane.
        The black points are exoplanets observed by the radial-velocity method.
        The red points are exoplanets observed by the radial-velocity + transit methods.
        As for masses of exoplanets indicated with the black points, the observe values of $M_{\rm p} \sin i$ are simply used.
        The gray area shows the theoretical sweet spot for planetesimal capture given by eqs.~(\ref{eq:sweet_spot_in_disk_1}) and (\ref{eq:sweet_spot_in_disk_2}) with $C=1$.
        }
        \label{fig:Application_Exoplanet}
    \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The location of the sweet spot depends on the ratio of the two timescales of gas drag and tidal damping.
We consider that the planet migrates in the type II regime, the migration rate for which is given  by \citet{Kanagawa+2018} and that the surface density profile in the protoplanetary disk is given by the so-called self-similar solution \citep{Lynden-Bell+1974}, where $\alpha_{\rm disk}\sim1$ except around the outer edge of the protoplanetary disk.
Assuming the optically thin disk $\beta_{\rm disk}=1/2$ and substituting eq.~(\ref{eq:fraction_timescales_simple}) into the analytical expressions of the sweet spots, eqs.~(\ref{eq:condition_for_aerodynamic_shepherding}), (\ref{eq:overstable_libration_due_to_gasdrag}) and (\ref{eq:condition_for_resonant_breaking_grow}), we obtain the inner and outer edge of the sweet spot $a_{\rm SS,in}$ and $a_{\rm SS,out}$ as
\begin{align}
    a_{\rm SS,in} &= {\rm max} \left.
            \begin{cases}
                1.4 C^{1/3} \left(\frac{M_{\rm p}/M_{\rm s}}{10^{-3}}\right)^{2/3} \left(\frac{j}{j-1} \right)^{7/9} \\
                1.1 C^{1/3} \left(\frac{M_{\rm p}/M_{\rm s}}{10^{-3}}\right)^{1/3} \left(\frac{j}{j-1} \right)^{5/18} \frac{e_{\rm cross}}{0.1}
            \end{cases} \right\} \AU, \label{eq:sweet_spot_in_disk_1} \\
    a_{\rm SS,out} &= 7.6 C^{1/3} \left(\frac{M_{\rm p}/M_{\rm s}}{10^{-3}}\right)^{1/3} \left\{ \frac{j^{5}}{(j-1)^{8}} \right\}^{1/18} \AU. \label{eq:sweet_spot_in_disk_2} %\frac{r_{\rm p}}{1\AU} <
    \end{align}
Hereafter, we consider the case of $C=1$ (see eq.~(\ref{eq:sweet_spot_constant_C})).

Figure~\ref{fig:Application_Exoplanet} shows observed exoplanets and the location of the sweet spot in the $a_{\rm p}$-$M_{\rm p}$ plane.
The sweet spot locates from $\sim0.3\AU$ to $10\AU$ and shifts outward with the increase of planetary mass.
The red and black dots show exoplanets observed using  the transit method and the radial velocity method, respectively.
After the onset of runaway gas accretion, $M_{\rm p}$ increases.
Also, $a_{\rm p}$ decreases due to type II planetary migration.
The evolution paths of gas giant planets plane can be drawn from right-bottom to left-top direction in the $a_{\rm p}$-$M_{\rm p}$.
If the runaway gas accretion started in the region exterior to the water snow line, which is considered to locate at $\sim1$-$3\AU$, the exoplanets currently observed in the region interior to the sweet spot crossed the sweet spot during their migration.
On the other hand, the exoplanets currently observed in the region exterior to the sweet spot did not crossed the sweet spot.
Planetesimal mass that is accreted onto the planets would differ between those two populations of planets.
If we observe the difference in the amount of heavy elements between gas giant planets inside and outside the predicted sweet spot, it could be an evidence of planetesimal accretion during planetary migration.
Hereafter, we estimate the heavy-element mass in gas giant planets expected from planetesimal accretion.



%\subsection{Heavy element contents in gas giant planets}\label{sec:Application_Model}
\subsection{A model of planetesimal accretion along formation paths of gas giant planets}\label{sec:Model_PlanetsimalAccretion}
We consider that a protoplanet with a critical core mass $M_{\rm p}=M_{\rm p,0}$ begins runaway gas accretion at $a_{\rm p}=a_{\rm p,0}$.
The planet grows in mass to $M_{\rm p}=M_{\rm p,f}$ thorough a rapid gas accretion, followed by inward migration in the Type II regime and stops at $a_{\rm p}=a_{\rm p,f}$ with $M_{\rm p}=M_{\rm p,f}$ due to disk dissipation.
The formation phase can be divided into two phases, mass growth phase ($M_{\rm p}:M_{\rm p,0}\rightarrow~M_{\rm p,f}$) and planetary migration phase ($r_{\rm p}:r_{\rm p,0}\rightarrow~r_{\rm p,f}$), and planetesimal accretion occurs in both phases.
In the reality the protoplanet is expected to start migrating before runaway gas accretion terminates, but for the sake of simplicity we assume that migration and gas accretion occur one after the other. 
In this case, the total accreted heavy-element mass  $M_{\rm Z,tot}$ is given by: 
\begin{align}
    M_{\rm Z,tot} = M_{\rm Z,core} +M_{\rm Z,grow} +M_{\rm Z,mig}, \label{eq:Application_Mztot}
\end{align}
where $M_{\rm Z,core}$, $M_{\rm Z,grow}$ and $M_{\rm Z,mig}$ are the core mass, planetesimal mass accreted onto the planet during the planetary growth, and the accreted mass during the planetary migration phase, respectively.
\shibata{
----- It would be better to use $M_{\rm Z,crit}$ instead of $M_{\rm Z,core}$.
$M_{\rm Z,crit}$ is a total amount of heavy elements at the onset of runaway gas accretion.
}

The core mass is set as the critical core mass $M_{\rm crit}$, at which runaway gas accretion begins.
Planetesimal accretion after the onset of the runaway gas accretion and core erosion could change the core mass from the critical core mass. 
{\bf what about Claudio's calculations that show that there is a lot of H-He accreted before runaway gas accretion takes place??\\}
Some of the accreted planetesimals during runaway gas accretion could reach the deeep interior  \citep{Mordasini+2006,Valletta2019}.
The convection of envelope gases can erode the solid core and reduce the core mass \citep{Guillot+2004}. 
{\bf but see Cumming et al and references therein  suggesting that giant planets could be radiative... \\}
%from $M_{\rm crit}$ 
Both effects could change the distribution of heavy elements inside the gas giant planet, but the total amount of heavy element $M_{\rm Z,tot}$ is conserved.
To focus on $M_{\rm Z,tot}$, we neglect the effects which could change the heavy-element distribution.
{\bf so why are we discussing it in detail??\\}
\shibata{
------ Maybe we don't need to discuss on this point...
}

%Thus, we consider that the core mass does not change after the onset of the rapid gas accretion.
Recent studies suggest $M_{\rm crit}\lesssim10\Mear$ \citep{Hori+2011,Venturini+2015,Brouwers+2018}.
Here we set $M_{\rm Z,core}=10\Mear$.

During the early stages of the planetary growth, the heavy-element accretion depends on the mass of planetesimals inside the planetary feeding zone.
The planetesimal accretion rate depends on the timescales of planetary mass growth and gas damping of planetesimal orbits \citep{Shiraishi+2008,Shibata+2019}.
We define the fraction of planetesimals captured by the planet in the early phase $f_{\rm growth}$ as
\begin{align}
    f_{\rm growth} \equiv \frac{M_{\rm Z,grow}}{M_{\rm Z,fz}(a_{\rm p,0},M_{\rm p,f})}.
\end{align}
where $M_{\rm Z,fz}$ is the mass of planetesimals inside the feeding zone given as
\begin{align}
    M_{\rm Z,fz} (a_{\rm p},M_{\rm p}) &= \int_{\rm a_{\rm fz,in}(a_{\rm p},M_{\rm p})}^{\rm a_{\rm fz,out}(a_{\rm p},M_{\rm p})} 2 \pi r \Sigma_{\rm solid} {\rm d} r,
\end{align}
with
\begin{align}
    a_{\rm fz,in}   &= a_{\rm p} \left\{1-2\sqrt{3} \left(\frac{M_{\rm p}}{3M_{\rm s}} \right)^{1/3} \right\}, \label{eq:feeding_zone_0_axi_in} \\
    a_{\rm fz,out}  &= a_{\rm p} \left\{1+2\sqrt{3} \left(\frac{M_{\rm p}}{3M_{\rm s}} \right)^{1/3} \right\}. \label{eq:feeding_zone_0_axi_out}
\end{align}
According to the results of numerical simulations by \citet{Shibata+2019}, $f_{\rm growth}$ takes $\lesssim0.3$. % and takes the maximum when the timescale of mass growth is shorter than the timescale of gas damping.

On the other hand, during planetary migration the  planet can capture planetesimals which are shepherded into the sweet spot $M_{\rm Z,shep}$.
During the migration, planetesimals initially located from the inner edge of the sweet spot $a_{\rm SS,in}$ to the inner edge of the feeding zone when the planet begins to migrate $a_{\rm fz,in}(a_{\rm p,0},M_{\rm p,f})$ have a possibility to be shepherded into the sweet spot.
$M_{\rm Z,shep}$ is given by
\begin{align}
    M_{\rm Z,shep} &= \int_{\rm a_{\rm SS,in}}^{\rm a_{\rm fz,in}} 2 \pi r \Sigma_{\rm solid} {\rm d} r. \label{eq:M_z_shep}
\end{align}
%$a_{\rm SS,in}$ is given by eqs.~(\ref{eq:sweet_spot_in_disk_1}) and (\ref{eq:sweet_spot_in_disk_2}).
We define the fraction of planetesimals captured by the planet during planetary migration as
\begin{align}
    f_{\rm mig} \equiv \frac{M_{\rm Z,mig}}{M_{\rm Z,shep}}.
\end{align}
where we found that $f_{\rm mig}$ is $\lesssim 0.3$.
%Note that $a_{\rm SS,in}$ depends on many parameters like $\alpha_{\rm vis}$ and $R_{\rm pl}$ as shown in eq.~\ref{eq:sweet_spot_constant_C}.
%Here we neglect those effects on $M_{\rm Z,tot}$ because the variation in $f_{\rm disk}$ is much more important for estimating $M_{\rm Z,tot}$ as shown below.

Both $M_{\rm Z,growth}$ and $M_{\rm Z,mig}$ depend on the radial distribution of planetesimals in the protoplanetary disk.
Two potential planetesimal formation mechanisms include:
continuous coagulation of fluffy dust particles \citep{Okuzumi+2012} and
gravitational contraction of particle clumps formed by the streaming instability \citep{Youdin+2005}.
In recent studies, the planetesimal formation through the streaming instability is actively discussed because it can directly form km-size planetesimals from pebble-size particles skipping problems concerning the continuous growth of small particles, such as the bouncing problem of collision growth \citep{Windmark+2012}.
In addition, observed features in Solar System's Kuiper belt objects support the formation of planetesimals through the streaming instability.
The Kuiper belt binaries are typically made of the similar size and the same color objects \citep{Noll+2008}, which is consistent with the result that the formation of a binary is the natural result of the gravitational collapse of the pebble clump \citep{Nesvorny+2010}.
The streaming instability requires sedimentation of particles in disks with more than $\sim1\%$ metallicity  \citep{Youdin+2002,Johansen+2009,Simon+2016}.
Certain locations like the vicinity of snowline \citep{Armitage+2016} or the vicinity of disk inner edge \citep{Drazkowska+2016} enhance the local disk metallicity due to the pile up of radially drifted pebbles.
Even in other locations, non-laminar flow, or zonal flow originating from various instabilities, traps radially drifted solid particles and enhances local solid-to-gas ratio \citep[see references in][]{Klahr+2018,Lenz+2019}.
These studies suggest that planetesimal formation through the streaming instability can be triggered everywhere in the circumstellar disk.
Assuming the planetesimal formation rate depends on the instantaneous radial pebble flux, \citet{Lenz+2019} found that the surface density profile of planetesimals tends to be steeper than that of gas.
Their model helps explain the discrepancy between the minimum-mass solar nebula, which is modeled from the distribution of solid materials in our solar system, and viscous accretion disks.
Here, we consider the limiting case where planetesimal formation occurs everywhere in the disk and all solid materials are in the form of planetesimals.
We set $\alpha_{\rm disk}^{\prime}=3/2$ and parameterize $\Sigma_{\rm solid}$ using a scaling factor $f_{\rm disk}$ as
\begin{align}
    \Sigma_{\rm solid}  &= f_{\rm disk} \times
        \begin{cases}
            7.1\times\left(\frac{r}{1\AU}\right)^{-3/2}~\text{ for } r<r_{\rm ice} \\
            30.\times\left(\frac{r}{1\AU}\right)^{-3/2}~\text{ for } r_{\rm ice}<r,
        \end{cases} \label{eq:disk_solid_MMSN}
\end{align}
where $r_{\rm ice}$ is the radial distance of the water ice line and given as $r_{\rm ice}\sim2.7\AU$ in our disk model.
The values of $\Sigma_{\rm solid}$ for $f_{\rm disk}=1$ is the same as that in the minimum-mass solar nebula.
Given the initial formation location $a_{\rm p,0}$ and observed parameters $a_{\rm p,f}$ and $M_{\rm p,f}$, we can calculate the amounts of heavy elements in gas giant planets $M_{\rm Z,tot}$ from the above equations.


\subsection{Heavy element content of inner gas giant planets}\label{sec:Application_Model_InnerPlanet_result}
\subsubsection{Model estimate}\label{sec:Application_result_innerplanet}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}%f1
  \begin{center}
    \includegraphics[width=80mm]{figure/discussion/Axip0_Mpz_Mcap.pdf}
    \caption{
    The estimated heavy-element mass in a gas giant planet as a function of the initial semi-major axis of the planet $a_{\rm p,0}$.
    We consider the case of $f_{\rm disk}=2$ and $M_{\rm p,f}/M_{\rm s}=10^{-3}$.
    The red, green, and blue lines show $M_{\rm Z,core}$, $M_{\rm Z,grow}$ and $M_{\rm Z,mig}$, respectively.
    The black solid line shows $M_{\rm Z,tot}$ for planets which crossed the sweet spot in the planetary migration phase.
    The black dashed line shows $M_{\rm Z,tot}$ for planets which did not reach the sweet spot, namely $M_{\rm Z,tot}=M_{\rm Z,core}+M_{\rm Z,mig}$.
    }
    \label{fig:Application_Mtot}
  \end{center}
\end{figure}
%
\begin{figure}%f1
  \begin{center}
    \includegraphics[width=80mm]{figure/discussion/mu_Mpz_Mcap_Axip20.pdf}
    \caption{
    Same as Fig.~\ref{fig:Application_Mtot}, but as a function of the final planet mass $M_{\rm p,f}$.
    We consider the case of $f_{\rm disk}=2$ and $a_{\rm p,0}=20~\AU$.
    }
    \label{fig:Application_Mtot2}
  \end{center}
\end{figure}
%
\begin{figure}%f1
  \begin{center}
    \includegraphics[width=80mm]{figure/discussion/hist_fdiskp.pdf}
    \caption{
    The distribution of $f_{\rm disk}$ of circumstellar disks in star formation regions.
    $f_{\rm disk}$ is calculated from the disk total mass $M_{\rm disk}$ and disk characteristic radius $R_{\rm disk}$ obtained in \citet{Andrews+2010}.
    Here, we assume that the disk inner edge locates at $0.1~\AU$ and $Z_{\rm s}=Z_{\rm \odot}$ for simplicity.
    }
    \label{fig:Application_fdisk}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Here we investigate the accreted heavy-element mass for  giant planets in regions interior to the sweet spot. 
These planets crossed the sweet spot during their formation stages if the planets started runaway gas accretion in the outer disk as $1\AU\lesssim~a_{\rm p,0}$.
We set $f_{\rm growth}=0.3$ and $f_{\rm mig}=0.15$, which was obtained from our numerical calculations in \citet{Shibata+2019} and in sec.~\ref{sec:sweet_spot_compare}.
The mass of the planetesimal disk is set as $f_{\rm disk}=2$.
Note that the value of $f_{\rm growth}$ and $f_{\rm mig}$ depends on various physical conditions such as the planetary growth rate and the  capture radius.
Here, we neglect those effects and use the results of specific numerical simulations.
Detailed investigations of $f_{\rm growth}$ and $f_{\rm mig}$ should be done in future works.

Figure~\ref{fig:Application_Mtot} shows the estimated heavy-element mass  $M_{\rm Z,tot}$ as a function of the initial semi-major axis of the planet $a_{\rm p,0}$. %where the planet started runaway gas accretion
During the accretion phase, the amount of planetesimals inside the feeding zone $M_{\rm Z,fz}$ increases with $a_{\rm p,0}$ because the area of the feeding zone expands. %increases approximately with ${a_{\rm p,0}}^2$.
During the planetary migration, the amount of planetesimals shepherded into the sweet spot $M_{\rm Z,shep}$ increases with $a_{\rm p,0}$.
As a result, both of the amounts of planetesimals accreting onto the planet during the accretion phase $M_{\rm Z,grow}$ and the planetary migration phase $M_{\rm Z,mig}$ increase with $a_{\rm p,0}$.
$M_{\rm Z,mig}$ more rapidly increases with $a_{\rm p,0}$ than $M_{\rm Z,grow}$ and $M_{\rm Z,mig}$ becomes larger than $M_{\rm Z,grow}$ around $\sim10\AU$.
The total heavy-element mass $M_{\rm Z,tot}$ also increases with $a_{\rm p,0}$ and several tens Earth-masses of planetesimals are captured by the planet if the planet starts the runaway gas accretion at $a_{\rm p,0}\gtrsim10\AU$.

Figure~\ref{fig:Application_Mtot2} shows $M_{\rm Z,tot}$ vs.~the final planetary mass $M_{\rm p,f}$.
Here, we set $a_{\rm p,0}=20\AU$.
As the planetary mass increases, $M_{\rm Z,grow}$ increases because the feeding zone expands with $M_{\rm p,f}$.
On the other hand, $M_{\rm Z,mig}$ decreases with $M_{\rm p,f}$ because the inner edge of the sweet spot $a_{\rm SS,in}$ moves outward.
As a result, $M_{\rm Z,tot}$ increases slightly with $M_{\rm p,f}$.

In the above results, we considered the case where the mass of the planetesimal disk $f_{\rm disk}$ is set as 2.
However, $f_{\rm disk}$ must change among between different disks and $M_{\rm Z,tot}$ linearly increases with $f_{\rm disk}$.
We consider that the disk of mass $M_{\rm disk}$ has a radius $R_{\rm disk}$ and a metallicity of $Z_{\rm s}$.
Assuming a continuous solid distribution, we can obtain $f_{\rm disk}$ from $M_{\rm disk}$, $R_{\rm disk}$ and $Z_{\rm s}$.
%We consider that $f_{\rm disk}$ relates with the disk total mass $M_{\rm disk}$, the characteristic disk radius $R_{\rm disk}$ and the metallicity of central star $Z_{\rm s}$.
According to observations of protoplanetary disks in star formation regions \citep{Andrews+2010}, the most frequent disk total mass and characteristic disk radius are $\sim0.03\Msun$ and $\sim50\AU$, respectively.
The disk mass and radius also have large scatterings: from $0.004\Msun$ to $0.136\Msun$ in disk total mass and from $14\AU$ to $198\AU$ in characteristic disk radius.
Given $M_{\rm disk}$ and $R_{\rm disk}$, we can obtain the value of $f_{\rm disk}$ solving
%\begin{align}
%    f_{\rm disk} = \frac{M_{\rm disk}}{4 \pi \Sigma_{\rm MMSN,0}} \left( R_{\rm disk}^{1/2}-R_{\rm disk,in}^{1/2} \right)^{-1}, \label{eq:Calculating_fdisk}
%\end{align}
\begin{align}
    Z_{\rm s} M_{\rm disk} = \int_{R_{\rm disk,in}}^{R_{\rm disk}} 2 \pi \Sigma_{\rm solid} {\rm d} r, \label{eq:Calculating_fdisk}
\end{align}
where $R_{\rm disk,in}$ is the radial distance of the disk inner edge.
Assuming the disk inner edge locates at $0.1\AU$ and $Z_{\rm s}=Z_{\odot}$, we can obtain $f_{\rm disk}$ from observed $M_{\rm disk}$ and $R_{\rm disk}$. % and metallicity of central star is same as solar metallicity $Z_{\rm \odot}$
Figure.~\ref{fig:Application_fdisk} shows the distribution of $f_{\rm disk}$ of disks used in \citet{Andrews+2010}.
Around stars with the solar metallicity, $f_{\rm disk}$ is most frequent around $\sim2$ and scattered in a wide range.
Considering the scattering in the metallicity of the  host stars, we suggest that $f_{\rm disk}$ changes from $\sim0.2$ to $\sim10$. % in two orders magnitude.
Thus, the distributions of $M_{\rm Z,tot}$ also has large scattering.

The scattering in $M_{\rm Z,tot}$ also comes from the scattering of other parameters.
$M_{\rm Z,tot}$ depends on $M_{\rm Z,shep}$, which decreases with the location of the inner edge of the sweet spot ${a_{\rm SS,in}}$. %^{1/2}
The location of the sweet spot depends on many parameters, such as disk viscosity $\alpha_{\rm vis}$, planetesimal density $\rho_{\rm pl}$, planetesimal size $R_{\rm pl}$, mass of central star $M_{\rm s}$, and disk temperature at $1\AU$ $T_{\rm disk,0}$ as shown in eqs.~(\ref{eq:sweet_spot_constant_C}) and (\ref{eq:sweet_spot_in_disk_2}). %sec.~\ref{sec:Part1_Discussion_SweetSpot}.
From eqs.~(\ref{eq:sweet_spot_constant_C}), (\ref{eq:sweet_spot_in_disk_2}) and (\ref{eq:M_z_shep}), we find that $M_{\rm Z,tot}$ depends on the $-1/6$ power of $\alpha_{\rm vis}$, $\rho_{\rm pl}$, $R_{\rm pl}$ and $M_{\rm s}$, and the $1/3$ power of $T_{\rm disk,0}$.
Here, we use the relation of $|h_{\rm s}/r|_{\rm 1AU}\propto {M_{\rm s}}^{-1/2} {T_{\rm disk,0}}^{1/2}$.
The effects of the scatterings in these parameters are smaller than the effect of the scattering in $f_{\rm disk}$, with which $M_{\rm Z,tot}$ increases linearly.
We conclude that the scattering in $M_{\rm Z,tot}$ mainly comes from the scattering in the disk mass $f_{\rm disk}$.


\subsubsection{Comparison with \citet{Thorngren+2016}}\label{sec:Application_Thorngren+2016}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}%f1
  \begin{center}
    \includegraphics[width=80mm]{figure/discussion/mu_Mpz.pdf}
    \caption{
    The amounts of heavy elements of gas giant planets estimated in \citet{Thorngren+2016} with the mass fraction $M_{\rm p}/M_{\rm s}$.
    }
    \label{fig:Application_Thorngren_mu_Mpz}
  \end{center}
\end{figure}
%
\begin{figure}%f1
  \begin{center}
    \includegraphics[width=80mm]{figure/discussion/hist_Mpz.pdf}
    \caption{
    The histogram of the amount of heavy elements $M_{\rm Z,tot}$ estimated in \citet{Thorngren+2016}.
    We select only the data the errors of which are less than $50\%$ from the samples in \citet{Thorngren+2016} and the number of selected samples is 32.
    The black bars show the histogram of all the samples and the red bars are Jupiter-size planets which have $10^{-3.5}<M_{\rm p}/M_{\rm s}<10^{-2.5}$.
    The width of the bin is set as $0.2$ in logarithmic scale.
    }
    \label{fig:Application_Thorngren}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Some of the gas giant planets that are located in the inner disk interior to the sweet spot are observed by both the radial velocity and transit methods and, thereby, their mass and radius are both measured.
\citet{Thorngren+2016} estimated the amounts of heavy elements in close-in gas giant planets and found some important features in the distribution of $M_{\rm Z,tot}$.
Figure~\ref{fig:Application_Thorngren_mu_Mpz} shows the $M_{\rm Z,tot}$ estimated in \citet{Thorngren+2016} with $M_{\rm p}/M_{\rm s}$. % instead of $M_{\rm p}$.
Here, we focus on the features found in the distribution of $M_{\rm Z,tot}$;
(i) $M_{\rm Z,tot}$ increases with $M_{\rm p}/M_{\rm s}$,
(ii) $M_{\rm Z,tot}$ have large diversity between similar mass planets,
(iii) there are some extremely enriched planets as $M_{\rm Z,tot}\gtrsim100\Mear$.
Note that \citet{Muller+2020} showed that the uncertainties originating from the model assumptions used in \citet{Thorngren+2016} are comparable or even larger than those from observation.
Hereafter we focus on the qualitative features obtained by \citet{Thorngren+2016} and discuss the formation of close-in gas giant planets using our model.

\citet{Thorngren+2016} derived a relation $M_{\rm Z,tot}~\propto~{M_{\rm p}}^{2/3}$ by fitting their estimated values.
In Fig.~\ref{fig:Application_Thorngren_mu_Mpz}, we take $M_{\rm p}/M_{\rm s}$ as the horizontal axis instead of $M_{\rm p}$ and find that $M_{\rm Z,tot}$ also increases with $M_{\rm p}/M_{\rm s}$.
In our model, $M_{\rm Z,tot}$ depends on $M_{\rm p}/M_{\rm s}$ but the dependence is too weak to explain the observed relation between $M_{\rm Z,tot}$ and $M_{\rm p}/M_{\rm s}$ (see Fig.~\ref{fig:Application_Mtot2}).
On the other hand, $M_{\rm Z,tot}$ increases with $a_{\rm p,0}$ (see Fig.~\ref{fig:Application_Mtot}).
To explain the relation between $M_{\rm Z,tot}$ and $M_{\rm p}/M_{\rm s}$, we suggest that heavier close-in gas giant planets had formed cores of critical mass farther away from the central stars and then migrated over longer radial distances.
Such a relation between the initial formation location and the final planet mass of gas giant planet is also suggested from the formation theories of gas giant planets.
The model combining the gas accretion rate and planetary migration rate \citep{Tanigawa+2007,Tanigawa+2016} showed that planets which start runaway gas accretion in the outer disk grow to be heavier planets.
The evolution paths shown in population synthesis models \citep[e.g.][]{Bitsch+2015,Mordasini2014,Ida+2018} also imply that heavier gas giant planets migrate longer radial distances and the possibility for Jupiter-mass planets to migrate several tens $\AU$ in planetary migration phase.
On the other hand, \citet{Tanaka+2020} showed that close-in gas giant planets with $M_{\rm p}/M_{\rm s}\lesssim10^{-2}$ had started runaway gas accretion interior to the water snow line and migrated only a few $\AU$ in their formation stages.
Along their formation paths, close-in gas giant planets barely capture planetesimals and the outcome is inconsistent with the result in \citet{Thorngren+2016}.
To migrate long distance, gas giant planets needs to move before reaching higher planetary mass, because migration timescale in type II regime increases with the planetary mass.
Our results suggest that the migration timescale compared to the mass growth timescale is smaller than that used in \citet{Thorngren+2016}.

\begin{comment}
In the above formation models, the radial migration distance of gas giant planets is determined by the competitions between the timescales of gas accretion and planetary migration.
Both timescales depend on the gap structure opened by the planet and the studies of these timescales are still under discussion, especially for the gas accretion timescale.
\citet{Tanigawa+2002} investigated the gas accretion rate of giant planets using a two-dimensional hydrodynamic simulations.
They found that gas accretion occurs through a narrow band and derived an analytical formula for the width of the accretion band.
Three-dimensional hydrodynamic simulations, however, showed the possibilities that gas accretion rate is smaller than that obtained in two-dimensional hydrodynamic simulations \citep{Lissauer+2009,Machida+2010}.
%The timescale of type II migration is regulated by the viscous timescale of the circumstellar disk in the classical regime \citep[e.g.][]{Lin+1993}.
\citet{Kanagawa+2018} investigated the migration timescale using two-dimensional hydrodynamic simulations and found that the migration timescale for gap opening planets depends on the surface density of disk gas at the gap bottom. %is longer than the classical one.
Their fitting model of migration timescale, which is written by eq.~(\ref{eq:type2_migration_regime_K18}), has still uncertainties up to 1 order.
In the model of \citet{Tanaka+2020}, the migration timescale is long relative to the gas accretion timescale, which results in the short migration distance.
If the migration rate is faster than that used in their model, the migration distance becomes longer.
Thus, our model suggests the possibility that gas accretion timescale is longer than that obtained in two-dimensional hydrodynamic simulations.
\end{comment}

The large scattering in $M_{\rm Z,tot}$ between similar mass planets is also important characteristic of close-in gas giant planets.
Figure~\ref{fig:Application_Thorngren} shows the histogram of $M_{\rm Z,tot}$ estimated in \citet{Thorngren+2016}.
To draw this figure, we select only the data, the errors of which are less than $50\%$ from the samples in \citet{Thorngren+2016} and the number of selected samples is 32.
The black bars show the histogram of all the samples and the red bars are Jupiter-size planets which have $10^{-3.5}<M_{\rm p}/M_{\rm s}<10^{-2.5}$.
The distribution of $M_{\rm Z,tot}$ of Jupiter-size planets spreads from $10\Mear$ to $200\Mear$ and the peak of the distribution is around $50\Mear$.
As discussed in sec.~\ref{sec:Application_result_innerplanet}, the scattering in $M_{\rm Z,tot}$ mainly comes from the scattering of $0.2~\lesssim~f_{\rm disk}~\lesssim~10$, which covers the scattering found in $M_{\rm Z,tot}$ estimated by \citet{Thorngren+2016}.
The effects of other parameters, such as the disk viscosity or planetesimal radius, are not enough to generate such a large scattering.
We suggests that the large scattering shown in the distribution of $M_{\rm Z,tot}$ comes from the scattering of $f_{\rm disk}$.
This suggestion should be discussed in future when the number of observations in $M_{\rm Z,tot}$ and circumstellar disk increases.

Finally, we focus on some close-in gas giant planets that contain more than $100\Mear$ heavy elements as shown in Fig.~\ref{fig:Application_Thorngren_mu_Mpz}.
To capture such massive heavy elements via planetesimal accretion, those planets need to be formed in a massive circumstellar disk as $f_{\rm disk}\sim10$ and migrate more than $\gtrsim50\AU$. %from the outer edge of the circumstellar disk.
Disk instability model is preferred for such formation paths of gas giant planets than core accretion model.
Our model suggests that close-in gas giant planets containing more than $100\Mear$ heavy elements formed via disk instability.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Heavy element contents in outer gas giant planets} \label{sec:Application_Model_OuterPlanet}
Gas giant planets which locate in the region exterior to the sweet spot are observed by radial velocity method and, thereby, their masses are measured as shown in fig.~\ref{fig:Application_Exoplanet}.
Jupiter and Saturn also locate in this region.
Here we consider the amounts of heavy elements contained in gas giant planets which locate in the region exterior to the sweet spot.

\subsubsection{In exoplanets}
\label{sec:Application_Model_OuterExoplanets}
%Here, we consider the single gas giant planet and do not consider the outward migration as considered in Grand-Tuck model \citep{Walsh+2011}, which occurs in multi-planetary systems.
We consider the heavy elements contents in exoplanets observed in the region exterior to the sweet spot.
During the formation phase, the circumstellar disk dissipated before the planets reached the sweet spot.
In this case, the accretion of planetesimals did not occur in the planetary migration phase.
Between the populations of planets which locate in the regions interior and exterior to the sweet spot, a clear difference in $M_{\rm Z,tot}$ would exist.
If we can observe the clear difference in $M_{\rm Z,tot}$ between these populations, it suggests that the heavy elements in gas giant planets are mainly brought by planetesimal accretion.

The transition frequency and probability decrease with the orbital period of planets.
So the transit observation of planets in the region exterior to the sweet spot is lack now.
Considering the scattering of $M_{\rm Z,tot}$, we need large number of observations to compare the populations.
In addition, we need high accuracy in measuring the radius of those gas giant planets.
If the formation of Jupiter-size planet starts around $a_{\rm p,0} \sim 20\AU$ in the disk of $f_{\rm disk}=2$, the planets which crossed the sweet spot contain more $\sim10\Mear$ heavy elements than the planets which did not reached the sweet spot during the planetary migration phase (see fig.~\ref{fig:Application_Mtot}).
The $10\Mear$ difference in the amount of heavy elements in Jupiter-mass planet makes a few percent difference in the radius of the planets $\sim0.01~R_{\rm Jup}$ \citep{Thorngren+2016}.
$\sim1\%$ accuracy in the observation of planet radius is limited for some planetary systems.
In conclusion, long term and wide field observations with high accuracy are required for comparing the populations of planets in the regions interior and exterior to the sweet spot.
Such observation should be done in future.

\subsubsection{Jupiter and Saturn}\label{sec:Application_Model_SolarSystem}
For the gas giant planets in our solar system, not only the mass and radius but also the gravitational moments $J_{n}$ are measured. 
%by spacecrafts exploration.
The bulk amounts of heavy elements contained in Jupiter and Saturn are not well-determined but are estimated to be $\sim24$-$46\Mear$ and $\sim16$-$30\Mear$, respectively.
Jupiter and Saturn are located in the region exterior to the sweet spot, and the accretion of planetesimals probably did not occur during  planetary migration phase. {\bf I am not sure I understand what you mean...\\}
The heavy elements in Jupiter come from the initial core and accretion of planetesimals in mass growth phase.
In this case, the amount of heavy elements increases with $f_{\rm disk}$, $a_{\rm p,0}$ and $M_{\rm p,f}$.
If this is indeed the case, it suggests that Jupiter formed in more than five times heavier circumstellar disk than the minimum-mass solar nebula \citep{Shibata+2019}, or Jupiter's core formed in outer disk.
Jupiter and Saturn formed in the same circumsolar disk, so the difference in the amount of heavy elements comes from the different values of $a_{\rm p,0}$ and $M_{\rm p,f}$.
Considering that Saturn contains comparable or smaller amount of heavy elements relative to Jupiter, we suggests that the core formation region of Saturn was outer than that of Jupiter, but at most two times outer than that of Jupiter.

The asteroid belt also gives important constraints on the formation of Jupiter and Saturn.
If Jupiter core formed in outer disk as several tens $\AU$, large amount of planetesimals were shepherded by the mean motion resonances.
More than several $\Mear$ planetesimals were shepherded into the region of asteroid belt even in the disk of $f_{\rm disk}=1$, which is inconsistent with the estimated total amount of solid materials currently distribute in the  asteroid belt $4\times10^{-4}\Mear$ \citep{Pitjeva+2018}.
Formation mechanisms of Kirkwood gaps could reduce the amount of planetesimals around the mean motion resonances of Jupiter, however, removing several Earth-masses planetesimals was difficult because removed planetesimals had been brought into the inner rocky planets.
As a result, the migration distance of Jupiter need to be small.

The grand-Tuck model \citep{Walsh+2011} proposed the solution for the small solid mass in asteroid belt considering the outward migration of giant planets. %triggered by the interactions between Jupiter and Saturn.
In their model, Jupiter and Saturn change migration direction at $1.5\AU$ from inward to outward, which makes it possible for the gas giant planets observed outer than the sweet spot to accrete planetesimals during their  migration phase.
Planetesimals initially located around $1$-$3\AU$ are shepherded into the inner planetesimals disk and terrestrial planets formed in the concentrated planetesimal disk.
After the passage of Jupiter migrating outward, a small amount of planetesimals are scattered from other regions and left in the asteroid belt.
In this case, Jupiter crossed the sweet spot and some parts of shepherded planetesimals accreted onto the planet.
In their original model, however, only a few Earth-masses of planetesimals are captured by Jupiter because the radial distance of inward migration is small $a_{\rm p,0}=3\AU$ and the initial distribution of solid material is similar to minimum-mass solar nebula $f_{\rm disk}\sim1$.
To accrete several tens Earth-masses of planetesimals, we need to consider the case where $a_{\rm p,0}$ and $f_{\rm disk}$ are larger than those in their original model.
For Saturn, $M_{\rm Z,mig}$ might be much smaller than that of Jupiter because planetesimals had been shepherded by Jupiter when Saturn migrates inward.
Thus, Grand-Tuck model does not only explain the structure of the asteroid belt but also the amount of heavy elements in Jupiter and Saturn.
However, large amount of planetesimals are shepherded into the inner disk and final structure of terrestrial planets might be changed from that of the original model.
It is clear that further investigations of ths topic are required. 
%Numerical simulations must be done for further discussions.
% as estimated from observations





\subsection{Model limitations} % and comparison with other models
\label{sec:Application_Model_HeavyElements}
First, in our model, we assume that all the solid material is in the form of planetesimals.
In addition, we neglect the continuous growth of planetesimals via mutual collision of planetesimals.
Second, other protoplanets could form before a gas giant planet starts migration.
%As discussed in \citet{Shibata+2020},
The existence of other planets would affect the accretion of planetesimals because the gravitational scattering of other planets breaks the resonant trapping.
In addition, we neglect the effect of planetesimal collisions on the capture of planetesimals.
Planetesimal collisions have a possibility to break resonant trapping \citep{Malhotra1993}.
So the amount of heavy elements obtained by the planetesimal accretion would be reduced by these effects.
%change the value of $f_{\rm mig}$ used in our model.
In this section, we set $f_{\rm mig}=0.15$ based on the results of numerical simulations in sec.~\ref{sec:sweet_spot_compare}.
In future work, the value of $f_{\rm mig}$ should be investigated in the model including above effects neglected in our model.

Nevertheless, some important features obtained in our model would be valid even in the case where $f_{\rm mig}$ is altered by the above effects.
The first one is that the amount of heavy elements increases with the semi-major axis of core formation region.
The second one is that the scattering in $M_{\rm Z,tot}$ mainly comes from the diversity of the planetesimal disk mass.
These features could explain the distribution of $M_{\rm Z,tot}$ obtained in close-in gas giant planets in \citet{Thorngren+2016}.
%Further observations in gas giant planets to obtain $M_{\rm Z,tot}$ are important for the theory of gas giant planet formation.


